Asymptotic Performance of TDOA Estimation using Satellites

We present novel lower bounds on the localization error using a network of satellites randomly deployed on a sphere around Earth. Our new analysis approach characterizes the localization performance by its asymptotic behavior as the number of satellites gets large while assuming a dense network. Using the law of large numbers, we derive closed-form expressions for the asymptotic Cramer Rao bound (CRB) from which we draw valuable insights. The resulting expressions depend solely on the network statistics and are not a function of a particular network configuration. We consider two types of estimators. The first uses the exact statistical model, and hence employs both timing and amplitude information. The second estimator ignores the amplitudes and hence uses only time difference of arrival (TDOA) information. The asymptotic CRB indicates that for practical system setup, a TDOA estimator approaches the performance of the ideal estimator. For both estimators, the localization accuracy improves as satellites get closer to Earth. The latter finding is essential in light of the proliferation of low-Earth-orbit (LEO) satellites and motivates a further study of localization-performance in such networks. Besides, we show that the vertical localization accuracy is lower than the horizontal accuracy and is also more sensitive to the receiver field-of-view.

==> Chapters/CRB_TDOA_derivation.tex <==
In this section, the derivation of TDOA CRB is presented.
The final result is:
\begin{eqnarray}
\textit{CRB}&=&\frac{6c^2\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij}))}{4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}[\sin(\alpha_{jk})+\sin(\alpha_{ki})+\sin(\alpha_{ij})]^2}\nonumber\\
&=&\frac{3c^2\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij})) }{4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})}
\label{CRBlast}\nonumber\\
&&
\end{eqnarray}
This is an intuitive and insightful expression. 
The matrix form of this bound is already known \cite{myref12}. After some adaptations to our model, and using the notation $\sum_i=\sum_{i=1}^M$, the FIM of estimating $\theta$ from the sensors is:
\begin{eqnarray}
\textbf{J}=\mu_1\overline{H}\Lambda\overline{H}^T=\mu_1
\begin{pmatrix}
\cos\phi_1&\cos\phi_2&\dots&\cos\phi_M\\
\sin\phi_1&\sin\phi_2&\dots&\sin\phi_M\\
-1&-1&\dots&-1\\
\end{pmatrix}
\Lambda
\begin{pmatrix}
\cos\phi_1&\sin\phi_1&-1\\
\cos\phi_2&\sin\phi_2&-1\\
\vdots&\vdots& \vdots\\
\cos\phi_M&\sin\phi_M&-1\\
\end{pmatrix}\nonumber\\
= 
\frac{4W_e\rho}{c^2}\begin{pmatrix}
\sum_iD_i^{-\gamma} \cos^2\phi_i&
\sum_iD_i^{-\gamma} \cos\phi_i\sin\phi_i& -\sum_iD_i^{-\gamma} \cos\phi_i\\
\sum_iD_i^{-\gamma} \cos\phi_i\sin\phi_i&
\sum_iD_i^{-\gamma} \sin^2\phi_i& -\sum_iD_i^{-\gamma} \sin\phi_i\\
-\sum_iD_i^{-\gamma} \cos\phi_i&
-\sum_iD_i^{-\gamma} \sin\phi_i&
\sum_iD_i^{-\gamma}
\end{pmatrix}.
\end{eqnarray}
We are only interested in finding $[x,y]$ and $T_0$ is a nuisance parameter. Thus:
\begin{equation}
\textit{CRB}=\trace \{\textbf{J}^{-1}\}_{2\times 2}=(\textbf{J}^{-1})_{1,1}+(\textbf{J}^{-1})_{2,2}
\end{equation}
In order to get an element $i,j$ of $\textbf{J}^{-1}$, the matched minor $M_{i,j}$ must be calculated and divided by $\det (\textbf{J})$.\\
The first minor is given by
\begin{equation}
\frac{M_{1,1}}{\eta^2}=\left(\sum_i D_i^{-\gamma} \right)\left(\sum_iD_i^{-\gamma} \sin^2 \phi_i  \right)-\left(\sum_iD_i^{-\gamma} \sin \phi_i\right)^2
\end{equation}
where $\eta=4W_e\rho/c^2$. The second minor is identical, but with a cosine instead of a sinus. Thus, the combination yields:
\begin{eqnarray}
\frac{M_{1,1}+M_{2,2}}{\eta^2}&=&\left(\sum_iD_i^{-\gamma}\right)^2-\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(\sin\phi_i\sin\phi_j+\cos\phi_i\cos\phi_j)\nonumber\\
&=&\left(\sum_iD_i^{-\gamma}\right)^2-\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}\cos(\phi_i-\phi_j)\nonumber\\
&=&\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}\left(1-\cos(\phi_i-\phi_j) \right)   
\end{eqnarray}
Now, the determinant needs to be calculated:
\begin{eqnarray}
\det\left(\frac{\textbf{J}}{\eta}\right)&=&\left(\sum_iD_i^{-\gamma}\cos^2\phi_i\right)\left(\left(\sum_iD_i^{-\gamma}\right)\left(\sum_iD_i^{-\gamma}\sin^2\phi_i\right)-\left(\sum_iD_i^{-\gamma} \sin\phi_i\right)^2\right)\nonumber\\ &\quad&-\left(\sum_iD_i^{-\gamma}\cos\phi_i\sin\phi_i\right)\left(\left(\sum_iD_i^{-\gamma}\cos\phi_i\sin\phi_i\right)\left(\sum_iD_i^{-\gamma}\right)\right.\nonumber\\ &\quad&\left.-\left(\sum_iD_i^{-\gamma} \sin \phi_i\right)\left(\sum_iD_i^{-\gamma}\cos\phi_i\right)\right)+\left(\sum_iD_i^{-\gamma} \cos\phi_i\right)\nonumber\\ &\quad&\left(\left(\sum_iD_i^{-\gamma} \cos\phi_i\sin\phi_i\right)\left(\sum_iD_i^{-\gamma}\sin\phi_i\right)-\left(\sum_iD_i^{-\gamma} \sin^2 \phi_i\right)\right.\nonumber\\ &\quad&\left.\left(\sum_iD_i^{-\gamma}\cos\phi_i\right)\right)  
\end{eqnarray}
and after combining the separate sums into three large ones:
\begin{eqnarray}
&=&\sum_i\sum_j\sum_k(D_i^{-\gamma}cos^2\phi_i(D_j^{-\gamma}D_k^{-\gamma}\sin^2\phi_k-D_j^{-\gamma} \sin\phi_jD_k^{-\gamma}\sin\phi_k)\nonumber\\ &\quad&-D_i^{-\gamma}\cos\phi_i\sin\phi_i(D_j^{-\gamma}\cos\phi_j\sin\phi_jD_k^{-\gamma}-D_j^{-\gamma}\sin\phi_jD_k^{-\gamma}\cos\phi_k)\nonumber\\ &\quad&+D_i^{-\gamma}\cos\phi_i(D_j^{-\gamma}\cos\phi_j\sin\phi_jD_k^{-\gamma}\sin\phi_k-D_j^{-\gamma}\sin^2\phi_j D_k^{-\gamma} \cos\phi_k))\nonumber\\
&=&\sum_i\sum_j\sum_k(D_i^{-\gamma}cos^2\phi_i(D_j^{-\gamma}D_k^{-\gamma}\sin\phi_k(\sin\phi_k-\sin \phi_j))\nonumber\\ &\quad&-D_i^{-\gamma}\cos\phi_i\sin\phi_i(D_j^{-\gamma}\sin\phi_jD_k^{-\gamma}(\cos\phi_j-\cos\phi_k))\nonumber\\ &\quad&+D_i^{-\gamma}\cos\phi_i(D_j^{-\gamma}D_k^{-\gamma}\sin\phi_j(\cos\phi_j\sin\phi_k -\sin\phi_j\cos\phi_k)))\nonumber\\
&=&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\cos\phi_i\sin\phi_k(\sin\phi_k-\sin\phi_j)\nonumber\\ &\quad&-\sin\phi_i\sin\phi_j(\cos\phi_j-\cos\phi_k)+\sin\phi_j\sin(\phi_k-\phi_j))  
\end{eqnarray}
This expression needs to be further simplified:
\begin{eqnarray}
&=&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_j(-\cos\phi_i\sin\phi_k-\sin\phi_i(\cos\phi_j-\cos\phi_k)\nonumber \\
&\quad&+\sin(\phi_k-\phi_j))+\cos\phi_i\sin^2\phi_k)\nonumber\\ &=&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)-\sin(\phi_j-\phi_k)\nonumber \\
&\quad&-\sin\phi_i\cos\phi_j)+\cos\phi_i\sin^2\phi_k)\nonumber \\
&\triangleq&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma} D_k^{-\gamma} \lambda(i,j,k)
\end{eqnarray}
A perfect symmetry between $i,j,k$ is expected, because the order of the sensors in the network has no impact on network performance. This expected symmetry, however, has yet to emerge. In order to explore this expression, the different combinations of $i,j,k$ are examined below:
\begin{equation}
\lambda(i,j,k)=\begin{cases}
0       & \quad i=j=k\\
0  & \quad i\neq (j=k)\\
\cos^2\phi_i(\sin^2\phi_i-\sin^2\phi_j)  & \quad j\neq (i=k)\\
\cos^2\phi_i(\sin^2\phi_k-\sin^2\phi_i)  & \quad k\neq (i=j)\\
\text{as writen}  & \quad i\neq j\neq k
\end{cases}
\end{equation}
Thus there is strong symmetry between $k$ and $j$ but without $i$. Moreover, because of the first two zeros, there is no contribution to the sum if $j=k$. Hence the large sum is split into three smaller ones:
\begin{eqnarray}
\det\left(\frac{J}{\eta}\right)&=&\sum_i\sum_{j\neq i}(D_i^{-\gamma} )^2 D_j^{-\gamma}\cos^2\phi_i(\sin^2\phi_i-\sin^2\phi_j)\nonumber\\
&\quad&-\sum_i\sum_{k\neq i}(D_i^{-\gamma})^2 D_k^{-\gamma}\cos^2\phi_i(\sin^2\phi_i-\sin^2\phi_k)\nonumber\\
&\quad&+\sum_i\sum_{j\neq i}\sum_{k\neq i,j}D_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)\nonumber\\
&\quad&-\sin(\phi_j-\phi_k)-\sin\phi_i\cos\phi_j)+\cos\phi_i\sin^2\phi_k)
\end{eqnarray}
The two first sums cancel each other out, so that we only have the last one. 
Let's examine the combination of swapped indices. In other words, $\lambda(i,j,k)+\lambda(i,k,j)$:
\begin{eqnarray}
\lambda(i,j,k)+\lambda(i,k,j)&=&\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)-\sin(\phi_j-\phi_k)-\sin\phi_i\cos\phi_j)\nonumber\\
&\quad&+\cos\phi_i\sin^2\phi_k)+\cos\phi_i(\sin\phi_k(\sin(\phi_i-\phi_j)-\sin(\phi_k-\phi_j)\nonumber\\
&\quad&-\sin\phi_i\cos\phi_k)+\cos\phi_i\sin^2\phi_j)\nonumber\\
&=&\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)-\sin(\phi_j-\phi_k)-\sin\phi_i\cos\phi_j)\nonumber\\
&\quad&+\cos\phi_i\sin^2\phi_k+\sin\phi_k(\sin(\phi_i-\phi_j)+\sin(\phi_j-\phi_k)\nonumber\\
&\quad&-\sin\phi_i\cos\phi_k)+\cos\phi_i\sin^2\phi_j)\nonumber\\
&=&\cos\phi_i[\cos\phi_i(\sin^2\phi_k+\sin^2\phi_j)+\sin(\phi_j-\phi_k)(\sin\phi_k-\sin\phi_j)\nonumber\\
&\quad&+\sin\phi_j(\sin\phi_i\cos\phi_k-\sin\phi_k\cos\phi_i-\sin\phi_i\cos\phi_j)\nonumber\\
&\quad&+\sin\phi_k(\sin\phi_i\cos\phi_j-\sin\phi_j\cos\phi_i-\sin\phi_i\cos\phi_k)]\nonumber\\
&=&\cos\phi_i[\cos\phi_i(\sin^2\phi_k+\sin^2\phi_j-2\sin\phi_j\sin\phi_k)\nonumber\\
&\quad&+\sin(\phi_j-\phi_k)(\sin\phi_k-\sin\phi_j)+\sin\phi_i(\sin\phi_j\cos\phi_k\nonumber\\
&\quad&-\sin\phi_j\cos\phi_j+\sin\phi_k\cos\phi_j-\sin\phi_k\cos\phi_k)]\nonumber\\
&=&\cos\phi_i(\sin\phi_k-\sin\phi_j)[\sin(\phi_j-\phi_k)+\cos\phi_i(\sin\phi_k-\sin\phi_j)\nonumber\\
&\quad&+\sin\phi_i(\cos\phi_j-\cos\phi_k)]\nonumber\\
&=&\cos\phi_i(\sin\phi_k-\sin\phi_j)[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)] \nonumber\\
&&	
\end{eqnarray}
Thus, it can be written as:
\begin{eqnarray}
&\det\left(\frac{\textbf{J}}{\eta}\right)&=\sum_i\sum_j\sum_{k<j}D_i^{-\gamma} D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_k-\sin\phi_j)\\ &\quad&\times[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]
\end{eqnarray}
for simplicity, simply define $\alpha_{ij}=\phi_i-\phi_j$. To conclude, 
\begin{equation}
\textit{CRB}=\frac{\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij})) }{\eta\sum_i\sum_j\sum_{k<j}D_i^{-\gamma} D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_k-\sin \phi_j)[\sin(\alpha_{jk})+\sin(\alpha_{ki})+\sin(\alpha_{ij})]}.
\end{equation}
and that for every $\lambda(i,j,k)$:
\begin{eqnarray}
\sum_i\sum_j\sum_k\lambda(i,j,k)&=&\sum_i\sum_{j<i}\sum_{k<j}\left(\lambda(i,j,k)+\lambda(i,k,j)+\lambda(j,i,k)+\lambda(j,k,i)\right.\nonumber\\
&\quad&\left.+\lambda(k,i,j)+\lambda(k,j,i)\right)\nonumber\\
&=&\frac{1}{6}\sum_i\sum_j\sum_k\left(\lambda(i,j,k)+\lambda(i,k,j)+\lambda(j,i,k)+\lambda(j,k,i)\right.\nonumber\\
&\quad&\left.+\lambda(k,i,j)+\lambda(k,j,i)\right)
\end{eqnarray}
In more explicit terms,
\begin{eqnarray}
&\quad&\lambda(i,j,k)+\lambda(i,k,j)+\lambda(j,i,k)+\lambda(j,k,i)+\lambda(k,i,j)+\lambda(k,j,i)\nonumber\\
&=&\cos\phi_i(\sin\phi_k-\sin\phi_j)[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]\nonumber\\
&\quad&+\cos\phi_j(\sin\phi_k-\sin\phi_i)[\sin(\phi_i-\phi_k)+\sin(\phi_k-\phi_j)+\sin(\phi_j-\phi_i)]\nonumber\\
&\quad&+\cos\phi_k(\sin\phi_i-\sin\phi_j)[\sin(\phi_j-\phi_i)+\sin(\phi_i-\phi_k)+\sin(\phi_k-\phi_j)]\nonumber\\
&=&[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]\left(\cos\phi_i(\sin\phi_k-\sin\phi_j)\right.\nonumber\\
&\quad&-\left.\cos\phi_j(\sin\phi_k-\sin\phi_i)-\cos\phi_k(\sin\phi_i-\sin\phi_j)\right)\nonumber\\
&=&[\sin(\alpha_{jk})+\sin(\alpha_{ki})+\sin(\alpha_{ij})]^2
\end{eqnarray}
Thus,
\begin{eqnarray}
\det\left(\frac{\textbf{J}}{\eta}\right)&=&\frac{1}{6}\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]^2\nonumber\\
&=&\frac{1}{6}\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}[\sin\alpha_{jk}+\sin\alpha_{ki}+\sin\alpha_{ij}]^2
\end{eqnarray}
Recall that 
\begin{equation}
\det(\textbf{J})=\eta^3\det\left(\frac{\textbf{J}}{\eta}\right)
\end{equation}
which concludes the explicit expression in (\ref{CRBlast}).
The transition to the second shape is quite easy, using the fact that by definition $\alpha_{ki}=-(\alpha_{ij}+\alpha_{jk})$:
\begin{eqnarray}
&&(\sin\alpha_{ij}+\sin\alpha_{jk}+\sin\alpha_{ki})^2=(\sin\alpha_{ij}+\sin\alpha_{jk}-\sin(\alpha_{ij}+\alpha_{jk}))^2\nonumber\\
&=&(\sin\alpha_{ij}+\sin\alpha_{jk}-\sin\alpha_{ij}\cos\alpha_{jk}-\sin\alpha_{jk}\cos\alpha_{ij})^2\nonumber\\
&=&\left(\sin\alpha_{ij}(1-\cos\alpha_{jk})+\sin\alpha_{jk}(1-\cos\alpha_{ij})\right)^2\nonumber\\
&=&(1-\cos\alpha_{jk})^2(1-\cos^2\alpha_{ij})+(1-\cos\alpha_{ij})^2(1-\cos^2\alpha_{jk})\nonumber\\
&\quad&+2(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})\sin\alpha_{ij}\sin\alpha_{jk}\nonumber\\
&=&(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})\left[(1-\cos\alpha_{ij})(1+\cos\alpha_{jk})\right.\nonumber\\
&\quad&\left.+(1-\cos\alpha_{jk})(1+\cos\alpha_{ij})+2\sin\alpha_{ij}\sin\alpha_{jk}\right]\nonumber\\
&=&2(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ij}\cos\alpha_{jk}+\sin\alpha_{ij}\sin\alpha_{jk})\nonumber\\
&=&2(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})
\end{eqnarray}
This expression is symmetric as expected, and reveals some of the features of the TDOA estimation method. For example, it requires at least three sensors that are not colinear in terms of the source. Otherwise, the denumerator equals zero and the estimation process is doomed to failure. Further insights and analyses are presented in the following sections \ref{chap:insight1UAA}, \ref{chap:insight2compModels}.

==> Chapters/CRB_TDOA_derivation_after_itsik.tex <==
	The following theorem gives a closed form expression for the localization CRB presented above. 
\begin{theorem}\label{CRBlast}
	The CRB on TDOA-based source-localization error is given by
	\begin{equation}
	\textrm{CRB}=\frac{3c^2\sum_i\sum_jA_i A_j \beta_{ij} }{4W_e\rho\sum_i\sum_j\sum_k A_i A_j A_k \beta_{ij}\beta_{jk}\beta_{ki}}
	\label{crbcos}
	\end{equation}
	where $\beta_{ij}=1-\cos(\phi_i-\phi_j)$ and $A_i=D_i^{-\gamma}$.
\end{theorem}
The resulting bound is much simpler to evaluate than the matrix form that presented in eq. (\ref{mtrx}). It also allows to draw insights and get a better understanding of the behavior in interesting scenarios (e.g., the effect of one sensor with very high SNR, the effect of two sensors at the same angle etc').


This expression is symmetric as expected, and reveals some of the features of the TDOA estimation method. For example, it requires at least three sensors that are not colinear in terms of the source. Otherwise, the denumerator equals zero and the estimation process is doomed to failure. Further insights and analyses are presented in the following sections \ref{chap:insight1UAA}, \ref{chap:insight2compModels}.

\begin{IEEEproof}
The matrix form of this bound is already known \cite{myref12}. After some adaptations to our model, and using the notation $\sum_i=\sum_{i=1}^M$, the FIM of estimating $\theta$ from the sensors is:
\begin{eqnarray}
\textbf{J}=\mu_1\overline{H}\Lambda\overline{H}^T=\mu_1
\begin{pmatrix}
\cos\phi_1&\cos\phi_2&\dots&\cos\phi_M\\
\sin\phi_1&\sin\phi_2&\dots&\sin\phi_M\\
-1&-1&\dots&-1\\
\end{pmatrix}
\Lambda
\begin{pmatrix}
\cos\phi_1&\sin\phi_1&-1\\
\cos\phi_2&\sin\phi_2&-1\\
\vdots&\vdots& \vdots\\
\cos\phi_M&\sin\phi_M&-1\\
\end{pmatrix}\nonumber\\
= 
\frac{4W_e\rho}{c^2}\begin{pmatrix}
\sum_iD_i^{-\gamma} \cos^2\phi_i&
\sum_iD_i^{-\gamma} \cos\phi_i\sin\phi_i& -\sum_iD_i^{-\gamma} \cos\phi_i\\
\sum_iD_i^{-\gamma} \cos\phi_i\sin\phi_i&
\sum_iD_i^{-\gamma} \sin^2\phi_i& -\sum_iD_i^{-\gamma} \sin\phi_i\\
-\sum_iD_i^{-\gamma} \cos\phi_i&
-\sum_iD_i^{-\gamma} \sin\phi_i&
\sum_iD_i^{-\gamma}
\end{pmatrix}.
\label{mtrx}
\end{eqnarray}
We are only interested in finding $[x,y]$ and $T_0$ is a nuisance parameter. Thus:
\begin{equation}
\textit{CRB}=\trace \{\textbf{J}^{-1}\}_{2\times 2}=(\textbf{J}^{-1})_{1,1}+(\textbf{J}^{-1})_{2,2}
\end{equation}
In order to get an element $i,j$ of $\textbf{J}^{-1}$, the matched minor $M_{i,j}$ must be calculated and divided by $\det (\textbf{J})$.\\
The first minor is given by
\begin{equation}
\frac{M_{1,1}}{\eta^2}=\left(\sum_i D_i^{-\gamma} \right)\left(\sum_iD_i^{-\gamma} \sin^2 \phi_i  \right)-\left(\sum_iD_i^{-\gamma} \sin \phi_i\right)^2
\end{equation}
where $\eta=4W_e\rho/c^2$. The second minor is identical, but with a cosine instead of a sinus. Thus, the combination yields:
\begin{eqnarray}
\frac{M_{1,1}+M_{2,2}}{\eta^2}&=&\left(\sum_iD_i^{-\gamma}\right)^2-\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(\sin\phi_i\sin\phi_j+\cos\phi_i\cos\phi_j)\nonumber\\
&=&\left(\sum_iD_i^{-\gamma}\right)^2-\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}\cos(\phi_i-\phi_j)\nonumber\\
&=&\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}\left(1-\cos(\phi_i-\phi_j) \right)   
\end{eqnarray}
Now, the determinant needs to be calculated:
\begin{eqnarray}
\det\left(\frac{\textbf{J}}{\eta}\right)&=&\left(\sum_iD_i^{-\gamma}\cos^2\phi_i\right)\left(\left(\sum_iD_i^{-\gamma}\right)\left(\sum_iD_i^{-\gamma}\sin^2\phi_i\right)-\left(\sum_iD_i^{-\gamma} \sin\phi_i\right)^2\right)\nonumber\\ &\quad&-\left(\sum_iD_i^{-\gamma}\cos\phi_i\sin\phi_i\right)\left(\left(\sum_iD_i^{-\gamma}\cos\phi_i\sin\phi_i\right)\left(\sum_iD_i^{-\gamma}\right)\right.\nonumber\\ &\quad&\left.-\left(\sum_iD_i^{-\gamma} \sin \phi_i\right)\left(\sum_iD_i^{-\gamma}\cos\phi_i\right)\right)+\left(\sum_iD_i^{-\gamma} \cos\phi_i\right)\nonumber\\ &\quad&\left(\left(\sum_iD_i^{-\gamma} \cos\phi_i\sin\phi_i\right)\left(\sum_iD_i^{-\gamma}\sin\phi_i\right)-\left(\sum_iD_i^{-\gamma} \sin^2 \phi_i\right)\right.\nonumber\\ &\quad&\left.\left(\sum_iD_i^{-\gamma}\cos\phi_i\right)\right)  
\end{eqnarray}
and after combining the separate sums into three large ones:
\begin{eqnarray}
\det\left(\frac{\textbf{J}}{\eta}\right)&=&\sum_i\sum_j\sum_k(D_i^{-\gamma}cos^2\phi_i(D_j^{-\gamma}D_k^{-\gamma}\sin^2\phi_k-D_j^{-\gamma} \sin\phi_jD_k^{-\gamma}\sin\phi_k)\nonumber\\ &\quad&-D_i^{-\gamma}\cos\phi_i\sin\phi_i(D_j^{-\gamma}\cos\phi_j\sin\phi_jD_k^{-\gamma}-D_j^{-\gamma}\sin\phi_jD_k^{-\gamma}\cos\phi_k)\nonumber\\ &\quad&+D_i^{-\gamma}\cos\phi_i(D_j^{-\gamma}\cos\phi_j\sin\phi_jD_k^{-\gamma}\sin\phi_k-D_j^{-\gamma}\sin^2\phi_j D_k^{-\gamma} \cos\phi_k))\nonumber\\
&=&\sum_i\sum_j\sum_k(D_i^{-\gamma}cos^2\phi_i(D_j^{-\gamma}D_k^{-\gamma}\sin\phi_k(\sin\phi_k-\sin \phi_j))\nonumber\\ &\quad&-D_i^{-\gamma}\cos\phi_i\sin\phi_i(D_j^{-\gamma}\sin\phi_jD_k^{-\gamma}(\cos\phi_j-\cos\phi_k))\nonumber\\ &\quad&+D_i^{-\gamma}\cos\phi_i(D_j^{-\gamma}D_k^{-\gamma}\sin\phi_j(\cos\phi_j\sin\phi_k -\sin\phi_j\cos\phi_k)))\nonumber\\
&=&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\cos\phi_i\sin\phi_k(\sin\phi_k-\sin\phi_j)\nonumber\\ &\quad&-\sin\phi_i\sin\phi_j(\cos\phi_j-\cos\phi_k)+\sin\phi_j\sin(\phi_k-\phi_j))  
\end{eqnarray}
This expression needs to be further simplified:
\begin{eqnarray}
\det\left(\frac{\textbf{J}}{\eta}\right)&=&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_j(-\cos\phi_i\sin\phi_k-\sin\phi_i(\cos\phi_j-\cos\phi_k)\nonumber \\
&\quad&+\sin(\phi_k-\phi_j))+\cos\phi_i\sin^2\phi_k)\nonumber\\ &=&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)-\sin(\phi_j-\phi_k)\nonumber \\
&\quad&-\sin\phi_i\cos\phi_j)+\cos\phi_i\sin^2\phi_k)\nonumber \\
&\triangleq&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma} D_k^{-\gamma} \lambda(i,j,k)
\end{eqnarray}
In order to explore this expression, the different combinations of $i,j,k$ are examined below:
\begin{equation}
\lambda(i,j,k)=\begin{cases}
0       & \quad i=j=k\\
0  & \quad i\neq (j=k)\\
\cos^2\phi_i(\sin^2\phi_i-\sin^2\phi_j)  & \quad j\neq (i=k)\\
\cos^2\phi_i(\sin^2\phi_k-\sin^2\phi_i)  & \quad k\neq (i=j)\\
\text{as writen}  & \quad i\neq j\neq k
\end{cases}
\end{equation}
Thus there is strong symmetry between $k$ and $j$ but without $i$. Moreover, because of the first two zeros, there is no contribution to the sum if $j=k$. Hence the large sum is split into three smaller ones:
\begin{eqnarray}
\det\left(\frac{J}{\eta}\right)&=&\sum_i\sum_{j\neq i}(D_i^{-\gamma} )^2 D_j^{-\gamma}\cos^2\phi_i(\sin^2\phi_i-\sin^2\phi_j)\nonumber\\
&\quad&-\sum_i\sum_{k\neq i}(D_i^{-\gamma})^2 D_k^{-\gamma}\cos^2\phi_i(\sin^2\phi_i-\sin^2\phi_k)\nonumber\\
&\quad&+\sum_i\sum_{j\neq i}\sum_{k\neq i,j}D_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)\nonumber\\
&\quad&-\sin(\phi_j-\phi_k)-\sin\phi_i\cos\phi_j)+\cos\phi_i\sin^2\phi_k)
\end{eqnarray}
The two first sums cancel each other out, so that we only have the last one. 
Let's examine the combination of swapped indices. In other words, $\lambda(i,j,k)+\lambda(i,k,j)$:
\begin{eqnarray}
\lambda(i,j,k)+\lambda(i,k,j)&=&\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)-\sin(\phi_j-\phi_k)-\sin\phi_i\cos\phi_j)\nonumber\\
&\quad&+\cos\phi_i\sin^2\phi_k)+\cos\phi_i(\sin\phi_k(\sin(\phi_i-\phi_j)-\sin(\phi_k-\phi_j)\nonumber\\
&\quad&-\sin\phi_i\cos\phi_k)+\cos\phi_i\sin^2\phi_j)\nonumber\\
&=&\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)-\sin(\phi_j-\phi_k)-\sin\phi_i\cos\phi_j)\nonumber\\
&\quad&+\cos\phi_i\sin^2\phi_k+\sin\phi_k(\sin(\phi_i-\phi_j)+\sin(\phi_j-\phi_k)\nonumber\\
&\quad&-\sin\phi_i\cos\phi_k)+\cos\phi_i\sin^2\phi_j)\nonumber\\
&=&\cos\phi_i[\cos\phi_i(\sin^2\phi_k+\sin^2\phi_j)+\sin(\phi_j-\phi_k)(\sin\phi_k-\sin\phi_j)\nonumber\\
&\quad&+\sin\phi_j(\sin\phi_i\cos\phi_k-\sin\phi_k\cos\phi_i-\sin\phi_i\cos\phi_j)\nonumber\\
&\quad&+\sin\phi_k(\sin\phi_i\cos\phi_j-\sin\phi_j\cos\phi_i-\sin\phi_i\cos\phi_k)]\nonumber\\
&=&\cos\phi_i[\cos\phi_i(\sin^2\phi_k+\sin^2\phi_j-2\sin\phi_j\sin\phi_k)\nonumber\\
&\quad&+\sin(\phi_j-\phi_k)(\sin\phi_k-\sin\phi_j)+\sin\phi_i(\sin\phi_j\cos\phi_k\nonumber\\
&\quad&-\sin\phi_j\cos\phi_j+\sin\phi_k\cos\phi_j-\sin\phi_k\cos\phi_k)]\nonumber\\
&=&\cos\phi_i(\sin\phi_k-\sin\phi_j)[\sin(\phi_j-\phi_k)+\cos\phi_i(\sin\phi_k-\sin\phi_j)\nonumber\\
&\quad&+\sin\phi_i(\cos\phi_j-\cos\phi_k)]\nonumber\\
&=&\cos\phi_i(\sin\phi_k-\sin\phi_j)[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)] \nonumber\\
&&	
\end{eqnarray}
Thus, it can be written as:
\begin{eqnarray}
&\det\left(\frac{\textbf{J}}{\eta}\right)&=\sum_i\sum_j\sum_{k<j}D_i^{-\gamma} D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_k-\sin\phi_j)\\ &\quad&\times[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]
\end{eqnarray}
for simplicity, simply define $\alpha_{ij}=\phi_i-\phi_j$. To conclude, 
\begin{equation}
\textit{CRB}=\frac{\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij})) }{\eta\sum_i\sum_j\sum_{k<j}D_i^{-\gamma} D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_k-\sin \phi_j)[\sin(\alpha_{jk})+\sin(\alpha_{ki})+\sin(\alpha_{ij})]}.
\end{equation}
and that for every $\lambda(i,j,k)$:
\begin{eqnarray}
\sum_i\sum_j\sum_k\lambda(i,j,k)&=&\sum_i\sum_{j<i}\sum_{k<j}\left(\lambda(i,j,k)+\lambda(i,k,j)+\lambda(j,i,k)+\lambda(j,k,i)\right.\nonumber\\
&\quad&\left.+\lambda(k,i,j)+\lambda(k,j,i)\right)\nonumber\\
&=&\frac{1}{6}\sum_i\sum_j\sum_k\left(\lambda(i,j,k)+\lambda(i,k,j)+\lambda(j,i,k)+\lambda(j,k,i)\right.\nonumber\\
&\quad&\left.+\lambda(k,i,j)+\lambda(k,j,i)\right)
\end{eqnarray}
In more explicit terms,
\begin{eqnarray}
&\quad&\lambda(i,j,k)+\lambda(i,k,j)+\lambda(j,i,k)+\lambda(j,k,i)+\lambda(k,i,j)+\lambda(k,j,i)\nonumber\\
&=&\cos\phi_i(\sin\phi_k-\sin\phi_j)[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]\nonumber\\
&\quad&+\cos\phi_j(\sin\phi_k-\sin\phi_i)[\sin(\phi_i-\phi_k)+\sin(\phi_k-\phi_j)+\sin(\phi_j-\phi_i)]\nonumber\\
&\quad&+\cos\phi_k(\sin\phi_i-\sin\phi_j)[\sin(\phi_j-\phi_i)+\sin(\phi_i-\phi_k)+\sin(\phi_k-\phi_j)]\nonumber\\
&=&[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]\left(\cos\phi_i(\sin\phi_k-\sin\phi_j)\right.\nonumber\\
&\quad&-\left.\cos\phi_j(\sin\phi_k-\sin\phi_i)-\cos\phi_k(\sin\phi_i-\sin\phi_j)\right)\nonumber\\
&=&[\sin(\alpha_{jk})+\sin(\alpha_{ki})+\sin(\alpha_{ij})]^2
\end{eqnarray}
Thus,
\begin{eqnarray}
\det\left(\frac{\textbf{J}}{\eta}\right)&=&\frac{1}{6}\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]^2\nonumber\\
&=&\frac{1}{6}\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}[\sin\alpha_{jk}+\sin\alpha_{ki}+\sin\alpha_{ij}]^2
\end{eqnarray}
Recall that 
\begin{equation}
\det(\textbf{J})=\eta^3\det\left(\frac{\textbf{J}}{\eta}\right)
\end{equation}
which concludes the explicit expression in (\ref{CRBlast}).
The transition to the second shape is quite easy, using the fact that by definition $\alpha_{ki}=-(\alpha_{ij}+\alpha_{jk})$:
\begin{eqnarray}
&&(\sin\alpha_{ij}+\sin\alpha_{jk}+\sin\alpha_{ki})^2=(\sin\alpha_{ij}+\sin\alpha_{jk}-\sin(\alpha_{ij}+\alpha_{jk}))^2\nonumber\\
&=&(\sin\alpha_{ij}+\sin\alpha_{jk}-\sin\alpha_{ij}\cos\alpha_{jk}-\sin\alpha_{jk}\cos\alpha_{ij})^2\nonumber\\
&=&\left(\sin\alpha_{ij}(1-\cos\alpha_{jk})+\sin\alpha_{jk}(1-\cos\alpha_{ij})\right)^2\nonumber\\
&=&(1-\cos\alpha_{jk})^2(1-\cos^2\alpha_{ij})+(1-\cos\alpha_{ij})^2(1-\cos^2\alpha_{jk})\nonumber\\
&\quad&+2(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})\sin\alpha_{ij}\sin\alpha_{jk}\nonumber\\
&=&(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})\left[(1-\cos\alpha_{ij})(1+\cos\alpha_{jk})\right.\nonumber\\
&\quad&\left.+(1-\cos\alpha_{jk})(1+\cos\alpha_{ij})+2\sin\alpha_{ij}\sin\alpha_{jk}\right]\nonumber\\
&=&2(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ij}\cos\alpha_{jk}+\sin\alpha_{ij}\sin\alpha_{jk})\nonumber\\
&=&2(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})
\end{eqnarray}
\end{IEEEproof}



==> Chapters/CRB_TDOA_derivation_after_itsik_yair.tex <==
	The following theorem provides a closed form expression for the localization CRB of the problem presented in Chap. \ref{Sec:PorblemFormulation}. 
\begin{theorem}\label{CRBlast}
	Given the observations in (\ref{sig_shape}), the CRB on TDOA-based source-localization error is given by
	\begin{equation}
	\textrm{CRB}=\frac{3c^2\sum_i\sum_jA_i A_j \beta_{ij} }{4W_e\rho\sum_i\sum_j\sum_k A_i A_j A_k \beta_{ij}\beta_{jk}\beta_{ki}}
	\label{crbcos}
	\end{equation}
	where $\beta_{ij}=1-\cos(\phi_i-\phi_j)$ and $A_i=D_i^{-\gamma}$.
\end{theorem}
The resulting bound is much simpler to evaluate than the matrix form that presented in eq. (\ref{mtrx}). It also allows to draw insights and get a better understanding of the behavior in interesting scenarios (e.g., the effect of one sensor with very high SNR, the effect of two sensors at the same angle etc').


This expression is symmetric as expected, and reveals some of the features of the TDOA estimation method. For example, it requires at least three sensors that are not colinear in terms of the source. Otherwise, the denumerator is equal to zero and the estimation process is doomed to failure. Further insights and analyses are presented in the following sections \ref{chap:insight1UAA}, \ref{chap:insight2compModels}.

\begin{IEEEproof}
The matrix form of this bound is already known \cite{myref12}. After some adaptations to our model, and using the notation $\sum_i=\sum_{i=1}^M$, the FIM of estimating $\theta$ from the sensors is:
\begin{eqnarray}
\textbf{J}=\mu_1\overline{H}\Lambda\overline{H}^T=\mu_1
\begin{pmatrix}
\cos\phi_1&\cos\phi_2&\dots&\cos\phi_M\\
\sin\phi_1&\sin\phi_2&\dots&\sin\phi_M\\
-1&-1&\dots&-1\\
\end{pmatrix}
\Lambda
\begin{pmatrix}
\cos\phi_1&\sin\phi_1&-1\\
\cos\phi_2&\sin\phi_2&-1\\
\vdots&\vdots& \vdots\\
\cos\phi_M&\sin\phi_M&-1\\
\end{pmatrix}\nonumber\\
= 
\frac{4W_e\rho}{c^2}\begin{pmatrix}
\sum_iD_i^{-\gamma} \cos^2\phi_i&
\sum_iD_i^{-\gamma} \cos\phi_i\sin\phi_i& -\sum_iD_i^{-\gamma} \cos\phi_i\\
\sum_iD_i^{-\gamma} \cos\phi_i\sin\phi_i&
\sum_iD_i^{-\gamma} \sin^2\phi_i& -\sum_iD_i^{-\gamma} \sin\phi_i\\
-\sum_iD_i^{-\gamma} \cos\phi_i&
-\sum_iD_i^{-\gamma} \sin\phi_i&
\sum_iD_i^{-\gamma}
\end{pmatrix}.
\label{mtrx}
\end{eqnarray}
We are only interested in finding $[x,y]$ and $T_0$ is a nuisance parameter. Thus:
\begin{equation}
\textit{CRB}=\trace \{\textbf{J}^{-1}\}_{2\times 2}=(\textbf{J}^{-1})_{1,1}+(\textbf{J}^{-1})_{2,2}
\end{equation}
In order to get an element $i,j$ of $\textbf{J}^{-1}$, the matched minor $M_{i,j}$ must be calculated and divided by $\det (\textbf{J})$.\\
The first minor is given by
\begin{equation}
\frac{M_{1,1}}{\eta^2}=\left(\sum_i D_i^{-\gamma} \right)\left(\sum_iD_i^{-\gamma} \sin^2 \phi_i  \right)-\left(\sum_iD_i^{-\gamma} \sin \phi_i\right)^2
\end{equation}
where $\eta=4W_e\rho/c^2$. The second minor is identical, but with a cosine instead of a sinus. Thus, the combination yields:
\begin{eqnarray}
\frac{M_{1,1}+M_{2,2}}{\eta^2}&=&\left(\sum_iD_i^{-\gamma}\right)^2-\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(\sin\phi_i\sin\phi_j+\cos\phi_i\cos\phi_j)\nonumber\\
&=&\left(\sum_iD_i^{-\gamma}\right)^2-\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}\cos(\phi_i-\phi_j)\nonumber\\
&=&\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}\left(1-\cos(\phi_i-\phi_j) \right)   
\end{eqnarray}
Now, the determinant needs to be calculated:
\begin{eqnarray}
\det\left(\frac{\textbf{J}}{\eta}\right)&=&\left(\sum_iD_i^{-\gamma}\cos^2\phi_i\right)\left(\left(\sum_iD_i^{-\gamma}\right)\left(\sum_iD_i^{-\gamma}\sin^2\phi_i\right)-\left(\sum_iD_i^{-\gamma} \sin\phi_i\right)^2\right)\nonumber\\ &\quad&-\left(\sum_iD_i^{-\gamma}\cos\phi_i\sin\phi_i\right)\left(\left(\sum_iD_i^{-\gamma}\cos\phi_i\sin\phi_i\right)\left(\sum_iD_i^{-\gamma}\right)\right.\nonumber\\ &\quad&\left.-\left(\sum_iD_i^{-\gamma} \sin \phi_i\right)\left(\sum_iD_i^{-\gamma}\cos\phi_i\right)\right)+\left(\sum_iD_i^{-\gamma} \cos\phi_i\right)\nonumber\\ &\quad&\left(\left(\sum_iD_i^{-\gamma} \cos\phi_i\sin\phi_i\right)\left(\sum_iD_i^{-\gamma}\sin\phi_i\right)-\left(\sum_iD_i^{-\gamma} \sin^2 \phi_i\right)\right.\nonumber\\ &\quad&\left.\left(\sum_iD_i^{-\gamma}\cos\phi_i\right)\right)  
\end{eqnarray}
and after combining the separate sums into three large ones:
\begin{eqnarray}
\det\left(\frac{\textbf{J}}{\eta}\right)&=&\sum_i\sum_j\sum_k(D_i^{-\gamma}cos^2\phi_i(D_j^{-\gamma}D_k^{-\gamma}\sin^2\phi_k-D_j^{-\gamma} \sin\phi_jD_k^{-\gamma}\sin\phi_k)\nonumber\\ &\quad&-D_i^{-\gamma}\cos\phi_i\sin\phi_i(D_j^{-\gamma}\cos\phi_j\sin\phi_jD_k^{-\gamma}-D_j^{-\gamma}\sin\phi_jD_k^{-\gamma}\cos\phi_k)\nonumber\\ &\quad&+D_i^{-\gamma}\cos\phi_i(D_j^{-\gamma}\cos\phi_j\sin\phi_jD_k^{-\gamma}\sin\phi_k-D_j^{-\gamma}\sin^2\phi_j D_k^{-\gamma} \cos\phi_k))\nonumber\\
&=&\sum_i\sum_j\sum_k(D_i^{-\gamma}cos^2\phi_i(D_j^{-\gamma}D_k^{-\gamma}\sin\phi_k(\sin\phi_k-\sin \phi_j))\nonumber\\ &\quad&-D_i^{-\gamma}\cos\phi_i\sin\phi_i(D_j^{-\gamma}\sin\phi_jD_k^{-\gamma}(\cos\phi_j-\cos\phi_k))\nonumber\\ &\quad&+D_i^{-\gamma}\cos\phi_i(D_j^{-\gamma}D_k^{-\gamma}\sin\phi_j(\cos\phi_j\sin\phi_k -\sin\phi_j\cos\phi_k)))\nonumber\\
&=&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\cos\phi_i\sin\phi_k(\sin\phi_k-\sin\phi_j)\nonumber\\ &\quad&-\sin\phi_i\sin\phi_j(\cos\phi_j-\cos\phi_k)+\sin\phi_j\sin(\phi_k-\phi_j))  
\end{eqnarray}
This expression needs to be further simplified:
\begin{eqnarray}
\det\left(\frac{\textbf{J}}{\eta}\right)&=&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_j(-\cos\phi_i\sin\phi_k-\sin\phi_i(\cos\phi_j-\cos\phi_k)\nonumber \\
&\quad&+\sin(\phi_k-\phi_j))+\cos\phi_i\sin^2\phi_k)\nonumber\\ &=&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)-\sin(\phi_j-\phi_k)\nonumber \\
&\quad&-\sin\phi_i\cos\phi_j)+\cos\phi_i\sin^2\phi_k)\nonumber \\
&\triangleq&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma} D_k^{-\gamma} \lambda(i,j,k)
\end{eqnarray}
In order to explore this expression, the different combinations of $i,j,k$ are examined below:
\begin{equation}
\lambda(i,j,k)=\begin{cases}
0       & \quad i=j=k\\
0  & \quad i\neq (j=k)\\
\cos^2\phi_i(\sin^2\phi_i-\sin^2\phi_j)  & \quad j\neq (i=k)\\
\cos^2\phi_i(\sin^2\phi_k-\sin^2\phi_i)  & \quad k\neq (i=j)\\
\text{as writen}  & \quad i\neq j\neq k
\end{cases}
\end{equation}
Thus there is strong symmetry between $k$ and $j$ but without $i$. Moreover, because of the first two zeros, there is no contribution to the sum if $j=k$. Hence the large sum is split into three smaller ones:
\begin{eqnarray}
\det\left(\frac{J}{\eta}\right)&=&\sum_i\sum_{j\neq i}(D_i^{-\gamma} )^2 D_j^{-\gamma}\cos^2\phi_i(\sin^2\phi_i-\sin^2\phi_j)\nonumber\\
&\quad&-\sum_i\sum_{k\neq i}(D_i^{-\gamma})^2 D_k^{-\gamma}\cos^2\phi_i(\sin^2\phi_i-\sin^2\phi_k)\nonumber\\
&\quad&+\sum_i\sum_{j\neq i}\sum_{k\neq i,j}D_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)\nonumber\\
&\quad&-\sin(\phi_j-\phi_k)-\sin\phi_i\cos\phi_j)+\cos\phi_i\sin^2\phi_k)
\end{eqnarray}
The two first sums cancel each other out, so that we only have the last one. 
Let's examine the combination of swapped indices. In other words, $\lambda(i,j,k)+\lambda(i,k,j)$:
\begin{eqnarray}
\lambda(i,j,k)+\lambda(i,k,j)&=&\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)-\sin(\phi_j-\phi_k)-\sin\phi_i\cos\phi_j)\nonumber\\
&\quad&+\cos\phi_i\sin^2\phi_k)+\cos\phi_i(\sin\phi_k(\sin(\phi_i-\phi_j)-\sin(\phi_k-\phi_j)\nonumber\\
&\quad&-\sin\phi_i\cos\phi_k)+\cos\phi_i\sin^2\phi_j)\nonumber\\
&=&\cos\phi_i(\sin\phi_j(\sin(\phi_i-\phi_k)-\sin(\phi_j-\phi_k)-\sin\phi_i\cos\phi_j)\nonumber\\
&\quad&+\cos\phi_i\sin^2\phi_k+\sin\phi_k(\sin(\phi_i-\phi_j)+\sin(\phi_j-\phi_k)\nonumber\\
&\quad&-\sin\phi_i\cos\phi_k)+\cos\phi_i\sin^2\phi_j)\nonumber\\
&=&\cos\phi_i[\cos\phi_i(\sin^2\phi_k+\sin^2\phi_j)+\sin(\phi_j-\phi_k)(\sin\phi_k-\sin\phi_j)\nonumber\\
&\quad&+\sin\phi_j(\sin\phi_i\cos\phi_k-\sin\phi_k\cos\phi_i-\sin\phi_i\cos\phi_j)\nonumber\\
&\quad&+\sin\phi_k(\sin\phi_i\cos\phi_j-\sin\phi_j\cos\phi_i-\sin\phi_i\cos\phi_k)]\nonumber\\
&=&\cos\phi_i[\cos\phi_i(\sin^2\phi_k+\sin^2\phi_j-2\sin\phi_j\sin\phi_k)\nonumber\\
&\quad&+\sin(\phi_j-\phi_k)(\sin\phi_k-\sin\phi_j)+\sin\phi_i(\sin\phi_j\cos\phi_k\nonumber\\
&\quad&-\sin\phi_j\cos\phi_j+\sin\phi_k\cos\phi_j-\sin\phi_k\cos\phi_k)]\nonumber\\
&=&\cos\phi_i(\sin\phi_k-\sin\phi_j)[\sin(\phi_j-\phi_k)+\cos\phi_i(\sin\phi_k-\sin\phi_j)\nonumber\\
&\quad&+\sin\phi_i(\cos\phi_j-\cos\phi_k)]\nonumber\\
&=&\cos\phi_i(\sin\phi_k-\sin\phi_j)[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)] \nonumber\\
&&	
\end{eqnarray}
Thus, it can be written as:
\begin{eqnarray}
&\det\left(\frac{\textbf{J}}{\eta}\right)&=\sum_i\sum_j\sum_{k<j}D_i^{-\gamma} D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_k-\sin\phi_j)\\ &\quad&\times[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]
\end{eqnarray}
for simplicity, simply define $\alpha_{ij}=\phi_i-\phi_j$. To conclude, 
\begin{equation}
\textit{CRB}=\frac{\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij})) }{\eta\sum_i\sum_j\sum_{k<j}D_i^{-\gamma} D_j^{-\gamma}D_k^{-\gamma}\cos\phi_i(\sin\phi_k-\sin \phi_j)[\sin(\alpha_{jk})+\sin(\alpha_{ki})+\sin(\alpha_{ij})]}.
\end{equation}
and that for every $\lambda(i,j,k)$:
\begin{eqnarray}
\sum_i\sum_j\sum_k\lambda(i,j,k)&=&\sum_i\sum_{j<i}\sum_{k<j}\left(\lambda(i,j,k)+\lambda(i,k,j)+\lambda(j,i,k)+\lambda(j,k,i)\right.\nonumber\\
&\quad&\left.+\lambda(k,i,j)+\lambda(k,j,i)\right)\nonumber\\
&=&\frac{1}{6}\sum_i\sum_j\sum_k\left(\lambda(i,j,k)+\lambda(i,k,j)+\lambda(j,i,k)+\lambda(j,k,i)\right.\nonumber\\
&\quad&\left.+\lambda(k,i,j)+\lambda(k,j,i)\right)
\end{eqnarray}
In more explicit terms,
\begin{eqnarray}
&\quad&\lambda(i,j,k)+\lambda(i,k,j)+\lambda(j,i,k)+\lambda(j,k,i)+\lambda(k,i,j)+\lambda(k,j,i)\nonumber\\
&=&\cos\phi_i(\sin\phi_k-\sin\phi_j)[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]\nonumber\\
&\quad&+\cos\phi_j(\sin\phi_k-\sin\phi_i)[\sin(\phi_i-\phi_k)+\sin(\phi_k-\phi_j)+\sin(\phi_j-\phi_i)]\nonumber\\
&\quad&+\cos\phi_k(\sin\phi_i-\sin\phi_j)[\sin(\phi_j-\phi_i)+\sin(\phi_i-\phi_k)+\sin(\phi_k-\phi_j)]\nonumber\\
&=&[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]\left(\cos\phi_i(\sin\phi_k-\sin\phi_j)\right.\nonumber\\
&\quad&-\left.\cos\phi_j(\sin\phi_k-\sin\phi_i)-\cos\phi_k(\sin\phi_i-\sin\phi_j)\right)\nonumber\\
&=&[\sin(\alpha_{jk})+\sin(\alpha_{ki})+\sin(\alpha_{ij})]^2
\end{eqnarray}
Thus,
\begin{eqnarray}
\det\left(\frac{\textbf{J}}{\eta}\right)&=&\frac{1}{6}\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}[\sin(\phi_j-\phi_k)+\sin(\phi_k-\phi_i)+\sin(\phi_i-\phi_j)]^2\nonumber\\
&=&\frac{1}{6}\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}[\sin\alpha_{jk}+\sin\alpha_{ki}+\sin\alpha_{ij}]^2
\end{eqnarray}
Recall that 
\begin{equation}
\det(\textbf{J})=\eta^3\det\left(\frac{\textbf{J}}{\eta}\right)
\end{equation}
which concludes the explicit expression in (\ref{CRBlast}).
The transition to the second shape is quite easy, using the fact that by definition $\alpha_{ki}=-(\alpha_{ij}+\alpha_{jk})$:
\begin{eqnarray}
&&(\sin\alpha_{ij}+\sin\alpha_{jk}+\sin\alpha_{ki})^2=(\sin\alpha_{ij}+\sin\alpha_{jk}-\sin(\alpha_{ij}+\alpha_{jk}))^2\nonumber\\
&=&(\sin\alpha_{ij}+\sin\alpha_{jk}-\sin\alpha_{ij}\cos\alpha_{jk}-\sin\alpha_{jk}\cos\alpha_{ij})^2\nonumber\\
&=&\left(\sin\alpha_{ij}(1-\cos\alpha_{jk})+\sin\alpha_{jk}(1-\cos\alpha_{ij})\right)^2\nonumber\\
&=&(1-\cos\alpha_{jk})^2(1-\cos^2\alpha_{ij})+(1-\cos\alpha_{ij})^2(1-\cos^2\alpha_{jk})\nonumber\\
&\quad&+2(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})\sin\alpha_{ij}\sin\alpha_{jk}\nonumber\\
&=&(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})\left[(1-\cos\alpha_{ij})(1+\cos\alpha_{jk})\right.\nonumber\\
&\quad&\left.+(1-\cos\alpha_{jk})(1+\cos\alpha_{ij})+2\sin\alpha_{ij}\sin\alpha_{jk}\right]\nonumber\\
&=&2(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ij}\cos\alpha_{jk}+\sin\alpha_{ij}\sin\alpha_{jk})\nonumber\\
&=&2(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})
\end{eqnarray}
\end{IEEEproof}



==> Chapters/GNSSWIKI.tex <==
%\documentclass[onecolumn,draftcls,12pt]{IEEEtran}
%
%\begin{document}

A global navigation satellite system (GNSS) is satellite navigation system with global coverage, which is a system that provides autonomous geo-spatial positioning using satellites. It allows small electronic receivers to determine their location to high precision\footnote{The precision can arrive to a few centimeters to metres, and can be concluded from the CRB.} using time signals transmitted along a line of sight by radio waves from satellites. The system can be used for providing position, navigation or for tracking the position of something fitted with a receiver. The signals also allow the electronic receiver to calculate the current local time to high precision, which allows time synchronisation. GNSS operates independently of any telephonic or internet reception, though these technologies can enhance the usefulness of the positioning information generated.
Nowadays, there are several GNSSs that belong to different nations all over the world, such as Russia, China and the United States. The different systems differ from each other in many properties, such as the radius of orbit.

\subsubsection{History and Theory}
Ground based radio navigation is decades old. The original systems used terrestrial longwave radio transmitters which broadcast a radio pulse from a known "master" location, followed by a pulse repeated from a number of "slave" stations. The delay between the reception of the master signal and the slave signals allowed the receiver to deduce the distance to each of the slaves, providing a fix.\\
Another system was based on the Doppler effect: the satellites travelled on well-known paths and broadcast their signals on a well-known radio frequency. The received frequency will differ slightly from the broadcast frequency because of the movement of the satellite with respect to the receiver. By monitoring this frequency shift over a short time interval, the receiver can determine its location to one side or the other of the satellite, and several such measurements combined with a precise knowledge of the satellite's orbit can fix a particular position. Satellite orbital position errors are caused by radio-wave refraction, gravity field changes (as the Earth's gravitational field is not uniform), and other phenomena. Using real-time data and recursive estimation, the systematic and residual errors were narrowed down to accuracy sufficient for navigation.\\

Modern systems are more direct. The satellite broadcasts a signal that contains orbital data (from which the position of the satellite can be calculated) and the precise time the signal was transmitted. Orbital data include a rough almanac for all satellites to aid in finding them, and a precise ephemeris for this satellite. The orbital ephemeris is transmitted in a data message that is superimposed on a code that serves as a timing reference. The satellite uses an atomic clock to maintain synchronization of all the satellites in the constellation. The receiver compares the time of broadcast encoded in the transmission of three or four different satellites, measuring the time-of-flight to each satellite, and actually implement time-difference-of-arrival estimation. Several such measurements can be made at the same time to different satellites, allowing a continual fix to be generated in real time using an adapted version of trilateration.However, in the case of fast-moving receivers, the position of the signal moves as signals are received from several satellites.\\
 Satellite navigation receivers reduce errors by using combinations of signals from multiple satellites and multiple correlators, and then using techniques such as Kalman filtering to combine the noisy, partial, and constantly changing data into a single estimate for position, time, and velocity.

\subsubsection{Applications}
The original motivation for satellite navigation was for military applications. Satellite navigation allows precision in the delivery of weapons to targets, greatly increasing their lethality whilst reducing inadvertent casualties from mis-directed weapons. Satellite navigation also allows forces to be directed and to locate themselves more easily.
\\
Now a GNSS is used to determine users location and the location of other objects at any given moment. The range of application of the satellite in the future is enormous, including both the public and private sectors across numerous market segments such as science, transport, agriculture etc.\cite{GNSSAPPmisc}
\nocite{nicolini2018investigation}
%\begin{small}
%	\bibliography{BibSatellitesHodaya}
%	\bibliographystyle{ieeetr}
%\end{small}
%\end{document}


==> Chapters/abbreviations.tex <==
\begin{acronym}
	\acro{SNR}{signal to noise ratio}
	\acro{CRB}{Cram\'{e}r-Rao Bound}
	\acro{FIM}{Fisher information Matrix}
	\acro{TOA}{time of arrival}
	\acro{RSS}{received signal strength}
	\acro{UAA}{uniform angular array}
	\acro{ML}{maximum likelihood}
	\acro{MLE}{maximum likelihood estimator}
	\acro{MSE}{mean square error}
	\acro{TDOA}{time difference of arrival}
	\acro{PDF}{probability density function}
	\acro{WLOG}{without loss of generality}
	\acro{AWGN}{additive white Gaussian noise}
	\acro{GNSS}{global navigation satellite system}
	
\end{acronym}

==> Chapters/background.tex <==
In this section, the theoretical background used for the thesis is presented. First of all, the different estimation methods are explained in detail. Then, some concepts derived from performance evaluation theory are presented, and the estimator is described.

\subsection{RSS}\label{chap:background_rss}
The assumption behind received-signal-strength (RSS) localization is that the most relevant information for source location estimation is included in the signal's amplitude. In other words, the strongest effect of distancing from the source is manifested by the amplitude attenuation. An optional mathematical formulation for rss estimation is found in \cite{fujiistudy}:
\begin{equation}
r=n\alpha d^{-\beta}
\end{equation}
where $r$ is the received power signal, $\alpha$ is a constant value corresponding to the transmitted signal power, $n$ is a scaling factor depending on the wireless system, $d$ is the distance from the source that needs to be estimated, and $\beta$ is the pathloss exponent. It is assumed that the RSS is constant, but $n$ is a random variable
in a typical wireless environment. The variation of $n$ involves
that of the RSS $r$. As a result, $r$ is also a random variable controlled by $n$, where $n$ is a sample of exponential random variable $N$. In other words, the Probability Density Function (PDF) of the random
variable is given by
\begin{equation}
p_N(n)=\exp (-n).
\end{equation}
As a consequence, and denoting $r$ as a sample of a random variable $R$, one can easily find the PDF of $R$:
\begin{equation}
p_R(r)=\frac{1}{\alpha d^{-\beta}}\exp \left(-\frac{r}{\alpha d^{-\beta}}\right).
\end{equation}
After finding the distance from a sensor to the source, one can define a circle around the sensor which is a collection of all the alternative source locations as a function of the specific sensor's measurements. In an ideal situation, the circles of all the sensors should intersect at one point, which is the real source location. However, because of noise, the circles are almost never intersect at one point, and the estimator needs to deal with ambiguity in estimating the source location. The solution is usually Maxiumm-Likelihood estimation (MLE), which is discussed later.\\
RSS assumption exists only for short distances. For long distances, the amplitude attenuation is hard to measure accurately and TOA estimation will probably yield better results.  % TOA

\subsection{TOA}
In time-of-arrival (TOA) localization, the sensors extract timing information from the received signals, whereas we assume that the exact transmission time is known to all sensors\footnote{In some publications, the term TOA is also used when the transmission time is not known in advance, but is estimated during the localization process. To clarify our notation, we use the term TOA if the transmission time is known in advance, and TDOA when this time is not known (regardless of the estimation algorithm).}. Accordingly, the transmission time is a known constant and can be chosen as zero without loss of generality (WLOG). For instance, the received signal's mathematical formulation can be
\begin{equation}
r(t)=s\left(t-\frac{d}{c}\right)+n(t)
\end{equation}
where $s(t)$ is the transmitted signal, $d$ is the distance from the source that should be estimated, $c$ is the signal's expansion speed, and $n(t)$ is additive white Gaussian noise (AWGN), so the signal's PDF is
\begin{equation}
p_R(r(t))=\frac{1}{\sqrt{2\pi \sigma_n^2}}\exp\left(-\frac{(r(t)-s(t-\frac{d}{c}))^2}{2\sigma_n^2}\right)
\end{equation}
This method has been explored extensively in the literature, even though its main assumption is hard to satisfy \cite{myref11,myref13}.  % TDOA

\subsection{TDOA}
In time-difference-of-arrival (TDOA), in contrast to TOA, the transmission time is unknown. Thus, such systems are much simpler to implement than TOA. Some TDOA models assume that all signals received by each sensor have the same signal to noise ratio (SNR) \cite{geofdtd,TDFD,myref2,accuracyanalysis}, while others are more general and allow different SNR at different sensors \cite{HybDis,generalMeasurements,myref12,myref13}. An optional mathematical formulation for the received signal in TDOA estimation is:
\begin{equation}
r(t)=s(t-\tau-T_0)+v(t)\qquad t\in\mathbb{R}_+
\end{equation}
where $s(t)$ is the known transmitted signal, $\tau = D/c$ is the time delay, $c$ is the speed of light,
\begin{equation}
D=\sqrt{(x_{s}-x)^2+(y_s-y)^2}
\end{equation}
is the distance between the source and the sensor, $v(t)$ is a white Gaussian noise with spectral density $N_0/2$, and $T_0$ is the transmission time which is assumed to be unknown. Thus, $r(t)$'s PDF can be trivially concluded from the case of TOA. Even though TOA and TDOA look very similar and close, there is at least one significant difference between them. In TOA the parameter vector for estimation only contains the wanted information; i.e., the source location. In TDOA, on the contrary, $T_0$ is added as a nuisance parameter and one dimension is added to the search process. As a result, one disadvantage of TDOA-based localization methods is computational complexity. It is therefore important to develop bounds on the estimation error. As noted above, some lower bounds for different signal models can be found in the literature, but only in matrix form. In other words, there is no explicit term for TDOA estimation performance evaluation. According to its computational complexity on the one hand, and its practical importance on the other, a short and intuitive expression for performance evaluation could considerably improve the human understanding in this method and as a result enhance its potential performance. %AOA

\subsection{AOA}
In contrast to the previous estimation methods described above, which are based on distance estimation for source localization, the angle-of-arrival (AOA) method estimates the angle between the source and the horizon to re-evaluate the source location. For angle estimation to be possible, directional sensors are needed, such as phased antenna arrays, mechanically steerable antennas, or
multiple antennas\cite{jais2015review}. The mathematical formulation of the received signal obviously depends on the antennas array's specific shape. As an example, when the antennas array is organized as a line with a constant space between each antenna, the formulation can be written as follows\cite{mohanna2013optimization}:
\begin{equation}
\textbf{r}(k)=\textbf{a}(\theta)s(k)+\textbf{n}(k)
\end{equation}
where $k$ is a discrete time index, $\textbf{r}$ is the received signal, $s$ is the transmitted signal, $\textbf{n}$ is AWGN and $\textbf{a}$ is the steering vector, which contains the total influence of $\theta$ on $\textbf{r}$ and is explicitly folmulated as follows:
\begin{equation}
\textbf{a}(\theta)=[1 e^{j\beta d\sin(\theta)} e^{j2\beta d\sin(\theta)} ... e^{j(M-1)\beta d\sin(\theta)}]^T
\end{equation}
or in other words:
\begin{equation}
\textbf{a}_m(\theta)=\exp(j(m-1)\beta d\sin(\theta))
\end{equation}
where $\beta=2\pi/\lambda$ is the incident wave number, $d$ is inter-element spacing, and $\theta$ is the wanted unknown angle of arrival. The received signal is a vector since the analysis is performed simultaneously for all the antennas in the array and each element in the vector belongs to a different antenna.\\
The noise model is the same as in TOA and TDOA so that the PDF can simply be concluded.

\subsection{FIM and CRB}
One of the most frequently used measures in statistical signal processing is the Fisher Information Matrix (FIM). In general, the Fisher Information is a way of measuring the amount of information that an observable random variable $X$ carries about an unknown parameter $\theta$ upon which the probability of $X$ depends. When $\theta$ is a scalar, the Fisher Information is defined as follows:
\begin{equation}
I(\theta)={\mathbb E}\left[\left.\left({\frac {\partial }{\partial \theta }}\log f(X;\theta )\right)^{2}\right|\theta \right].
\end{equation}
When the regularity condition 
\begin{equation}
{\mathbb E} \left[\frac{\partial }{\partial \theta }\log f(X;\theta )|\theta \right]=0
\end{equation}
exists and $\log f(x;\theta)$ is twice differentiable with respect to $\theta$, it can be shown that 
\begin{equation}
{\mathbb E} \left[\left(\frac{\partial }{\partial \theta }\log f(X;\theta )\right)^{2}|\theta \right]=-{\mathbb E} \left[{\frac {\partial^2 }{\partial \theta^2 }}\log f(X;\theta )|\theta \right].
\end{equation}
The Fisher Information may be seen as the curvature of the support curve (the graph of the log-likelihood). Near the maximum likelihood estimate, low Fisher Information therefore indicates that the maximum appears "blunt"; that is, the maximum is shallow and there are many nearby values with a similar log-likelihood. Conversely, high Fisher Information indicates that the maximum is sharp. \\
When $\theta$ is a vector of $N$ parameters, the Fisher Information takes an $N\times N$ matrix form, and its $i,j$ element is defined as follows:
\begin{equation}
\bigl [I(\theta ){\bigr ]}_{i,j}={\mathbb E} \left[\left({\frac {\partial }{\partial \theta _{i}}}\log f(X;\theta )\right)\left({\frac {\partial }{\partial \theta _{j}}}\log f(X;\theta )\right)|\theta \right]
\end{equation}
or as in the previous case,
\begin{equation}
\bigl [I(\theta )\bigr ]_{i,j}=-{\mathbb E} \left[{\frac {\partial ^{2}}{\partial \theta _{i}\partial \theta _{j}}}\log f(X;\theta )|\theta \right].
\end{equation}
The FIM has several interpretations in different fields. In machine learning, for example, it is used in elastic weight consolidation\cite{kirkpatrick2017overcoming}, which reduces catastrophic forgetting in artificial neural networks. Another use of Fisher Information is in computational neuroscience, where it is used to find bounds on the accuracy of neural codes.\\
In the estimation theory context, FIM is interpreted as the inverse of the lower bound on the estimator variance, which is known as the Cram\'{e}r-Rao bound (CRB). The CRB has slightly different versions for biased and unbiased estimators, and in this thesis the unbiased estimator's version is discussed. In mathematical terms, if $\widehat{\theta}$ is any estimator of the unknown parameter $\theta$, then
\begin{equation}
VAR(\widehat{\theta})\geq I(\theta )^{-1}.
\end{equation}
When $\theta$ is a scalar, the meaning of $I(\theta)$ is clear. However, if $\theta$ is a vector, $I(\theta)$ is a matrix whose elements' meaning is not initially clear. To clarify this point, the elements need to be seperated into two different groups- on the diagonal, and not on the diagonal. The elements in the diagonal have a similar meaning as in the scalar case:
\begin{equation}
VAR(\widehat{\theta}_i)\geq [I(\theta )^{-1}]_{ii}
\end{equation}
but an interpretation of this kind is not suitable for elements from the second group. In general, non-zero off-diagonal terms in the FIM indicate correlations between inferred parameters\cite{heavens2016generalisations}. More specifically, the FIM of a parameter vector $\theta=[\theta_1^T\quad\theta_2^T]^T$ can be written as a block- matrix:
\begin{equation}
I(\theta)=\begin{pmatrix}
I_{11} & I_{12}\\
I_{21} & I_{22}
\end{pmatrix}
\end{equation}
where $I_{ii}=I(\theta_i)$ contains the FIM of the sub vectors when another one is known, and $I_{12}=I_{21}^T$ contains the mixed second derivation expectations. In order to extract the CRB, the inversed matrix parts need to be examined; for example the part that belongs to $\theta_1$:
\begin{equation}
I^{-1}(\theta)_{\theta_1,\theta_1}=(I_{11}-I_{12}I_{22}^{-1}I_{21})^{-1}
\end{equation}
If $I_{12}=\boldmath{0}$, so $I^{-1}(\theta)_{\theta_1,\theta_1}=I_{11}^{-1}$ and there is no interference caused by lack of knowledge of $\theta_2$. If not, lack of knowledge of $\theta_2$ damages the $\theta_1$ estimation quality. As a result, its estimator's lowest variance increases. \\
The CRB and FIM point to asymptotic behavior. Thus, even though $I_{12}=\boldmath{0}$, there is not an absolute independence between the estimations, but rather an asymptotic one. For instance, if the $\theta_2$ estimation converges extremely fast then the $\theta_1$ estimation, the cross elements in the joint FIM will be zero, because in the asymptotic case, $\theta_2$ is "constant" in comparison to $\theta_1$.

\subsection{Maximum Likelihood Estimation}
In this thesis, the estimator that was chosen is the maximum-likelihood-estimator (MLE).\\
MLE's basic formula for estimating $\theta$ from a sample vector $\textbf{x}$ is:
\begin{equation}
\hat{\theta}=\arg\max_{\theta} L(\theta)
\end{equation}   
where $L(\theta)$ is the likelihood function:
\begin{equation}
L(\theta)=f(\textbf{x}|\theta).
\end{equation}
This simplst and most straightforward estimation method has some very strong properties, as described below.
\subsubsection{Consistency}
Under the conditions outlined below, the maximum likelihood estimator is consistent. Consistency means that if the data were generated by $f(\cdot;\theta _{0})$ and there is a sufficiently large number of observations $n$, then it is possible to find the value of $\theta_0$ with arbitrary precision. In mathematical terms this means that as $n$ goes to infinity the estimator $\widehat{\theta}$ converges in probability to its true value:
\begin{equation}
\widehat{\theta}_{\mathrm {mle}}\xrightarrow{\text{p}}\theta _{0}.
\end{equation}
In other words, MLE is an asymptotic unbiased estimator.
To establish consistency, the following conditions are sufficient.
\begin{itemize}
	\item Identification of the model:
	\begin{equation}
	\theta \neq \theta _{0}\quad \Leftrightarrow \quad f(\cdot \mid \theta )\neq f(\cdot \mid \theta _{0}).
	\end{equation}
	In other words, different parameter values $\theta$ correspond to different distributions within the model. If this condition did not hold, there would be some value $\theta_1$ such that $\theta_0$ and $\theta_1$ would generate an identical distribution of the observable data. In this case we would not be able to distinguish between these two parameters even with an infinite amount of data, since these parameters would be observationally equivalent.
	The identification condition is absolutely necessary for the ML estimator to be consistent. When this condition holds, the limiting likelihood function $L(\theta)$ has a single global maximum at $\theta_0$.
	\item Compactness: the parameter space $\Theta$ of the model is compact.\\
	The identification condition establishes that the log-likelihood has a single global maximum. Compactness implies that the likelihood cannot approach the maximum value arbitrarily close at some other point.\\
	Compactness is only a sufficient condition and not a necessary condition. It can be replaced by some other conditions, such as:
	\begin{itemize}
		\item both concavity of the log-likelihood function and compactness of some (nonempty) upper level sets of the log-likelihood function.
		\item existence of a compact neighborhood $N$ of $\theta_0$ such that outside of $N$ the log-likelihood function is less than the maximum by at least some $\epsilon>0$.
	\end{itemize}
	\item Continuity: the function $\ln f(x|\theta)$ is continuous in $\theta$ for almost all values of $x$:
	\begin{equation}
	\operatorname {P} \big[\ln f(x\mid \theta )\in C^0(\Theta )\big]=1.
	\end{equation}
	\item Dominance: there exists $D(x)$ integrable with respect to the distribution $f(x | \theta_0)$ such that
	\begin{equation}
	{\big|}\ln f(x\mid \theta ){\big |}<D(x)\quad {\text{ for all }}\theta \in \Theta .
	\end{equation}
	The dominance condition can be employed in the case of i.i.d. observations. 
\end{itemize}

\subsubsection{Invariance}
This property means that the estimation of the transformation of parameter equals the transformation of the estimation of the parameter. Invariance is very helpful in many cases, such as the case where the probability density function of the transformed parameter is complicated. If $g(\theta )$ is any transformation of $\theta$, then the MLE for $\alpha =g(\theta )$ is by definition
\begin{equation}
\widehat{\alpha }=g(\widehat{\theta}).
\end{equation}
It maximizes the so-called profile likelihood:
\begin{equation}
{\bar {L}}(\alpha )=\sup_{\theta :\alpha =g(\theta )}L(\theta ).
\end{equation}
The explanation is simple: if $y=g(x)$ where $g$ is an injective function and does not depend on the parameters to be estimated, then the density functions satisfy
\begin{equation}
f_{Y}(y)=\frac{f_{X}(x)}{|g'(x)|}
\end{equation}
and hence the likelihood functions for $X$ and $Y$ differ only by a factor that does not depend on the model parameters.

\subsubsection{Efficiency}
As assumed above, and the data were generated by $f(\cdot;\theta_{0})$, then under certain conditions, it can also be shown that the maximum likelihood estimator converges in distribution to a normal distribution. It is $\sqrt{n}$ -consistent and asymptotically efficient; in other words, its variance reaches the CRB. Specifically,
\begin{equation}
\sqrt{n}(\widehat{\theta}_{\text{mle}}-\theta_0)\xrightarrow{d}\mathcal{N}(0,I(\theta_0)^{-1}),
\end{equation}
where $I(\theta_{0})$ is the Fisher Information matrix, as explained above.


==> Chapters/background_after_itsik.tex <==
In this section, the theoretical background used for the thesis is presented. First of all, the relevant estimation methods are explained in detail. Then, some concepts derived from performance evaluation theory are presented, and the estimator is described.

\subsection{RSS}\label{chap:background_rss}
The assumption behind received-signal-strength (RSS) localization is that a significant information for source location estimation is included in the signal's amplitude.\\ 
\begin{comment}
In other words, the strongest effect of distancing from the source is manifested by the amplitude attenuation. An optional mathematical formulation for rss estimation is found in \cite{fujiistudy}:
\begin{equation}
r=n\alpha d^{-\beta}
\end{equation}
where $r$ is the received power signal, $\alpha$ is a constant value corresponding to the transmitted signal power, $n$ is a scaling factor depending on the wireless system, $d$ is the distance from the source that needs to be estimated, and $\beta$ is the pathloss exponent. It is assumed that the RSS is constant, but $n$ is a random variable
in a typical wireless environment. The variation of $n$ involves
that of the RSS $r$. As a result, $r$ is also a random variable controlled by $n$, where $n$ is a sample of exponential random variable $N$. In other words, the Probability Density Function (PDF) of the random
variable is given by
\begin{equation}
p_N(n)=\exp (-n).
\end{equation}
As a consequence, and denoting $r$ as a sample of a random variable $R$, one can easily find the PDF of $R$:
\begin{equation}
p_R(r)=\frac{1}{\alpha d^{-\beta}}\exp \left(-\frac{r}{\alpha d^{-\beta}}\right).
\end{equation}
\end{comment}
The signal's amplitude is used to measure the distance from a sensor to the source. After finding the distance, one can define a circle around the sensor which is a collection of all the alternative source locations as a function of the specific sensor's measurements. In an ideal situation, the circles of all the sensors should intersect at one point, which is the real source location. However, because of noise, the circles are almost never intersect at one point, and the estimator needs to deal with ambiguity in estimating the source location. The solution is usually Maxiumm-Likelihood estimation (MLE), which is discussed later.\\
RSS assumption exists only for short distances. For long distances, the amplitude attenuation is hard to measure accurately and TOA estimation will probably yield better results.  % TOA

\subsection{TOA}
In time-of-arrival (TOA) localization, the sensors extract timing information from the received signals, whereas we assume that the exact transmission time is known to all sensors\footnote{In some publications, the term TOA is also used when the transmission time is not known in advance, but is estimated during the localization process. To clarify our notation, we use the term TOA if the transmission time is known in advance, and TDOA when this time is not known (regardless of the estimation algorithm).}. Accordingly, the transmission time is a known constant and can be chosen as zero without loss of generality (WLOG). For instance, the received signal's mathematical formulation can be
\begin{equation}
r(t)=s\left(t-\frac{d}{c}\right)+n(t)
\end{equation}
where $s(t)$ is the transmitted signal, $d$ is the distance from the source that should be estimated, $c$ is the signal's expansion speed, and $n(t)$ is additive white Gaussian noise (AWGN), so the signal's PDF is
\begin{equation}
p_R(r(t))=\frac{1}{\sqrt{2\pi \sigma_n^2}}\exp\left(-\frac{(r(t)-s(t-\frac{d}{c}))^2}{2\sigma_n^2}\right)
\end{equation}
This method has been explored extensively in the literature, even though its main assumption is hard to satisfy \cite{myref11,myref13}.  % TDOA

\subsection{TDOA}
In time-difference-of-arrival (TDOA), in contrast to TOA, the transmission time is unknown. Thus, such systems are much simpler to implement than TOA. Some TDOA models assume that all signals received by each sensor have the same signal to noise ratio (SNR) \cite{geofdtd,TDFD,myref2,accuracyanalysis}, while others are more general and allow different SNR at different sensors \cite{HybDis,generalMeasurements,myref12,myref13}. An optional mathematical formulation for the received signal in TDOA estimation is:
\begin{equation}
r(t)=s(t-\tau-T_0)+v(t)\qquad t\in\mathbb{R}_+
\end{equation}
where $s(t)$ is the known transmitted signal, $\tau = D/c$ is the time delay, $c$ is the speed of light,
\begin{equation}
D=\sqrt{(x_{s}-x)^2+(y_s-y)^2}
\end{equation}
is the distance between the source and the sensor, $v(t)$ is a white Gaussian noise with spectral density $N_0/2$, and $T_0$ is the transmission time which is assumed to be unknown. Thus, $r(t)$'s PDF can be trivially concluded from the case of TOA. Even though TOA and TDOA look very similar and close, there is at least one significant difference between them. In TOA the parameter vector for estimation only contains the wanted information; i.e., the source location. In TDOA, on the contrary, $T_0$ is added as a nuisance parameter and one dimension is added to the search process. As a result, one disadvantage of TDOA-based localization methods is computational complexity. It is therefore important to develop bounds on the estimation error. As noted above, some lower bounds for different signal models can be found in the literature, but only in matrix form. In other words, there is no explicit term for TDOA estimation performance evaluation. According to its computational complexity on the one hand, and its practical importance on the other, a short and intuitive expression for performance evaluation could considerably improve the human understanding in this method and as a result enhance its potential performance. %AOA

\begin{comment}
	\subsection{AOA}
In contrast to the previous estimation methods described above, which are based on distance estimation for source localization, the angle-of-arrival (AOA) method estimates the angle between the source and the horizon to re-evaluate the source location. For angle estimation to be possible, directional sensors are needed, such as phased antenna arrays, mechanically steerable antennas, or
multiple antennas\cite{jais2015review}. The mathematical formulation of the received signal obviously depends on the antennas array's specific shape. As an example, when the antennas array is organized as a line with a constant space between each antenna, the formulation can be written as follows\cite{mohanna2013optimization}:
\begin{equation}
\textbf{r}(k)=\textbf{a}(\theta)s(k)+\textbf{n}(k)
\end{equation}
where $k$ is a discrete time index, $\textbf{r}$ is the received signal, $s$ is the transmitted signal, $\textbf{n}$ is AWGN and $\textbf{a}$ is the steering vector, which contains the total influence of $\theta$ on $\textbf{r}$ and is explicitly folmulated as follows:
\begin{equation}
\textbf{a}(\theta)=[1 e^{j\beta d\sin(\theta)} e^{j2\beta d\sin(\theta)} ... e^{j(M-1)\beta d\sin(\theta)}]^T
\end{equation}
or in other words:
\begin{equation}
\textbf{a}_m(\theta)=\exp(j(m-1)\beta d\sin(\theta))
\end{equation}
where $\beta=2\pi/\lambda$ is the incident wave number, $d$ is inter-element spacing, and $\theta$ is the wanted unknown angle of arrival. The received signal is a vector since the analysis is performed simultaneously for all the antennas in the array and each element in the vector belongs to a different antenna.\\
The noise model is the same as in TOA and TDOA so that the PDF can simply be concluded.


\end{comment}
\subsection{FIM and CRB}
One of the most frequently used measures in statistical signal processing is the Fisher Information Matrix (FIM). In general, the Fisher Information is a way of measuring the amount of information that an observable random variable $X$ carries about an unknown parameter $\theta$ upon which the probability of $X$ depends. When $\theta$ is a scalar, the Fisher Information is defined as follows:
\begin{equation}
I(\theta)={\mathbb E}\left[\left.\left({\frac {\partial }{\partial \theta }}\log f(X;\theta )\right)^{2}\right|\theta \right].
\end{equation}
When the regularity condition 
\begin{equation}
{\mathbb E} \left[\frac{\partial }{\partial \theta }\log f(X;\theta )|\theta \right]=0
\end{equation}
exists and $\log f(x;\theta)$ is twice differentiable with respect to $\theta$, it can be shown that 
\begin{equation}
{\mathbb E} \left[\left(\frac{\partial }{\partial \theta }\log f(X;\theta )\right)^{2}|\theta \right]=-{\mathbb E} \left[{\frac {\partial^2 }{\partial \theta^2 }}\log f(X;\theta )|\theta \right].
\end{equation}
The Fisher Information may be seen as the curvature of the support curve (the graph of the log-likelihood). Near the maximum likelihood estimate, low Fisher Information therefore indicates that the maximum appears "blunt"; that is, the maximum is shallow and there are many nearby values with a similar log-likelihood. Conversely, high Fisher Information indicates that the maximum is sharp. \\
When $\theta$ is a vector of $N$ parameters, the Fisher Information takes an $N\times N$ matrix form, and its $i,j$ element is defined as follows:
\begin{equation}
\bigl [I(\theta ){\bigr ]}_{i,j}={\mathbb E} \left[\left({\frac {\partial }{\partial \theta _{i}}}\log f(X;\theta )\right)\left({\frac {\partial }{\partial \theta _{j}}}\log f(X;\theta )\right)|\theta \right]
\end{equation}
or as in the previous case,
\begin{equation}
\bigl [I(\theta )\bigr ]_{i,j}=-{\mathbb E} \left[{\frac {\partial ^{2}}{\partial \theta _{i}\partial \theta _{j}}}\log f(X;\theta )|\theta \right].
\end{equation}
The FIM has several interpretations in different fields. In machine learning, for example, it is used in elastic weight consolidation\cite{kirkpatrick2017overcoming}, which reduces catastrophic forgetting in artificial neural networks. Another use of Fisher Information is in computational neuroscience, where it is used to find bounds on the accuracy of neural codes.\\
In the estimation theory context, FIM is interpreted as the inverse of the lower bound on the estimator variance, which is known as the Cram\'{e}r-Rao bound (CRB). The CRB has slightly different versions for biased and unbiased estimators, and in this thesis the unbiased estimator's version is discussed. In mathematical terms, if $\widehat{\theta}$ is any estimator of the unknown parameter $\theta$, then
\begin{equation}
VAR(\widehat{\theta})\geq I(\theta )^{-1}.
\end{equation}
When $\theta$ is a scalar, the meaning of $I(\theta)$ is clear. However, if $\theta$ is a vector, $I(\theta)$ is a matrix whose elements' meaning is not initially clear. To clarify this point, the elements need to be seperated into two different groups- on the diagonal, and not on the diagonal. The elements in the diagonal have a similar meaning as in the scalar case:
\begin{equation}
VAR(\widehat{\theta}_i)\geq [I(\theta )^{-1}]_{ii}
\end{equation}
but an interpretation of this kind is not suitable for elements from the second group. In general, non-zero off-diagonal terms in the FIM indicate correlations between inferred parameters\cite{heavens2016generalisations}. More specifically, the FIM of a parameter vector $\theta=[\theta_1^T\quad\theta_2^T]^T$ can be written as a block- matrix:
\begin{equation}
I(\theta)=\begin{pmatrix}
I_{11} & I_{12}\\
I_{21} & I_{22}
\end{pmatrix}
\end{equation}
where $I_{ii}=I(\theta_i)$ contains the FIM of the sub vectors when another one is known, and $I_{12}=I_{21}^T$ contains the mixed second derivation expectations. In order to extract the CRB, the inversed matrix parts need to be examined; for example the part that belongs to $\theta_1$:
\begin{equation}
I^{-1}(\theta)_{\theta_1,\theta_1}=(I_{11}-I_{12}I_{22}^{-1}I_{21})^{-1}
\end{equation}
If $I_{12}=\boldmath{0}$, so $I^{-1}(\theta)_{\theta_1,\theta_1}=I_{11}^{-1}$ and there is no interference caused by lack of knowledge of $\theta_2$. If not, lack of knowledge of $\theta_2$ damages the $\theta_1$ estimation quality. As a result, its estimator's lowest variance increases. \\
The CRB and FIM point to asymptotic behavior. Thus, even though $I_{12}=\boldmath{0}$, there is not an absolute independence between the estimations, but rather an asymptotic one. For instance, if the $\theta_2$ estimation converges extremely fast then the $\theta_1$ estimation, the cross elements in the joint FIM will be zero, because in the asymptotic case, $\theta_2$ is "constant" in comparison to $\theta_1$.

\subsection{Maximum Likelihood Estimation}
In this thesis, the estimator that was chosen is the maximum-likelihood-estimator (MLE).\\
MLE's basic formula for estimating $\theta$ from a sample vector $\textbf{x}$ is:
\begin{equation}
\hat{\theta}=\arg\max_{\theta} L(\theta)
\end{equation}   
where $L(\theta)$ is the likelihood function:
\begin{equation}
L(\theta)=f(\textbf{x}|\theta).
\end{equation}
This simplst and most straightforward estimation method has some very strong properties, as described below.
\subsubsection{Consistency}
Under the conditions outlined below, the maximum likelihood estimator is consistent. Consistency means that if the data were generated by $f(\cdot;\theta _{0})$ and there is a sufficiently large number of observations $n$, then it is possible to find the value of $\theta_0$ with arbitrary precision. In mathematical terms this means that as $n$ goes to infinity the estimator $\widehat{\theta}$ converges in probability to its true value:
\begin{equation}
\widehat{\theta}_{\mathrm {mle}}\xrightarrow{\text{p}}\theta _{0}.
\end{equation}
In other words, MLE is an asymptotic unbiased estimator.
To establish consistency, the following conditions are sufficient.
\begin{itemize}
	\item Identification of the model:
	\begin{equation}
	\theta \neq \theta _{0}\quad \Leftrightarrow \quad f(\cdot \mid \theta )\neq f(\cdot \mid \theta _{0}).
	\end{equation}
	In other words, different parameter values $\theta$ correspond to different distributions within the model. If this condition did not hold, there would be some value $\theta_1$ such that $\theta_0$ and $\theta_1$ would generate an identical distribution of the observable data. In this case we would not be able to distinguish between these two parameters even with an infinite amount of data, since these parameters would be observationally equivalent.
	The identification condition is absolutely necessary for the ML estimator to be consistent. When this condition holds, the limiting likelihood function $L(\theta)$ has a single global maximum at $\theta_0$.
	\item Compactness: the parameter space $\Theta$ of the model is compact.\\
	The identification condition establishes that the log-likelihood has a single global maximum. Compactness implies that the likelihood cannot approach the maximum value arbitrarily close at some other point.\\
	Compactness is only a sufficient condition and not a necessary condition. It can be replaced by some other conditions, such as:
	\begin{itemize}
		\item both concavity of the log-likelihood function and compactness of some (nonempty) upper level sets of the log-likelihood function.
		\item existence of a compact neighborhood $N$ of $\theta_0$ such that outside of $N$ the log-likelihood function is less than the maximum by at least some $\epsilon>0$.
	\end{itemize}
	\item Continuity: the function $\ln f(x|\theta)$ is continuous in $\theta$ for almost all values of $x$:
	\begin{equation}
	\operatorname {P} \big[\ln f(x\mid \theta )\in C^0(\Theta )\big]=1.
	\end{equation}
	\item Dominance: there exists $D(x)$ integrable with respect to the distribution $f(x | \theta_0)$ such that
	\begin{equation}
	{\big|}\ln f(x\mid \theta ){\big |}<D(x)\quad {\text{ for all }}\theta \in \Theta .
	\end{equation}
	The dominance condition can be employed in the case of i.i.d. observations. 
\end{itemize}

\subsubsection{Invariance}
This property means that the estimation of the transformation of parameter equals the transformation of the estimation of the parameter. Invariance is very helpful in many cases, such as the case where the probability density function of the transformed parameter is complicated. If $g(\theta )$ is any transformation of $\theta$, then the MLE for $\alpha =g(\theta )$ is by definition
\begin{equation}
\widehat{\alpha }=g(\widehat{\theta}).
\end{equation}
It maximizes the so-called profile likelihood:
\begin{equation}
{\bar {L}}(\alpha )=\sup_{\theta :\alpha =g(\theta )}L(\theta ).
\end{equation}
The explanation is simple: if $y=g(x)$ where $g$ is an injective function and does not depend on the parameters to be estimated, then the density functions satisfy
\begin{equation}
f_{Y}(y)=\frac{f_{X}(x)}{|g'(x)|}
\end{equation}
and hence the likelihood functions for $X$ and $Y$ differ only by a factor that does not depend on the model parameters.

\subsubsection{Efficiency}
As assumed above, and the data were generated by $f(\cdot;\theta_{0})$, then under certain conditions, it can also be shown that the maximum likelihood estimator converges in distribution to a normal distribution. It is $\sqrt{n}$ -consistent and asymptotically efficient; in other words, its variance reaches the CRB. Specifically,
\begin{equation}
\sqrt{n}(\widehat{\theta}_{\text{mle}}-\theta_0)\xrightarrow{d}\mathcal{N}(0,I(\theta_0)^{-1}),
\end{equation}
where $I(\theta_{0})$ is the Fisher Information matrix, as explained above.


==> Chapters/background_after_itsik_yair.tex <==
In this section, the theoretical background used for the thesis is presented. First of all, the relevant estimation methods are explained in detail. Then, some concepts from performance evaluation theory are presented, and the estimator is described.

\subsection{RSS}\label{chap:background_rss}
The assumption behind received-signal-strength (RSS) localization is that a significant information for source location estimation is included in the signal amplitude.\\ 
\begin{comment}
In other words, the strongest effect of distancing from the source is manifested by the amplitude attenuation. An optional mathematical formulation for rss estimation is found in \cite{fujiistudy}:
\begin{equation}
r=n\alpha d^{-\beta}
\end{equation}
where $r$ is the received power signal, $\alpha$ is a constant value corresponding to the transmitted signal power, $n$ is a scaling factor depending on the wireless system, $d$ is the distance from the source that needs to be estimated, and $\beta$ is the pathloss exponent. It is assumed that the RSS is constant, but $n$ is a random variable
in a typical wireless environment. The variation of $n$ involves
that of the RSS $r$. As a result, $r$ is also a random variable controlled by $n$, where $n$ is a sample of exponential random variable $N$. In other words, the Probability Density Function (PDF) of the random
variable is given by
\begin{equation}
p_N(n)=\exp (-n).
\end{equation}
As a consequence, and denoting $r$ as a sample of a random variable $R$, one can easily find the PDF of $R$:
\begin{equation}
p_R(r)=\frac{1}{\alpha d^{-\beta}}\exp \left(-\frac{r}{\alpha d^{-\beta}}\right).
\end{equation}
\end{comment}
The signal amplitude is used to measure the distance from a sensor to the source. After finding the distance, one can define a circle around the sensor which is a collection of all the alternative source locations as a function of the specific sensor measurements. In an ideal situation, the circles of all the sensors should intersect at one point, which is the real source location. However, because of noise, the circles are almost never intersect at one point, and the estimator must deal with ambiguity in estimating the source location. The solution is usually Maxiumm-Likelihood estimation (MLE), which is discussed later.\\
RSS assumption exists only for short distances. In the long distance, it is difficult to measure the amplitude attenuation accurately and TOA estimation usually yield better results.  % TOA

\subsection{TOA}
In time-of-arrival (TOA) localization, the sensors extract timing information from the received signals, whereas we assume that the exact transmission time is known to all sensors\footnote{In some publications, the term TOA is also used when the transmission time is not known in advance, but is estimated during the localization process. To clarify our notation, we use the term TOA if the transmission time is known in advance, and TDOA when this time is not known (regardless of the estimation algorithm).}. Accordingly, the transmission time is a known constant and can be chosen as zero without loss of generality (WLOG). For instance, the received signal mathematical formulation can be
\begin{equation}
r(t)=s\left(t-\frac{d}{c}\right)+n(t)
\end{equation}
where $s(t)$ is the transmitted signal, $d$ is the distance from the source that should be estimated, $c$ is the signal expansion speed, and $n(t)$ is additive white Gaussian noise (AWGN), so the signal PDF is
\begin{equation}
p_R(r(t))=\frac{1}{\sqrt{2\pi \sigma_n^2}}\exp\left(-\frac{(r(t)-s(t-\frac{d}{c}))^2}{2\sigma_n^2}\right)
\end{equation}
This method has been explored extensively in the literature, even though its main assumption is hard to satisfy \cite{myref11,myref13}.  % TDOA

\subsection{TDOA}
In time-difference-of-arrival (TDOA), in contrast to TOA, the transmission time is unknown. Thus, such systems are much simpler to implement than TOA. Some TDOA models assume that all signals received by each sensor have the same signal to noise ratio (SNR) \cite{geofdtd,TDFD,myref2,accuracyanalysis}, while others are more general and allow different SNR at different sensors \cite{HybDis,generalMeasurements,myref12,myref13}. An optional mathematical formulation for the received signal in TDOA estimation is:
\begin{equation}
r(t)=s(t-\tau-T_0)+v(t)\qquad t\in\mathbb{R}_+
\end{equation}
where $s(t)$ is the known transmitted signal, $\tau = D/c$ is the time delay, $c$ is the speed of light,
\begin{equation}
D=\sqrt{(x_{s}-x)^2+(y_s-y)^2}
\end{equation}
is the distance between the source and the sensor, $v(t)$ is a white Gaussian noise with spectral density $N_0/2$, and $T_0$ is the transmission time which is assumed to be unknown. Thus,the likelihood for TDOA estimation from $r(t)$ can be trivially concluded from the case of TOA. Even though TOA and TDOA look very similar and close, there is at least one significant difference between them. In TOA the parameter vector for estimation only contains the desirable information; i.e., the source location. In TDOA, on the contrary, $T_0$ is added as a nuisance parameter and one dimension is added to the search process. As a result, one disadvantage of TDOA-based localization methods is computational complexity. It is therefore important to develop bounds on the estimation error. As noted above, some lower bounds for different signal models can be found in the literature, but only in matrix form. In other words, there is no explicit term for TDOA estimation performance evaluation. Since TDOA estimation is a fundamental problem in signal processing, it is important to develop a short and intuitive expression for performance evaluation. %AOA

\begin{comment}
	\subsection{AOA}
In contrast to the previous estimation methods described above, which are based on distance estimation for source localization, the angle-of-arrival (AOA) method estimates the angle between the source and the horizon to re-evaluate the source location. For angle estimation to be possible, directional sensors are needed, such as phased antenna arrays, mechanically steerable antennas, or
multiple antennas\cite{jais2015review}. The mathematical formulation of the received signal obviously depends on the antennas array's specific shape. As an example, when the antennas array is organized as a line with a constant space between each antenna, the formulation can be written as follows\cite{mohanna2013optimization}:
\begin{equation}
\textbf{r}(k)=\textbf{a}(\theta)s(k)+\textbf{n}(k)
\end{equation}
where $k$ is a discrete time index, $\textbf{r}$ is the received signal, $s$ is the transmitted signal, $\textbf{n}$ is AWGN and $\textbf{a}$ is the steering vector, which contains the total influence of $\theta$ on $\textbf{r}$ and is explicitly folmulated as follows:
\begin{equation}
\textbf{a}(\theta)=[1 e^{j\beta d\sin(\theta)} e^{j2\beta d\sin(\theta)} ... e^{j(M-1)\beta d\sin(\theta)}]^T
\end{equation}
or in other words:
\begin{equation}
\textbf{a}_m(\theta)=\exp(j(m-1)\beta d\sin(\theta))
\end{equation}
where $\beta=2\pi/\lambda$ is the incident wave number, $d$ is inter-element spacing, and $\theta$ is the wanted unknown angle of arrival. The received signal is a vector since the analysis is performed simultaneously for all the antennas in the array and each element in the vector belongs to a different antenna.\\
The noise model is the same as in TOA and TDOA so that the PDF can simply be concluded.


\end{comment}
\subsection{FIM and CRB}
One of the most frequently used measures in statistical signal processing is the Fisher Information Matrix (FIM). In general, the Fisher Information is a way of measuring the amount of information that an observable random variable $X$ carries about an unknown parameter $\theta$ upon which the probability of $X$ depends. When $\theta$ is a scalar, the Fisher Information is defined as follows:
\begin{equation}
I(\theta)={\mathbb E}\left[\left.\left({\frac {\partial }{\partial \theta }}\log f(X;\theta )\right)^{2}\right|\theta \right].
\end{equation}
When the regularity condition 
\begin{equation}
{\mathbb E} \left[\frac{\partial }{\partial \theta }\log f(X;\theta )|\theta \right]=0
\end{equation}
exists and $\log f(x;\theta)$ is twice differentiable with respect to $\theta$, it can be shown that 
\begin{equation}
{\mathbb E} \left[\left(\frac{\partial }{\partial \theta }\log f(X;\theta )\right)^{2}|\theta \right]=-{\mathbb E} \left[{\frac {\partial^2 }{\partial \theta^2 }}\log f(X;\theta )|\theta \right].
\end{equation}
The Fisher Information may be seen as the curvature of the support curve (the graph of the log-likelihood). Near the maximum likelihood estimate, low Fisher Information therefore indicates that the maximum appears "blunt"; that is, the maximum is shallow and there are many nearby values with a similar log-likelihood. Conversely, high Fisher Information indicates that the maximum is sharp. \\
When $\boldsymbol{\theta}$ is a vector of $N$ parameters, the Fisher Information takes an $N\times N$ matrix form, and its $i,j$ element is defined as follows:
\begin{equation}
\bigl [I(\boldsymbol{\theta}){\bigr ]}_{i,j}={\mathbb E} \left[\left({\frac {\partial }{\partial \boldsymbol{\theta} _{i}}}\log f(X;\boldsymbol{\theta})\right)\left({\frac {\partial }{\partial \boldsymbol{\theta}_{j}}}\log f(X;\boldsymbol{\theta} )\right)|\boldsymbol{\theta}\right]
\end{equation}
or as in the previous case,
\begin{equation}
\bigl [I(\boldsymbol{\theta})\bigr ]_{i,j}=-{\mathbb E} \left[{\frac {\partial ^{2}}{\partial\boldsymbol{\theta}_{i}\partial\boldsymbol{\theta} _{j}}}\log f(X;\boldsymbol{\theta})|\boldsymbol{\theta}\right].
\end{equation}
The FIM has several interpretations in different fields. In machine learning, for example, it is used in elastic weight consolidation\cite{kirkpatrick2017overcoming}, which reduces catastrophic forgetting in artificial neural networks. Another use of Fisher Information is in computational neuroscience, where it is used to find bounds on the accuracy of neural codes.\\
In the estimation theory context, FIM is interpreted as the inverse of the lower bound on the estimator variance, which is known as the Cram\'{e}r-Rao bound (CRB). The CRB has slightly different versions for biased and unbiased estimators, and in this thesis the unbiased estimator's version is discussed. In mathematical terms, if $\widehat{\theta}$ is any estimator of the unknown parameter $\theta$, then
\begin{equation}
VAR(\widehat{\theta})\geq I(\theta )^{-1}.
\end{equation}
When $\theta$ is a scalar, the meaning of $I(\theta)$ is clear. However, if $\boldsymbol{\theta}$ is a vector, $I(\theta)$ is a matrix whose elements' meaning is not initially clear. To clarify this point, the elements need to be seperated into two different groups- on the diagonal, and not on the diagonal. The elements in the diagonal have a similar meaning as in the scalar case:
\begin{equation}
VAR(\widehat{\boldsymbol{\theta}}_i)\geq [I(\boldsymbol{\theta})^{-1}]_{ii}
\end{equation}
but an interpretation of this kind is not suitable for elements from the second group. In general, non-zero off-diagonal terms in the FIM indicate correlations between inferred parameters\cite{heavens2016generalisations}. More specifically, the FIM of a parameter vector $\boldsymbol{\theta}=[\boldsymbol{\theta}_1^T\quad\boldsymbol{\theta}_2^T]^T$ can be written as a block- matrix:
\begin{equation}
I(\boldsymbol{\theta})=\begin{pmatrix}
I_{11} & I_{12}\\
I_{21} & I_{22}
\end{pmatrix}
\end{equation}
where $I_{ii}=I(\boldsymbol{\theta}_i)$ contains the FIM of the sub vectors when another one is known, and $I_{12}=I_{21}^T$ contains the mixed second derivation expectations. In order to extract the CRB, the inversed matrix parts need to be examined; for example the part that belongs to $\boldsymbol{\theta}_1$:
\begin{equation}
I^{-1}(\boldsymbol{\theta})_{\boldsymbol{\theta}_1,\boldsymbol{\theta}_1}=(I_{11}-I_{12}I_{22}^{-1}I_{21})^{-1}
\end{equation}
If $I_{12}=\boldmath{0}$, so $I^{-1}(\boldsymbol{\theta})_{\boldsymbol{\theta}_1,\boldsymbol{\theta}_1}=I_{11}^{-1}$ and there is no interference caused by lack of knowledge of $\boldsymbol{\theta}_2$. If not, lack of knowledge of $\boldsymbol{\theta}_2$ damages the $\boldsymbol{\theta}_1$ estimation quality. As a result, its estimator's lowest variance increases. \\
The CRB and FIM point to asymptotic behavior. Thus, even though $I_{12}=\boldmath{0}$, there is not an absolute independence between the estimations, but rather an asymptotic one. For instance, if the $\boldsymbol{\theta}_2$ estimation converges extremely fast then the $\boldsymbol{\theta}_1$ estimation, the cross elements in the joint FIM will be zero, because in the asymptotic case, $\boldsymbol{\theta}_2$ is "constant" in comparison to $\boldsymbol{\theta}_1$.

\subsection{Maximum Likelihood Estimation}
In this thesis, the estimator that was chosen is the maximum-likelihood-estimator (MLE).\\
MLE's basic formula for estimating $\boldsymbol{\theta}$ from a sample vector $\textbf{x}$ is:
\begin{equation}
\hat{\boldsymbol{\theta}}=\arg\max_{\boldsymbol{\theta}} L(\boldsymbol{\theta})
\end{equation}   
where $L(\boldsymbol{\theta})$ is the likelihood function:
\begin{equation}
L(\boldsymbol{\theta})=f(\textbf{x}|\boldsymbol{\theta}).
\end{equation}
This simplst and most straightforward estimation method has some very strong properties, as described below.
\subsubsection{Consistency}
Under the conditions outlined below, the maximum likelihood estimator is consistent. Consistency means that if the data were generated by $f(\cdot;\boldsymbol{\theta}_{0})$ and there is a sufficiently large number of observations $n$, then it is possible to find the value of $\boldsymbol{\theta}_0$ with arbitrary precision. In mathematical terms this means that as $n$ goes to infinity the estimator $\widehat{\boldsymbol{\theta}}$ converges in probability to its true value:
\begin{equation}
\widehat{\boldsymbol{\theta}}_{\mathrm {mle}}\xrightarrow{\text{p}}\boldsymbol{\theta}_{0}.
\end{equation}
In other words, MLE is an asymptotic unbiased estimator.
To establish consistency, the following conditions are sufficient.
\begin{itemize}
	\item Identification of the model:
	\begin{equation}
	\boldsymbol{\theta} \neq \boldsymbol{\theta} _{0}\quad \Leftrightarrow \quad f(\cdot \mid \boldsymbol{\theta})\neq f(\cdot \mid \boldsymbol{\theta}_{0}).
	\end{equation}
	In other words, different parameter values $\boldsymbol{\theta}$ correspond to different distributions within the model. If this condition did not hold, there would be some value $\boldsymbol{\theta}_1$ such that $\boldsymbol{\theta}_0$ and $\boldsymbol{\theta}_1$ would generate an identical distribution of the observable data. In this case we would not be able to distinguish between these two parameters even with an infinite amount of data, since these parameters would be observationally equivalent.
	The identification condition is absolutely necessary for the ML estimator to be consistent. When this condition holds, the limiting likelihood function $L(\boldsymbol{\theta})$ has a single global maximum at $\boldsymbol{\theta}_0$.
	\item Compactness: the parameter space $\Theta$ of the model is compact.\\
	The identification condition establishes that the log-likelihood has a single global maximum. Compactness implies that the likelihood cannot approach the maximum value arbitrarily close at some other point.\\
	Compactness is only a sufficient condition and not a necessary condition. It can be replaced by some other conditions, such as:
	\begin{itemize}
		\item both concavity of the log-likelihood function and compactness of some (nonempty) upper level sets of the log-likelihood function.
		\item existence of a compact neighborhood $N$ of $\boldsymbol{\theta}_0$ such that outside of $N$ the log-likelihood function is less than the maximum by at least some $\epsilon>0$.
	\end{itemize}
	\item Continuity: the function $\ln f(x|\boldsymbol{\theta})$ is continuous in $\boldsymbol{\theta}$ for almost all values of $x$:
	\begin{equation}
	\operatorname {P} \big[\ln f(x\mid \boldsymbol{\theta})\in C^0(\Theta )\big]=1.
	\end{equation}
	\item Dominance: there exists $D(x)$ integrable with respect to the distribution $f(x |\boldsymbol{\theta}_0)$ such that
	\begin{equation}
	{\big|}\ln f(x\mid \boldsymbol{\theta}){\big |}<D(x)\quad {\text{ for all }}\boldsymbol{\theta} \in \Theta .
	\end{equation}
	The dominance condition can be employed in the case of i.i.d. observations. 
\end{itemize}

\subsubsection{Invariance}
This property means that the estimation of the transformation of parameter equals the transformation of the estimation of the parameter. Invariance is very helpful in many cases, such as the case where the probability density function of the transformed parameter is complicated. If $g(\boldsymbol{\theta})$ is any transformation of $\boldsymbol{\theta}$, then the MLE for $\alpha =g(\boldsymbol{\theta})$ is by definition
\begin{equation}
\widehat{\alpha }=g(\widehat{\boldsymbol{\theta}}).
\end{equation}
It maximizes the so-called profile likelihood:
\begin{equation}
{\bar {L}}(\alpha )=\sup_{\boldsymbol{\theta}:\alpha =g(\boldsymbol{\theta} )}L(\boldsymbol{\theta} ).
\end{equation}
The explanation is simple: if $y=g(x)$ where $g$ is an injective function and does not depend on the parameters to be estimated, then the density functions satisfy
\begin{equation}
f_{Y}(y)=\frac{f_{X}(x)}{|g'(x)|}
\end{equation}
and hence the likelihood functions for $X$ and $Y$ differ only by a factor that does not depend on the model parameters.

\subsubsection{Efficiency}
As assumed above, and the data were generated by $f(\cdot;\boldsymbol{\theta}_{0})$, then under certain conditions, it can also be shown that the maximum likelihood estimator converges in distribution to a normal distribution. It is $\sqrt{n}$ -consistent and asymptotically efficient; in other words, its variance reaches the CRB. Specifically,
\begin{equation}
\sqrt{n}(\widehat{\boldsymbol{\theta}}_{\text{mle}}-\boldsymbol{\theta}_0)\xrightarrow{d}\mathcal{N}(0,I(\boldsymbol{\theta}_0)^{-1}),
\end{equation}
where $I(\boldsymbol{\theta}_{0})$ is the Fisher Information matrix, as explained above.


==> Chapters/conclusions.tex <==
In this thesis we considered the source localization problem using TDOA measurements. The amplitudes of the signals received by the sensors are assumed to be known to the estimator. For the first time, a closed-form expression for a TDOA network localization CRB is derived. This expression is simple and intuitive, agrees with known facts about TDOA estimation such as the need for at least three sensors to achieve an estimation, but also reveals some new important insights. These insights discussed in depth in this work were the cases where TDOA estimation is equivalent to TOA, or the cases where knowledge of the transmission time becomes meaningless, and a comparison of different amplitude calculation methods was made. This comparison showed that the asymptotic performance is equal in the two cases when the amplitudes are a-priori known or when they are estimated during the localization process as nuisance parameters. One direct conclusion is that the new explicit bound is even appropriate for to the second estimation type.
\par 
This explicit expression paves the way for a variety of future research directions. These could include optimizing the sensor scattering to minimize the resulting CRB. Because of the MLE efficiency property, minimizing the CRB is equivalent to upgrading MLE performance. Another direction for future research would be to examine the influence of small fluctuations in the sensors' locations on the CRB. This direction is important with respect to actual settings today, when sensor location accuracy is not always perfect.

==> Chapters/formulation.tex <==
In this section, the model formulation and assumptions are detailed. We consider a single source, with an unknown location that transmits a known signal $s(t)$ isotropically over $\mathbb{R}^2$. The signal transmission begins at an unknown time, $T_0$, and is received by an infinitely countable number of sensors. Ideal communication to the fusion center is assumed. While this assumption is not practical, it simplifies the theoretical study and enables a closed-form derivation of the bound. For the same reasons, we also assume that there are no random fluctuations in the pathloss between the source and each sensor; i.e., no fading effect. In this work, the estimation is based on a continuous time signal and exploits TDOA.\par 
Denote the number of sensors as $M$, the location of sensor $m$ by $\psi_m=(x_m,y_m)\in\mathbb{R}^2$, and the unknown source location by $(x,y)$. We collect these unknown parameters in a vector denoted by $\boldsymbol{\theta}$; i.e., $\boldsymbol{\theta}=[x,y,T_0]^T$. We assume that the locations of the sensors, ${\Psi}=\{\psi_m\}_{m=1}^{M}$, are known to the fusion center. The received signal at the $m$-th sensor is given by\cite{YnoamIbergelTOA}:
\begin{equation}
r_m(t)=k_0D_m^{-\gamma/2}s(t-\tau_m-T_0)+v_m(t)\qquad t\in\mathbb{R}_+;m\in [1,M]\cap\mathbb{N}
\label{sig_shape}
\end{equation}
where $s(t)$ is the known transmitted signal, $\gamma$ as the path-loss exponent, $k_0$ is a constant that depends on the transmission power, antenna gains and carrier frequency, $\tau_m = D_m/c$ is the time delay, $c$ is the speed of light,
\begin{equation}
D_m=\sqrt{(x_m-x)^2+(y_m-y)^2}
\end{equation}
is the distance between the source and the $m$-th sensor, and $v_m(t)$ is a white Gaussian noise with spectral density $N_0/2$. As stated above, in this thesis we assume that there are no random fluctuations in the pathloss between the source and sensors; i.e., no channel fading. In order to exploit TDOA estimation alone and avoid TDOA-RSS estimation, we denote the received amplitudes as $A_m=k_0D_m^{-\gamma/2}$ and assume that $\{A_m\}$ are known to the sensors, but without their RSS interpretation. The derivation requires $s(t)$ to be a continuous, differentiable signal waveform with $s(t)=0$ for all $t\leq 0$ which satisfies
\begin{equation}
|s(t)|, \left|\frac{ds(t)}{dt}\right|, \int_{0}^{\infty}|s(t)|dt,  \int_{0}^{\infty}\left|\frac{ds(t)}{dt}\right|dt <\infty
\end{equation} 
and there exists a monotonic decreasing function $h(t)$, with $\int_{0}^{\infty}h(t)dt<\infty$, such that:
\begin{equation}
|s(t)|, \left|\frac{ds(t)}{dt}\right|\leq h(t)\qquad\forall t.
\end{equation}
In addition, it is convenient to define $E_s=k_0^2\int_{-\infty}^{\infty}s(t)dt$, which is the received signal power at one meter, $\rho=E_s/2N_0$ is the SNR at that distance, 
\begin{equation}
W_e=\frac{\int_{-\infty}^{\infty}(ds(t)/dt)^2dt}{\int_{-\infty}^{\infty}s^2(t)dt}
\end{equation}
is the effective bandwidth, $\phi_m$ is the angle between the source and the $m$th sensor; i.e., $\cos\phi_m=(x-x_m)/D_m$ and $\sin\phi_m=(y-y_m)/D_m$, and $\alpha_{ij}=\phi_i-\phi_j$.

==> Chapters/formulationPPP.tex <==
In this section, the model formulation and assumptions are detailed. We consider a single source, with an unknown location that transmits a known signal $s(t)$ isotropically over $\mathbb{R}^2$. The signal transmission begins at an unknown time, $T_0$, and is received by an infinitely countable number of sensors, scattered according to an HPPP in $\mathbb{R}^2$. Ideal communication to the fusion center is assumed. While this assumption is not practical, it simplifies the theoretical study and enables a closed-form derivation of the bound. For the same reasons, we also assume that there are no random fluctuations in the pathloss between the source and each sensor, i.e., no fading effect. In this work, the estimation is based on a continuous time signal and exploits TDOA.\par 
Denote the location of sensor $m$ by $\psi_m=(x_m,y_m)\in\mathbb{R}^2$, and the unknown source location is $(x,y)$. We collect these unknown parameters in a vector denoted by $\theta$; i.e. $\theta=[x,y,T_0]^T$. The locations of the sensors, $\boldmath{\psi}=\{\psi_m\}_{m=1}^\infty$ is a realization of a $\lambda$-density two-dimensional HPPP, $\Psi$. After the sensors have been randomly scattered in the plane, we assume that the fusion center knows $\mathbb{\psi}$. The received signal at the $m$-th sensor is given by\cite{YnoamIbergelTOA}:
\begin{equation}
	r_m(t)=k_0D_m^{-\gamma/2}s(t-\tau_m-T_0)+v_m(t)\qquad t\in\mathbb{R}_+;m\in\mathbb{N}
\end{equation}
where $s(t)$ is the known transmitted signal, $\gamma$ is the path-loss exponent, $k_0$ is a constant that depends on the transmission power, antenna gains and carrier frequency, $\tau_m = D_m/c$ is the time delay, $c$ is the speed of light,
\begin{equation}
	D_m=\sqrt{(x_m-x)^2+(y_m-y)^2}
\end{equation}
is the distance between the source and the $m$-th sensor, and $v_m(t)$ is a white Gaussian noise with spectral density $N_0/2$. As stated above, in this thesis we assume that there are no random fluctuations in the pathloss between the source and sensors; i.e., no channel fading. The derivation requires $s(t)$ to be a continuous, differentiable signal waveform with $s(t)=0$ for all $t\leq 0$ which satisfies
\begin{equation}
	|s(t)|, \left|\frac{ds(t)}{dt}\right|, \int_{0}^{\infty}|s(t)|dt,  \int_{0}^{\infty}\left|\frac{ds(t)}{dt}\right|dt <\infty
\end{equation} 
and there exists a monotonic decreasing function $h(t)$, with $\int_{0}^{\infty}h(t)dt<\infty$, such that:
\begin{equation}
	|s(t)|, \left|\frac{ds(t)}{dt}\right|\leq h(t)\qquad\forall t.
\end{equation}
In addition, it is convenient to define: $E_s=k_0^2\int_{-\infty}^{\infty}s(t)dt$ is the received signal power at a unit distance, $\rho=E_s/2N_0$ is the SNR, 
\begin{equation}
	W_e=\frac{\int_{-\infty}^{\infty}(ds(t)/dt)^2dt}{\int_{-\infty}^{\infty}s^2(t)dt}
\end{equation}
is the effective bandwidth; $\phi_m$ is the angle between the source and the $m$th sensor; i.e. $\cos\phi_m=(x-x_m)/D_m$ and $\sin\phi_m=(y-y_m)/D_m$, and $\alpha_{ij}=\phi_i-\phi_j$.


==> Chapters/insight1UAA.tex <==
One interesting insight related to the explicit shape of theTDOA CRB explicit shape, is finding the conditions or even situations when the TOA CRB (which is taken from \cite{YnoamIbergelTOA}) equals the TDOA CRB. In other words, the conditions when knowledge of the transmission time $T_0$ has no influence on the quality of the asymptotic estimation. First, the expressions for both TOA CRB and TDOA CRB are given below:
\begin{eqnarray}
\textit{CRB}_{\textit{TDOA}}&=&\frac{6c^2\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij}))}{4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}[\sin(\alpha_{jk})+\sin(\alpha_{ki})+\sin(\alpha_{ij})]^2}\nonumber\\
&=&\frac{3c^2\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij})) }{4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})}.\nonumber\\
&&
\end{eqnarray}
\begin{equation}
\textit{CRB}_{\textit{TOA}}=\frac{c^2\sum_{i=1}^{M}D_i^{-\gamma}}{2W_e\rho\sum_{i=1}^{M}\sum_{j=1}^{M}D_i^{-\gamma}D_j^{-\gamma}\sin^2\alpha_{ij}}
\end{equation}
A basic configuration that should be verified is when all the $M$ sensors are located in the vertices of a perfect polygon around the source, or on a circle centered on the source, with the same angle differences. In mathematic terms:
\begin{equation}
D_i=r\quad\forall i;\qquad \phi_i=\frac{2\pi}{M}i.
\end{equation} 
In this section, the following formula will be used frequently:
\begin{equation}
\sum_{n=0}^{M-1}\cos(\psi+n\alpha)=\frac{\sin(\frac{M\alpha}{2})\cos(\psi+\frac{(M-1)\alpha}{2})}{\sin(\frac{\alpha}{2})}.
\label{gen_sum}
\end{equation}
By plugging in $\alpha=\frac{2\pi}{M};\quad\psi=\frac{2\pi}{M}(1-j)$ we get
\begin{equation}
\sum_{k=1}^{M}\cos\alpha_{jk}=0.
\end{equation}
Thus,
\begin{eqnarray}
\textit{CRB}_{\textit{TDOA,num}}&=&3c^2\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij}))=3c^2r^{-2\gamma}M^2\nonumber\\
\textit{CRB}_{\textit{TDOA,den}}&=&4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})\nonumber\\
&=&4W_e\rho r^{-3\gamma}\sum_i\sum_j\sum_k(1-\cos\alpha_{ij}-\cos\alpha_{jk}-\cos\alpha_{ki}+\cos\alpha_{ij}\cos\alpha_{jk}\nonumber\\
&&+\cos\alpha_{jk}\cos\alpha_{ki}+\cos\alpha_{ki}\cos\alpha_{ij}-\cos\alpha_{ij}\cos\alpha_{jk}\cos\alpha_{ki})\nonumber\\
\cos\alpha_{jk}\cos\alpha_{ki}&=&\frac{1}{2}\left(\cos\alpha_{ji}+\cos\left(\frac{2\pi}{M}(j+i-2k)\right)\right)\nonumber\\
\cos\alpha_{ij}\cos\alpha_{jk}\cos\alpha_{ki}&=&\cos\alpha_{ij}\cdot\frac{1}{2}\left(\cos\alpha_{ji}+\cos\left(\frac{2\pi}{M}(j+i-2k)\right)\right)\nonumber\\
&=&0.25(1+\cos(2\alpha_{ij})+\cos(2\alpha_{jk})+\cos(2\alpha_{ki})) \nonumber\\
\rightarrow \textit{CRB}_{\textit{TDOA,den}}&=&0.75\cdot 4W_e\rho r^{-3\gamma}M^3\nonumber\\
\rightarrow \textit{CRB}_{\textit{TDOA}}&=&\frac{c^2}{W_e\rho r^{-\gamma}M}
\end{eqnarray}
In comparison, the TOA CRB in this case is:
\begin{eqnarray}
\textit{CRB}_{\textit{TOA}}&=&\frac{c^2\sum_{i=1}^{M}r^{-\gamma}}{2W_e\rho\sum_{i=1}^{M}\sum_{j=1}^{M}r^{-2\gamma}\sin^2\alpha_{ij}}\nonumber\\
&=&\frac{c^2Mr^{-\gamma}}{2W_e\rho\sum_{i=1}^{M}\sum_{j=1}^{M}r^{-2\gamma}0.5(1-\cos(2\alpha_{ij}))}\nonumber\\
&=&\frac{c^2}{W_e\rho r^{-\gamma}M}
\end{eqnarray}
In other words, when the sensors are located as presented above, the transmission time estimation does not affect the source localization process itself.
The next stage is a more complicated case when there are two circles of sensors located in the same angles. In other words, there are $M$ sensors at distance $r_1$ from the source with angles $\phi_i=\frac{2\pi}{M}i$, and $M$ sensors at distance $r_2$ from the source with angles $\phi_i=\frac{2\pi}{M}i$.
For simplicity, the numerator and the denominator of TDOA CRB are dealt with separately: 
\begin{eqnarray}
\sum_{i=1}^{2M}\sum_{j=1}^{2M}D_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})&=&\sum_{i=1}^{2M}D_i^{-\gamma}\big(\sum_{j=1}^{M}D_j^{-\gamma}(1-\cos\alpha_{ij})+\sum_{j=M-1}^{2M}D_j^{-\gamma}(1-\cos\alpha_{ij})\big)\nonumber\\
&=&\sum_{i=1}^{2M}D_i^{-\gamma}\big(Mr_1^{-\gamma}+Mr_2^{-\gamma}\big)=\big(Mr_1^{-\gamma}+Mr_2^{-\gamma}\big)^2
\end{eqnarray}

\begin{eqnarray}
&&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})\nonumber\\
&=&\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})\sum_kD_k^{-\gamma}(1-\cos\alpha_{jk}-\cos\alpha_{ki}\nonumber\\
&&+0.5(\cos\alpha_{ji}+\cos(\frac{2\pi}{M}(j+i-2k))))\nonumber\\
&=&\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})(1+0.5\cos\alpha_{ji})(Mr_1^{-\gamma}+Mr_2^{-\gamma})\nonumber\\
&=&(Mr_1^{-\gamma}+Mr_2^{-\gamma})\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-0.5\cos\alpha_{ij}-0.25\cos(2\alpha_{ji})-0.25)\nonumber\\
&=&0.75(Mr_1^{-\gamma}+Mr_2^{-\gamma})^3
\end{eqnarray}
One can easily conclude that the technique of sum contribution can be done for any number of circles. In order to avoid definition problems, such as division by zero, each circle must include at least 3 sensors.\\
Thus overall, this model can be expanded to any number of circles, where in each circle the sensors are uniformly distributed, even though the angles are different in each circle. In addition, the number of sensors in each circle can be different. Thus, the sensors can be divided into $L$ groups as follows. In the $l$ group there are $M_l$ sensors located at distance $r_l$ from the source and at angles $\phi_j=\psi_l+\frac{2\pi}{M_l}j,\quad j\in[1,M_l]$. Thus, the numerator of TDOA CRB is:
\begin{eqnarray}
\textit{CRB}_{\textit{TDOA,num}}&=&3c^2\sum_iD_i^{-\gamma}\sum_{l=1}^L\sum_{j=1}^{M_l}D_j^{-\gamma}(1-\cos(\alpha_{ij}))=3c^2\sum_iD_i^{-\gamma}\sum_{l=1}^L(M_lr_l^{-\gamma})\nonumber\\
&=&3c^2\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)^2
\end{eqnarray}
In the previous steps of the formula (\ref{gen_sum}) was used separately for each group. Similarly, the denominator is:
\begin{eqnarray}
&&\textit{CRB}_{\textit{TDOA,den}}=4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})\nonumber\\
&=&4W_e\rho\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})\sum_{l=1}^L\sum_{k=1}^{M_l}D_k^{-\gamma}\Bigg(1-\cos\alpha_{jk}-\cos\alpha_{ki}\nonumber\\
&&\left.+0.5\left(\cos\alpha_{ji}+\cos\left(\frac{2\pi}{M}(j+i-2k)\right)\right)\right)\nonumber\\
&=&4W_e\rho\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})(1+0.5\cos\alpha_{ji})\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)\nonumber\\
&=&4W_e\rho\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(0.75-0.5\cos\alpha_{ij}-0.25\cos(2\alpha_{ji}))\nonumber\\
&=&3W_e\rho\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)^3
\end{eqnarray}
Combining the two last results yields
\begin{equation}
\textit{CRB}_{\textit{TDOA}}=\frac{c^2}{W_e\rho\sum_{l=1}^LM_lr_l^{-\gamma}}
\end{equation}
It is easy to prove that it equals $\textit{CRB}_{\textit{TOA}}$ in the same configuration.\\
The formula above can be extended to more the general condition for TOA and TDOA CRBs equality. For any configuration that can be divided into groups of sensors, so that all the $M_l$ sensors in the group are located at the same distance from the source and the following condition exists:
\begin{equation}
\sum_{k=1}^{M_l}\cos\alpha_{jk}=0.
\end{equation}
for every $j$ out of the group, the TDOA CRB equals the TOA CRB of the configuration.

==> Chapters/insight1UAA_after_itsik.tex <==
One interesting insight related to the explicit shape of the TDOA CRB explicit shape, is finding the conditions or even situations when the TOA CRB (which is taken from \cite{YnoamIbergelTOA}\footnote{In \cite{YnoamIbergelTOA} the CRB is developed for TOA-RSS case, but the derivation contains two seperate parts: one part belongs to TOA estimation and the other part belongs to RSS estimation. Thus, the CRB for TOA estimation can be easily concluded from this article by using only the TOA part in the derivation.}) equals the TDOA CRB. In other words, the conditions when knowledge of the transmission time $T_0$ has no influence on the quality of the asymptotic estimation. First, the expressions for both TOA CRB and TDOA CRB are given below:
\begin{eqnarray}
\textit{CRB}_{\textit{TDOA}}=\frac{3c^2\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij})) }{4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})}.\nonumber\\
&&
\end{eqnarray}
\begin{equation}
\textit{CRB}_{\textit{TOA}}=\frac{c^2\sum_{i=1}^{M}D_i^{-\gamma}}{2W_e\rho\sum_{i=1}^{M}\sum_{j=1}^{M}D_i^{-\gamma}D_j^{-\gamma}\sin^2\alpha_{ij}}
\end{equation}
A basic but interesting configuration that should be verified is a UAA network.
\begin{definition}A Uniform angular array (UAA) of sensors is a set of $3$ or more sensors that have the same amplitude $A_m$ and are located in uniform intervals over a circle around the source\footnote{This placement is problematic, as we do not know the source location prior to the placement of the sensors. Yet, it is an interesting scenario that gives much insight on the performance.}. That is, the angle difference between nearby sensors is $2\pi$ divided by the number of sensors in the array.
\end{definition}
\begin{definition}A UAA network is a network of sensors that is composed of $K\ge 1$ UAAs, where the $k$-th UAA has $M_k$ sensors each with amplitude $A_k$, where all UAAs are centered at the source location. (Examples of UAA networks are illustrated in Fig. \ref{fig:uaa_confs}.)
\end{definition}

\begin{corrolary}\label{CRB_UAA}
	The CRB of a UAA network is given by:
	\begin{equation}
	\textrm{CRB}=\frac{c^2}{W_e\rho\sum_k M_k A_k}
	\label{crbuaa}
	\end{equation}
\end{corrolary}
\begin{IEEEproof}
In this section, the following formula will be used frequently:
\begin{equation}
\sum_{n=0}^{M-1}\cos(\psi+n\alpha)=\frac{\sin(\frac{M\alpha}{2})\cos(\psi+\frac{(M-1)\alpha}{2})}{\sin(\frac{\alpha}{2})}.
\label{gen_sum}
\end{equation}
By plugging in $\alpha=\frac{2\pi}{M};\quad\psi=\frac{2\pi}{M}(1-j)$ we get
\begin{equation}
\sum_{k=1}^{M}\cos\alpha_{jk}=0.
\end{equation}
Thus,
\begin{eqnarray}
\textit{CRB}_{\textit{TDOA,num}}&=&3c^2\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij}))=3c^2r^{-2\gamma}M^2\nonumber\\
\textit{CRB}_{\textit{TDOA,den}}&=&4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})\nonumber\\
&=&4W_e\rho r^{-3\gamma}\sum_i\sum_j\sum_k(1-\cos\alpha_{ij}-\cos\alpha_{jk}-\cos\alpha_{ki}+\cos\alpha_{ij}\cos\alpha_{jk}\nonumber\\
&&+\cos\alpha_{jk}\cos\alpha_{ki}+\cos\alpha_{ki}\cos\alpha_{ij}-\cos\alpha_{ij}\cos\alpha_{jk}\cos\alpha_{ki})\nonumber\\
\cos\alpha_{jk}\cos\alpha_{ki}&=&\frac{1}{2}\left(\cos\alpha_{ji}+\cos\left(\frac{2\pi}{M}(j+i-2k)\right)\right)\nonumber\\
\cos\alpha_{ij}\cos\alpha_{jk}\cos\alpha_{ki}&=&\cos\alpha_{ij}\cdot\frac{1}{2}\left(\cos\alpha_{ji}+\cos\left(\frac{2\pi}{M}(j+i-2k)\right)\right)\nonumber\\
&=&0.25(1+\cos(2\alpha_{ij})+\cos(2\alpha_{jk})+\cos(2\alpha_{ki})) \nonumber\\
\rightarrow \textit{CRB}_{\textit{TDOA,den}}&=&0.75\cdot 4W_e\rho r^{-3\gamma}M^3\nonumber\\
\rightarrow \textit{CRB}_{\textit{TDOA}}&=&\frac{c^2}{W_e\rho r^{-\gamma}M}
\end{eqnarray}
In comparison, the TOA CRB in this case is:
\begin{eqnarray}
\textit{CRB}_{\textit{TOA}}&=&\frac{c^2\sum_{i=1}^{M}r^{-\gamma}}{2W_e\rho\sum_{i=1}^{M}\sum_{j=1}^{M}r^{-2\gamma}\sin^2\alpha_{ij}}\nonumber\\
&=&\frac{c^2Mr^{-\gamma}}{2W_e\rho\sum_{i=1}^{M}\sum_{j=1}^{M}r^{-2\gamma}0.5(1-\cos(2\alpha_{ij}))}\nonumber\\
&=&\frac{c^2}{W_e\rho r^{-\gamma}M}
\end{eqnarray}
In other words, when the sensors are located as presented above, the transmission time estimation does not affect the source localization process itself.
The next stage is a more complicated case when there are two circles of sensors located in the same angles. In other words, there are $M$ sensors at distance $r_1$ from the source with angles $\phi_i=\frac{2\pi}{M}i$, and $M$ sensors at distance $r_2$ from the source with angles $\phi_i=\frac{2\pi}{M}i$.
For simplicity, the numerator and the denominator of TDOA CRB are dealt with separately: 
\begin{eqnarray}
\sum_{i=1}^{2M}\sum_{j=1}^{2M}D_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})&=&\sum_{i=1}^{2M}D_i^{-\gamma}\left(\sum_{j=1}^{M}D_j^{-\gamma}(1-\cos\alpha_{ij})+\sum_{j=M-1}^{2M}D_j^{-\gamma}(1-\cos\alpha_{ij})\right)\nonumber\\
&=&\sum_{i=1}^{2M}D_i^{-\gamma}\big(Mr_1^{-\gamma}+Mr_2^{-\gamma}\big)=\big(Mr_1^{-\gamma}+Mr_2^{-\gamma}\big)^2
\end{eqnarray}

\begin{eqnarray}
&&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})\nonumber\\
&=&\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})\sum_kD_k^{-\gamma}(1-\cos\alpha_{jk}-\cos\alpha_{ki}\nonumber\\
&&+0.5(\cos\alpha_{ji}+\cos(\frac{2\pi}{M}(j+i-2k))))\nonumber\\
&=&\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})(1+0.5\cos\alpha_{ji})(Mr_1^{-\gamma}+Mr_2^{-\gamma})\nonumber\\
&=&(Mr_1^{-\gamma}+Mr_2^{-\gamma})\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-0.5\cos\alpha_{ij}-0.25\cos(2\alpha_{ji})-0.25)\nonumber\\
&=&0.75(Mr_1^{-\gamma}+Mr_2^{-\gamma})^3
\end{eqnarray}
One can easily conclude that the technique of sum contribution can be done for any number of circles. In order to avoid definition problems, such as division by zero, each circle must include at least 3 sensors.\\
Thus overall, this model can be expanded to any number of circles, where in each circle the sensors are uniformly distributed, even though the angles are different in each circle. In addition, the number of sensors in each circle can be different. Thus, the sensors can be divided into $L$ groups as follows. In the $l$ group there are $M_l$ sensors located at distance $r_l$ from the source and at angles $\phi_j=\psi_l+\frac{2\pi}{M_l}j,\quad j\in[1,M_l]$. Thus, the numerator of TDOA CRB is:
\begin{eqnarray}
\textit{CRB}_{\textit{TDOA,num}}&=&3c^2\sum_iD_i^{-\gamma}\sum_{l=1}^L\sum_{j=1}^{M_l}D_j^{-\gamma}(1-\cos(\alpha_{ij}))=3c^2\sum_iD_i^{-\gamma}\sum_{l=1}^L(M_lr_l^{-\gamma})\nonumber\\
&=&3c^2\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)^2
\end{eqnarray}
In the previous steps of the formula (\ref{gen_sum}) was used separately for each group. Similarly, the denominator is:
\begin{eqnarray}
&&\textit{CRB}_{\textit{TDOA,den}}=4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})\nonumber\\
&=&4W_e\rho\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})\sum_{l=1}^L\sum_{k=1}^{M_l}D_k^{-\gamma}\Bigg(1-\cos\alpha_{jk}-\cos\alpha_{ki}\nonumber\\
&&\left.+0.5\left(\cos\alpha_{ji}+\cos\left(\frac{2\pi}{M}(j+i-2k)\right)\right)\right)\nonumber\\
&=&4W_e\rho\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})(1+0.5\cos\alpha_{ji})\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)\nonumber\\
&=&4W_e\rho\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(0.75-0.5\cos\alpha_{ij}-0.25\cos(2\alpha_{ji}))\nonumber\\
&=&3W_e\rho\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)^3
\end{eqnarray}
Combining the two last results yields
\begin{equation}
\textit{CRB}_{\textit{TDOA}}=\frac{c^2}{W_e\rho\sum_{l=1}^LM_lr_l^{-\gamma}}
\end{equation}
It is easy to prove that it equals $\textit{CRB}_{\textit{TOA}}$ in the same configuration.
\end{IEEEproof}
The formula above can be extended to more the general condition for TOA and TDOA CRBs equality. For any configuration that can be divided into groups of sensors, so that all the $M_l$ sensors in the group are located at the same distance from the source and the following condition exists:
\begin{equation}
\sum_{k=1}^{M_l}\cos\alpha_{jk}=0.
\end{equation}
for every $j$ out of the group, the TDOA CRB equals the TOA CRB of the configuration.

==> Chapters/insight1UAA_after_itsik_yair.tex <==
One interesting insight related to the TDOA CRB explicit shape, is finding the conditions or even situations when the TOA CRB (which is taken from \cite{YnoamIbergelTOA}\footnote{In \cite{YnoamIbergelTOA} the CRB is developed for TOA-RSS case, but the derivation contains two seperate parts: one part belongs to TOA estimation and the other part belongs to RSS estimation. Thus, the CRB for TOA estimation can be easily concluded from this article by using only the TOA part in the derivation.}) equals the TDOA CRB. In other words, the conditions when knowledge of the transmission time $T_0$ does not affect the quality of the asymptotic estimation. First, the expressions for both TOA CRB and TDOA CRB are given below:
\begin{eqnarray}
\textit{CRB}_{\textit{TDOA}}=\frac{3c^2\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij})) }{4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})}.\nonumber\\
&&
\end{eqnarray}
\begin{equation}
\textit{CRB}_{\textit{TOA}}=\frac{c^2\sum_{i=1}^{M}D_i^{-\gamma}}{2W_e\rho\sum_{i=1}^{M}\sum_{j=1}^{M}D_i^{-\gamma}D_j^{-\gamma}\sin^2\alpha_{ij}}
\end{equation}
A basic but interesting configuration that should be verified is a UAA network.
\begin{definition}A Uniform angular array (UAA) of sensors is a set of $3$ or more sensors that have the same amplitude $A_m$ and are located in uniform intervals over a circle around the source\footnote{This placement is problematic, as we do not know the source location prior to the placement of the sensors. Yet, it is an interesting scenario that gives much insight on the performance.}. That is, the angle difference between nearby sensors is $2\pi$ divided by the number of sensors in the array.
\end{definition}
\begin{definition}A UAA network is a network of sensors that is composed of $K\ge 1$ UAAs, where the $k$-th UAA has $M_k$ sensors, each with amplitude $A_k$, and all UAAs are centered at the source location. (Examples of UAA networks are illustrated in Fig. \ref{fig:uaa_confs}.)
\end{definition}

\begin{corrolary}\label{CRB_UAA}
	The CRB of a UAA network is given by:
	\begin{equation}
	\textrm{CRB}=\frac{c^2}{W_e\rho\sum_k M_k A_k}
	\label{crbuaa}
	\end{equation}
\end{corrolary}
\begin{IEEEproof}
In this section, the following formula will be used frequently:
\begin{equation}
\sum_{n=0}^{M-1}\cos(\psi+n\alpha)=\frac{\sin(\frac{M\alpha}{2})\cos(\psi+\frac{(M-1)\alpha}{2})}{\sin(\frac{\alpha}{2})}.
\label{gen_sum}
\end{equation}
By plugging in $\alpha=\frac{2\pi}{M};\quad\psi=\frac{2\pi}{M}(1-j)$ we get
\begin{equation}
\sum_{k=1}^{M}\cos\alpha_{jk}=0.
\end{equation}
Thus,
\begin{eqnarray}
\textit{CRB}_{\textit{TDOA,num}}&=&3c^2\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos(\alpha_{ij}))=3c^2r^{-2\gamma}M^2\nonumber\\
\textit{CRB}_{\textit{TDOA,den}}&=&4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})\nonumber\\
&=&4W_e\rho r^{-3\gamma}\sum_i\sum_j\sum_k(1-\cos\alpha_{ij}-\cos\alpha_{jk}-\cos\alpha_{ki}+\cos\alpha_{ij}\cos\alpha_{jk}\nonumber\\
&&+\cos\alpha_{jk}\cos\alpha_{ki}+\cos\alpha_{ki}\cos\alpha_{ij}-\cos\alpha_{ij}\cos\alpha_{jk}\cos\alpha_{ki})\nonumber\\
\cos\alpha_{jk}\cos\alpha_{ki}&=&\frac{1}{2}\left(\cos\alpha_{ji}+\cos\left(\frac{2\pi}{M}(j+i-2k)\right)\right)\nonumber\\
\cos\alpha_{ij}\cos\alpha_{jk}\cos\alpha_{ki}&=&\cos\alpha_{ij}\cdot\frac{1}{2}\left(\cos\alpha_{ji}+\cos\left(\frac{2\pi}{M}(j+i-2k)\right)\right)\nonumber\\
&=&0.25(1+\cos(2\alpha_{ij})+\cos(2\alpha_{jk})+\cos(2\alpha_{ki})) \nonumber\\
\rightarrow \textit{CRB}_{\textit{TDOA,den}}&=&0.75\cdot 4W_e\rho r^{-3\gamma}M^3\nonumber\\
\rightarrow \textit{CRB}_{\textit{TDOA}}&=&\frac{c^2}{W_e\rho r^{-\gamma}M}
\end{eqnarray}
In comparison, the TOA CRB in this case is:
\begin{eqnarray}
\textit{CRB}_{\textit{TOA}}&=&\frac{c^2\sum_{i=1}^{M}r^{-\gamma}}{2W_e\rho\sum_{i=1}^{M}\sum_{j=1}^{M}r^{-2\gamma}\sin^2\alpha_{ij}}\nonumber\\
&=&\frac{c^2Mr^{-\gamma}}{2W_e\rho\sum_{i=1}^{M}\sum_{j=1}^{M}r^{-2\gamma}0.5(1-\cos(2\alpha_{ij}))}\nonumber\\
&=&\frac{c^2}{W_e\rho r^{-\gamma}M}
\end{eqnarray}
In other words, when the sensors are located as presented above, the transmission time estimation does not affect the source localization process itself.
The next stage is a more complicated case when there are two circles of sensors located in the same angles. In other words, there are $M$ sensors at distance $r_1$ from the source with angles $\phi_i=\frac{2\pi}{M}i$, and $M$ sensors at distance $r_2$ from the source with angles $\phi_i=\frac{2\pi}{M}i$.
For simplicity, the numerator and the denominator of TDOA CRB are dealt with separately: 
\begin{eqnarray}
\sum_{i=1}^{2M}\sum_{j=1}^{2M}D_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})&=&\sum_{i=1}^{2M}D_i^{-\gamma}\left(\sum_{j=1}^{M}D_j^{-\gamma}(1-\cos\alpha_{ij})+\sum_{j=M-1}^{2M}D_j^{-\gamma}(1-\cos\alpha_{ij})\right)\nonumber\\
&=&\sum_{i=1}^{2M}D_i^{-\gamma}\big(Mr_1^{-\gamma}+Mr_2^{-\gamma}\big)=\big(Mr_1^{-\gamma}+Mr_2^{-\gamma}\big)^2
\end{eqnarray}

\begin{eqnarray}
&&\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})\nonumber\\
&&=\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})\sum_kD_k^{-\gamma}(1-\cos\alpha_{jk}-\cos\alpha_{ki}\nonumber\\
&&\quad+0.5(\cos\alpha_{ji}+\cos(\frac{2\pi}{M}(j+i-2k))))\nonumber\\
&&=\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})(1+0.5\cos\alpha_{ji})(Mr_1^{-\gamma}+Mr_2^{-\gamma})\nonumber\\
&&=(Mr_1^{-\gamma}+Mr_2^{-\gamma})\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-0.5\cos\alpha_{ij}-0.25\cos(2\alpha_{ji})-0.25)\nonumber\\
&&=0.75(Mr_1^{-\gamma}+Mr_2^{-\gamma})^3
\end{eqnarray}
One can easily conclude that the technique of sum contribution can be done for any number of circles. In order to avoid definition problems, such as division by zero, each circle must include at least 3 sensors.\\
Thus, this model can be extended to any number of circles, where in each circle the sensors are uniformly distributed, even though the angles are different in each circle. In addition, the number of sensors in each circle can be different. Thus, the sensors can be divided into $L$ groups as follows. In the $l$ group there are $M_l$ sensors located at distance $r_l$ from the source and at angles $\phi_j=\psi_l+\frac{2\pi}{M_l}j,\quad j\in[1,M_l]$. An example of UAA network with three UAAs is illustrated in Fig. $\ref{fig:3UAA_NET}$.
\begin{figure}
	\centering
	\includegraphics[width=0.7\textwidth]{3UAA_NET}
	\caption{Three UAAs Configuration}
	\label{fig:3UAA_NET} 
\end{figure}

Thus, the numerator of TDOA CRB is:
\begin{eqnarray}
\textit{CRB}_{\textit{TDOA,num}}&=&3c^2\sum_iD_i^{-\gamma}\sum_{l=1}^L\sum_{j=1}^{M_l}D_j^{-\gamma}(1-\cos(\alpha_{ij}))=3c^2\sum_iD_i^{-\gamma}\sum_{l=1}^L(M_lr_l^{-\gamma})\nonumber\\
&=&3c^2\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)^2
\end{eqnarray}
In the previous steps of the formula (\ref{gen_sum}) was used separately for each group. Similarly, the denominator is:
\begin{eqnarray}
&&\textit{CRB}_{\textit{TDOA,den}}=4W_e\rho\sum_i\sum_j\sum_kD_i^{-\gamma}D_j^{-\gamma}D_k^{-\gamma}(1-\cos\alpha_{ij})(1-\cos\alpha_{jk})(1-\cos\alpha_{ki})\nonumber\\
&=&4W_e\rho\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})\sum_{l=1}^L\sum_{k=1}^{M_l}D_k^{-\gamma}\Bigg(1-\cos\alpha_{jk}-\cos\alpha_{ki}\nonumber\\
&&\left.+0.5\left(\cos\alpha_{ji}+\cos\left(\frac{2\pi}{M}(j+i-2k)\right)\right)\right)\nonumber\\
&=&4W_e\rho\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(1-\cos\alpha_{ij})(1+0.5\cos\alpha_{ji})\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)\nonumber\\
&=&4W_e\rho\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)\sum_i\sum_jD_i^{-\gamma}D_j^{-\gamma}(0.75-0.5\cos\alpha_{ij}-0.25\cos(2\alpha_{ji}))\nonumber\\
&=&3W_e\rho\left(\sum_{l=1}^LM_lr_l^{-\gamma}\right)^3
\end{eqnarray}
Combining the two last results yields
\begin{equation}
\textit{CRB}_{\textit{TDOA}}=\frac{c^2}{W_e\rho\sum_{l=1}^LM_lr_l^{-\gamma}}
\end{equation}
It is easy to prove that it equals $\textit{CRB}_{\textit{TOA}}$ in the same configuration.
\end{IEEEproof}
The formula above can be extended to more the general condition for TOA and TDOA CRBs equality. For any configuration that can be divided into groups of sensors, so that all the $M_l$ sensors in the group are located at the same distance from the source and the following condition exists:
\begin{equation}
\sum_{k=1}^{M_l}\cos\alpha_{jk}=0.
\end{equation}
for every $j$ out of the group, the TDOA CRB equals the TOA CRB of the configuration.

==> Chapters/insight2compModels.tex <==
Another insight from the  explicit shape of the TDOA CRB involves the comparison between our model and two very similar ones:
\begin{enumerate}
	\item The case where the received signal amplitudes are unknown at the fusion center and are estimated as nuisance parameters. 
	
	\item The case of RSS TDOA estimation; i.e., the amplitudes are derived directly from the distance estimation. 
\end{enumerate} 
In these cases, the prime comparison technique is comparing certain parts of the different FIMs.\\
In order to compare the first case and our model, its FIM is discussed now. This FIM can be presented as a block matrix:
\begin{eqnarray}
I_1=\begin{pmatrix}
I_{1,11}&I_{1,12}\\
I_{1,21}&I_{1,22}\\
\end{pmatrix}
\end{eqnarray} 
where $I_{{1,11}_{3\times3}}$ is the FIM of the original case, $I_{1,12}=I_{1,21}^T$ contains the expectation of the mixed derivations due to the amplitude and due to the original parameters from $\{x,y,T_0\}$, and $I_{1,22}$ is the FIM of the amplitudes themselves. A requisite step is to calculate some typical elements of $I_1$, where the interesting correlations are $T_0\leftrightarrow A_m$ and $x\leftrightarrow A_m$. The correlation $y\leftrightarrow A_m$ is symmetric to $x\leftrightarrow A_m$ and hence will not be examined. First, one can easily conclude that derivating the whole log-likelihood according to $A_m$ is the equivalent of only deriving the $m$ log-likelihood target:
\begin{equation}
\frac{\partial \log f(r_m;\theta)}{\partial A_m}=\frac{2}{N_0}\int_{0}^{\infty}s(t-\tau_m(\theta))r_m(t)dt-\frac{2}{N_0}\int_{0}^{\infty}A_ms^2(t-\tau_m(\theta))dt
\label{first_der}
\end{equation}
In order to derive the FIM elements, (\ref{first_der}) needs to be derived again according to the relevant parameter and be expectated:
\begin{eqnarray}
&&\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial T_0}=-\frac{2}{N_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))r_m(t)dt+\frac{4}{N_0}\int_{0}^{\infty}A_ms(t-\tau_m(\theta))\dot{s}(t-\tau_m(\theta))dt\nonumber\\
&&=-\frac{2}{N_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))[r_m(t)-2A_ms(t-\tau_m(\theta))]dt\nonumber\\
&&\rightarrow {\mathbb E}\left(\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial T_0}|\theta\right)=\frac{2}{N_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))A_ms(t-\tau_m(\theta))dt=0\nonumber\\
&&\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial x}=-\frac{2}{cN_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))r_m(t)\cos\phi_mdt\nonumber\\
&&+\frac{4}{cN_0}\int_{0}^{\infty}A_ms(t-\tau_m(\theta))\dot{s}(t-\tau_m(\theta))\cos\phi_mdt\nonumber\\
&&=-\frac{2\cos\phi_m}{cN_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))[r_m(t)-2A_ms(t-\tau_m(\theta))]dt\nonumber\\
&&\rightarrow {\mathbb E}\left(\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial x}|\theta\right)=\frac{2\cos\phi_m}{cN_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))A_ms(t-\tau_m(\theta))dt=0
\end{eqnarray}
where $\tau_m=D_m/c+T_0$. After calculation of the off-diagonal elements, one typical element from $I_{1,22}$ is calculated:
\begin{eqnarray}
&&\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial A_n}=-\frac{2}{N_0}\int_{0}^{\infty}s^2(t-\tau_m(\theta))dt \times \delta(m,n)\nonumber\\
&&\rightarrow {\mathbb E}\left(\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial A_n}|\theta\right)=-\frac{2E_sD_m^{-\gamma}}{N_0} \delta(m,n)\nonumber\\
\end{eqnarray}
In other words, $I_{1,12}=I_{1,21}^T$ are zero matrices and $I_{1,22}$ is a diagonal matrix. The latter results are almost obvious and predictable, because there should be no connection between two different aplitude estimations. The former results, in contrast, are a little bit surprising. At first glance, the amplitude estimation has some affect on the estimation of the source location, or on the estimated transmission time. This suggests that the amplitudes' estimators converge much faster than the estimation of the source location or the transmission time, as explained above. However, in the asymptotic situation, a convergence of this case to a known amplitudes case is expected.\par
The second highly similar situation is RSS-TDOA estimation, when all the information in the received signal about the source is considered. In the RSS-TDOA assumption, the received signal is modeled as:
\begin{equation}
r_m(t)=k_0D_m^{-\gamma/2}s(t-D_m/c-T_0)+v_m(t)=s_m(t)+v_m(t).
\label{signal}
\end{equation} 
In other words, information about the density between the source and the sensor exists in both the sensor's amplitude and its time delay. Usually, this is the most realistic description of the received signal, but the most complicated to work with. Thus, we will be satisfied with stating that the MSE for this case must be equal to or less than the MSE for case of known amplitudes, since the estimator utilizes more information.


==> Chapters/insight2compModels_after_itsik.tex <==
Another insight from the  explicit shape of the TDOA CRB involves the comparison between our model and two very similar ones:
\begin{enumerate}
	\item The case where the received signal amplitudes are unknown at the fusion center and are estimated as nuisance parameters. 
	
	\item The case of RSS TDOA estimation; i.e., the amplitudes are derived directly from the distance estimation. 
\end{enumerate} 
In these cases, the prime comparison technique is comparing certain parts of the different FIMs.\\
In order to compare the first case and our model, its FIM is discussed now. This FIM can be presented as a block matrix:
\begin{eqnarray}
I_1=\begin{pmatrix}
I_{1,11}&I_{1,12}\\
I_{1,21}&I_{1,22}\\
\end{pmatrix}
\end{eqnarray} 
where $I_{{1,11}_{3\times3}}$ is the FIM of the original case, $I_{1,12}=I_{1,21}^T$ contains the expectation of the mixed derivations due to the amplitude and due to the original parameters from $\{x,y,T_0\}$, and $I_{1,22}$ is the FIM of the amplitudes themselves.\\ 
A requisite step is to calculate some typical elements of $I_1$, where the interesting correlations are $T_0\leftrightarrow A_m$ and $x\leftrightarrow A_m$. The correlation $y\leftrightarrow A_m$ is symmetric to $x\leftrightarrow A_m$ and hence will not be examined. \\
First, one can easily conclude that derivating the whole log-likelihood with respect to $A_m$ is equivalent to only deriving the $m$ log-likelihood target:
\begin{equation}
\frac{\partial \log f(r_m;\theta)}{\partial A_m}=\frac{2}{N_0}\int_{0}^{\infty}s(t-\tau_m(\theta))r_m(t)dt-\frac{2}{N_0}\int_{0}^{\infty}A_ms^2(t-\tau_m(\theta))dt
\label{first_der}
\end{equation}
In order to derive the FIM elements, (\ref{first_der}) needs to be derived again according to the relevant parameter and be expectated:
\begin{eqnarray}
&&\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial T_0}=-\frac{2}{N_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))r_m(t)dt+\frac{4}{N_0}\int_{0}^{\infty}A_ms(t-\tau_m(\theta))\dot{s}(t-\tau_m(\theta))dt\nonumber\\
&&=-\frac{2}{N_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))[r_m(t)-2A_ms(t-\tau_m(\theta))]dt\nonumber\\
&&\rightarrow {\mathbb E}\left(\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial T_0}|\theta\right)=\frac{2}{N_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))A_ms(t-\tau_m(\theta))dt=0\nonumber\\
&&\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial x}=-\frac{2}{cN_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))r_m(t)\cos\phi_mdt\nonumber\\
&&+\frac{4}{cN_0}\int_{0}^{\infty}A_ms(t-\tau_m(\theta))\dot{s}(t-\tau_m(\theta))\cos\phi_mdt\nonumber\\
&&=-\frac{2\cos\phi_m}{cN_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))[r_m(t)-2A_ms(t-\tau_m(\theta))]dt\nonumber\\
&&\rightarrow {\mathbb E}\left(\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial x}|\theta\right)=\frac{2\cos\phi_m}{cN_0}\int_{0}^{\infty}\dot{s}(t-\tau_m(\theta))A_ms(t-\tau_m(\theta))dt=0
\end{eqnarray}
where $\tau_m=D_m/c+T_0$. After calculation of the off-diagonal elements, one typical element from $I_{1,22}$ is calculated:
\begin{eqnarray}
&&\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial A_n}=-\frac{2}{N_0}\int_{0}^{\infty}s^2(t-\tau_m(\theta))dt \times \delta(m,n)\nonumber\\
&&\rightarrow {\mathbb E}\left(\frac{\partial^2 \log f(r_m;\theta)}{\partial A_m\partial A_n}|\theta\right)=-\frac{2E_sD_m^{-\gamma}}{N_0} \delta(m,n)\nonumber\\
\end{eqnarray}
In other words, $I_{1,12}=I_{1,21}^T$ are zero matrices and $I_{1,22}$ is a diagonal matrix. \\
The latter results are almost obvious and predictable, because there should be no connection between two different aplitude estimations. The former results, in contrast, are a little bit surprising. \\
At first glance, the amplitude estimation has some affect on the estimation of the source location, or on the estimated transmission time. This suggests that the amplitudes' estimators converge much faster than the estimation of the source location or the transmission time, as explained above. However, in the asymptotic situation, a convergence of this case to a known amplitudes case is expected.\par
The second highly similar situation is RSS-TDOA estimation, when all the information in the received signal about the source is considered. In the RSS-TDOA assumption, the received signal is modeled as:
\begin{equation}
r_m(t)=k_0D_m^{-\gamma/2}s(t-D_m/c-T_0)+v_m(t)=s_m(t)+v_m(t).
\label{signal}
\end{equation} 
In other words, information about the distance from the source to the sensor exists in both the sensor's amplitude and its time delay. Usually, this is the most realistic description of the received signal, but the most complicated to work with. Thus, we will be satisfied with stating that the MSE for this case must be equal to or less than the MSE for case of known amplitudes, since the estimator utilizes more information.


==> Chapters/introduction.tex <==
\hypersetup{
	colorlinks   = true, %Colours links instead of ugly boxes
	urlcolor     = black, %Colour for external hyperlinks
	linkcolor    = black, %Colour of internal links
	citecolor   = black %Colour of citations
}
Localization by sensor networks is important in many applications, such as location-based billing, personal security and safety, intelligent transportation systems, machinery monitoring, radio resource management, etc; see for example \cite{TermSelfLoc,smarts,lastilp,Caire2010Multiuser,hkoshJhosh,EnerEffe,Semantic}. 
To determine the source location, each sensor takes measurements about the source. Then, the location is estimated by a fusion center which receives the measurements from all the sensors. It typically generates time-of-arrival (TOA), time-difference-of-arrival (TDOA), angle-of-arrival (AOA), received-signal-strength (RSS), or a combination of these from the measurements\cite{myref5,myref12}\footnote{There are some reports of the frequency-difference-of-arrival (FDOA) (e.g. \cite{TDFD,geofdtd}) but this method is uncommon in the literature.}. For instance, \cite{myref1} compares between TOA and TDOA and presents a matrix form for the Cram\'{e}r-Rao Bound (CRB), which is a lower bound for the estimator variance, as discussed in detail below. Common combinations are TOA-RSS or TDOA-RSS, due to the fact that both RSS and TDOA or TOA measure distance as a middle step toward source localization, but from different parts of the signal. Thus, the integrations produce all the information about the distance from the signal. One example of this combination is \cite{HybDis}. All these types of measurements have been explored in different conditions, and under a variety of assumptions \cite{myref5,myref6,myref9,myref10,myref13}.  For example,  in \cite{myref5} the authors deal with TDOA source estimation in the far field limit. Using prolate spheroidal coordinates, the TDOA equation set becomes linear and hence can be solved analytically as an intersection of hyperbolic asymptotes. Quazi \cite{myref6} explores the effects of signal constants (such as bandwidth and center frequency) on the CRB in time delay estimation. Low SNR is assumed, and both active and passive systems are examined. In the suggested formulation, the noise appears in the time delay estimation, not in the signal receiving process, although the latter would appear to be a more natural description. The non-line-of-sight situation, when there is no straight path from the source to the sensor and the sensor only receives the sent signal's reflection, is discussed extensively in \cite{myref13}, with respect to almost every estimation method. Methods have considered different parts of the whole signal, or make different assumptions about the received signal and the sensors' output, as explained in detail in the next section. 
Currently, there is no closed-form CRB for TDOA localization with sensors of non-identical SNR. In this thesis we derive a closed-form expression for the CRB on the mean square error in TDOA localization. This bound is presented in Theorem \ref{CRBlast} in the form of a division of sums, and it is very easy to evaluate for any sensor constellation. We also use this bound to study the performance in sensor constellations that consists of concentric uniform angular arrays (UAA), which are known to optimize the localization accuracy. We show that for these special constellations, the CRB for TDOA localization coincides with the CRB for TOA localization. Thus, in these constellations, prior knowledge of the transmission time does not improve localization performance in the asymptotic regime. \par

The thesis is organized as follows. The problem is formulated in Sec. \ref{Sec:PorblemFormulation}, which includes
the signal model, assumptions about the system , and the unknown parameters.
In Sec. \ref{chap:derivation}, we derive the CRB for TDOA source localization and discuss some interesting insights about it. The simulation results for the proposed CRB
are presented in Sec. \ref{chap:results}. The summary and conclusions appear in Sec. \ref{chap:conclusions}.

==> Chapters/introduction_after_yair.tex <==
\hypersetup{
	colorlinks   = true, %Colours links instead of ugly boxes
	urlcolor     = black, %Colour for external hyperlinks
	linkcolor    = black, %Colour of internal links
	citecolor   = black %Colour of citations
}
Localization by sensor networks is important in many applications, such as location-based billing, personal security and safety, intelligent transportation systems, machinery monitoring, radio resource management, etc; see for example \cite{TermSelfLoc,smarts,lastilp,Caire2010Multiuser,hkoshJhosh,EnerEffe,Semantic}. 
To determine the source location, each sensor takes measurements about the source. Then, the location is estimated by a fusion center which receives the measurements from all the sensors. It typically generates time-of-arrival (TOA), time-difference-of-arrival (TDOA), angle-of-arrival (AOA), received-signal-strength (RSS), or a combination of these from the measurements\cite{myref5,myref12}\footnote{There are some reports of the frequency-difference-of-arrival (FDOA) (e.g. \cite{TDFD,geofdtd}) but this method is uncommon in the literature.}. For instance, \cite{myref1} compares between TOA and TDOA and presents a matrix form for the Cram\'{e}r-Rao Bound (CRB), which is a lower bound for the estimation error of unbiased estimates, as discussed in detail below. Common combinations are TOA-RSS or TDOA-RSS, due to the fact that both RSS and TDOA or TOA measure distance as an intermediate step toward source localization, using different signal components. Thus, the integrations extract all the information about the distance out of the signal. An example of this combination can be found in \cite{HybDis}. All these types of measurements have been explored in different conditions, and under a variety of assumptions \cite{myref5,myref6,myref9,myref10,myref13}.  For example,  \cite{myref5} deals with TDOA source estimation in the far field limit. Using prolate spheroidal coordinates, the TDOA equation set becomes linear and hence can be solved analytically as an intersection of hyperbolic asymptotes. Quazi \cite{myref6} explores the effects of signal, such as bandwidth and carrier frequency, on the CRB for time delay estimation. Low SNR is assumed, and both active and passive systems are examined. In the suggested formulation, the noise appears in the time delay estimation, not in the signal receiving process, although the latter would appear to be a more natural description. The non-line-of-sight situation, when there is no straight path from the source to the sensor and the sensor only receives signal reflections, is discussed extensively in \cite{myref13}, with respect to numerous estimation methods, which differ in the assumptions made, or the signal component which is utilized and the sensors' output, as explained in detail in the next section. 
Currently, there is no closed-form expression of the CRB for TDOA localization with sensors with non-identical SNR. Such a closed-form expression is derived in this thesis (cf. Theorem \ref{CRBlast}) and is very easy to evaluate for any sensor constellation. We also use this bound to study the localization performance using sensor constellations that consists of concentric uniform angular arrays (UAA), which are known to optimize the localization accuracy. We show that for these special constellations, the CRB for TDOA localization coincides with the CRB for TOA localization. Thus, in these constellations, prior knowledge of the transmission time does not improve localization performance in the asymptotic regime. \par

The thesis is organized as follows. The problem is formulated in Sec. \ref{Sec:PorblemFormulation}, which includes
the signal model, assumptions about the system , and the unknown parameters.
In Sec. \ref{chap:derivation}, we derive the CRB for TDOA source localization and discuss some interesting insights about it. The simulation results for the proposed CRB
are presented in Sec. \ref{chap:results}. The summary and conclusions appear in Sec. \ref{chap:conclusions}.

==> Chapters/myshorts.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% macros by Amir

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{assumption}{Assumption}
%\newtheorem{ObservonConstraint}{Observation  Constraint}
%\newtheorem{OC}{Comment}
%\newtheorem{Comment}{Comment}
%%\newtheorem{}{Comment}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{observation}[theorem]{Observation}

%\theoremstyle{definition}
\newtheorem{definition}{Definition}
%\theoremstyle{remark}
\newcommand{\SINR}{{\rm SINR}_i\left(k, \vp\right)}
\newcommand{\SINRnu}{{\rm SINR}_i\left(k, \vp^\nu\right)}
\newcommand{\va}{\mbox{${\bf a}$}}
\newcommand{\vah}{\mbox{${\bf \hat a}$}}
\newcommand{\vat}{\mbox{${\bf \tilde a}$}}
\newcommand{\vb}{\mbox{${\bf b}$}}
\newcommand{\vp}{\mbox{${\bf p}$}}
\newcommand{\vd}{\mbox{${\bf d}$}}
\newcommand{\rh}{\mbox{${\hat r}$}}
\newcommand{\Var}{{\rm Var}}
\newcommand{\vx}{\mbox{${\bf x}$}}
\newcommand{\vxt}{\mbox{${\bf \tilde x}$}}
\newcommand{\vh}{\mbox{${\bf h}$}}
\newcommand{\htld}{\mbox{${\tilde h}$}}
\newcommand{\vhh}{\mbox{${\bf \hat h}$}}
\newcommand{\hhat}{\mbox{${\hat h}$}}
\newcommand{\ve}{\mbox{${\bf e}$}}
\newcommand{\vg}{\mbox{${\bf g}$}}
\newcommand{\vgh}{\mbox{${\bf \hat g}$}}
\newcommand{\vq}{\mbox{${\bf q}$}}
\newcommand{\vt}{\mbox{${\bf t}$}}
\newcommand{\vw}{\mbox{${\bf w}$}}
\newcommand{\vdw}{\mbox{${\bf dw}$}}
\newcommand{\vwh}{\mbox{${\bf \hat w}$}}
\newcommand{\wh}{\mbox{${\hat w}$}}
\newcommand{\vwt}{\mbox{${\bf \tilde w}$}}
\newcommand{\wt}{\mbox{${\tilde w}$}}
\newcommand{\vs}{\mbox{${\bf s}$}}
\newcommand{\vsh}{\mbox{${\bf \hat s}$}}
\newcommand{\vst}{\mbox{${\bf \tilde s}$}}
\newcommand{\vr}{\mbox{${\bf r}$}}
\newcommand{\vv}{\mbox{${\bf v}$}}
\newcommand{\vu}{\mbox{${\bf u}$}}
\newcommand{\vy}{\mbox{${\bf y}$}}
\newcommand{\vz}{\mbox{${\bf z}$}}
\newcommand{\vn}{\mbox{${\bf n}$}}
\newcommand{\vnt}{\mbox{${\bf \tilde n}$}}
\newcommand{\ntld}{\mbox{${\tilde n}$}}
\newcommand{\nhat}{\mbox{${\hat n}$}}
\newcommand{\phat}{\mbox{${\hat p}$}}
\newcommand{\vzero}{\mbox{${\bf 0}$}}
\newcommand{\vone}{\mbox{${\bf 1}$}}
% abbreviations for matrices
\newcommand{\mA}{\hbox{{\bf A}}}
\newcommand{\mAh}{\mbox{${\bf \hat A}$}}
\newcommand{\mAt}{\mbox{$\bf \tilde A$}}
\newcommand{\mB}{\hbox{{\bf B}}}
\newcommand{\mBh}{\mbox{${\bf \hat B}$}}
\newcommand{\mC}{\hbox{{\bf C}}}
\newcommand{\mCh}{\mbox{${\bf \hat C}$}}
\newcommand{\mD}{\hbox{{\bf D}}}
\newcommand{\mDt}{\mbox{$\bf \tilde D$}}
\newcommand{\mE}{\hbox{{\bf E}}}
\newcommand{\mG}{\hbox{{\bf G}}}
\newcommand{\mF}{\hbox{{\bf F}}}
\newcommand{\mH}{\hbox{{\bf H}}}
\newcommand{\mHb}{\mbox{${\bf \bar H}$}}
\newcommand{\mHt}{\mbox{${\bf \tilde H}$}}
\newcommand{\mI}{\hbox{{\bf I}}}
\newcommand{\mIh}{\mbox{${\bf \hat I}$}}
\newcommand{\mN}{\hbox{{\bf N}}}
\newcommand{\mM}{\hbox{{\bf M}}}
\newcommand{\mMh}{\mbox{{$\bf \hat M$}}}
\newcommand{\mP}{\hbox{{\bf P}}}
\newcommand{\mQ}{\hbox{{\bf Q}}}
\newcommand{\mR}{\mbox{{$\bf R$}}}
\newcommand{\mRh}{\mbox{{$\bf \hat R$}}}
\newcommand{\mRt}{\mbox{{$\bf \tilde R$}}}
\newcommand{\mS}{\mbox{{$\bf S$}}}
\newcommand{\mSb}{\mbox{{$\bf \bar S$}}}
\newcommand{\mSh}{\mbox{{$\bf \hat S$}}}
\newcommand{\mSt}{\mbox{{$\bf \tilde S$}}}
\newcommand{\mT}{\mbox{{$\bf T$}}}
\newcommand{\mU}{\mbox{{$\bf U$}}}
\newcommand{\mUh}{\mbox{{$\bf \hat U$}}}
\newcommand{\mV}{\mbox{{$\bf V$}}}
\newcommand{\mVh}{\mbox{{$\bf \hat V$}}}
\newcommand{\mW}{\hbox{{\bf W}}}
\newcommand{\mWh}{\mbox{${\bf \hat W}$}}
\newcommand{\mWt}{\mbox{${\bf \tilde W}$}}
\newcommand{\mX}{\mbox{{$\bf X$}}}
\newcommand{\mY}{\mbox{{$\bf Y$}}}
\newcommand{\mZ}{\mbox{{$\bf Z$}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{array}}
\newcommand{\ena}{\end{array}}
%\newcommand{\bds}{\begin {description}}
%\newcommand{\eds}{\end {description}}
\newcommand{\bds}{\begin {itemize}}
\newcommand{\eds}{\end {itemize}}
\newcommand{\bdf}{\begin{definition}}
\newcommand{\blm}{\begin{lemma}}
\newcommand{\edf}{\end{definition}}
\newcommand{\elm}{\end{lemma}}
\newcommand{\bthm}{\begin{theorem}}
\newcommand{\ethm}{\end{theorem}}
\newcommand{\bprp}{\begin{prop}}
\newcommand{\eprp}{\end{prop}}
\newcommand{\bcl}{\begin{claim}}
\newcommand{\ecl}{\end{claim}}
\newcommand{\bcr}{\begin{coro}}
\newcommand{\ecr}{\end{coro}}
\newcommand{\bquest}{\begin{question}}
\newcommand{\equest}{\end{question}}
\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\grg}{\gamma}
\newcommand{\gd}{\delta}
\newcommand{\gre}{\varepsilon}
\newcommand{\gep}{\epsilon}
\newcommand{\gz}{\zeta}
\newcommand{\gzh}{\mbox{$ \hat \zeta$}}
\newcommand{\gh}{\eta}
\newcommand{\gth}{\theta}
\newcommand{\gi}{iota}
\newcommand{\gk}{\kappa}
\newcommand{\gl}{\lambda}
\newcommand{\gm}{\mu}
\newcommand{\gn}{\nu}
\newcommand{\gx}{\xi}
\newcommand{\gp}{\pi}
\newcommand{\gph}{\phi}
\newcommand{\gr}{\rho}
\newcommand{\gs}{\sigma}
\newcommand{\gsh}{\hat \sigma}
\newcommand{\gt}{\tau}
\newcommand{\gu}{\upsilon}
\newcommand{\gf}{\varphi}
\newcommand{\gc}{\chi}
\newcommand{\go}{\omega}

%Uppercase Greek

\newcommand{\gG}{\Gamma}
\newcommand{\gD}{\Delta}
\newcommand{\gTh}{\Theta}
\newcommand{\gL}{\Lambda}
\newcommand{\gX}{\Xi}
\newcommand{\gP}{\Pi}
\newcommand{\gS}{\Sigma}
\newcommand{\gU}{\Upsilon}
\newcommand{\gF}{\Phi}
\newcommand{\gO}{\Omega}
\def\bm#1{\mbox{\boldmath $#1$}}
\newcommand{\vga}{\mbox{$\bm \alpha$}}
\newcommand{\vgb}{\mbox{$\bm \beta$}}
\newcommand{\vgd}{\mbox{$\bm \delta$}}
\newcommand{\vge}{\mbox{$\bm \epsilon$}}
\newcommand{\vgl}{\mbox{$\bm \lambda$}}
\newcommand{\vgr}{\mbox{$\bm \rho$}}
\newcommand{\vgrh}{\mbox{$\bm \hat \rho$}}
\newcommand{\vgrt}{\mbox{$\bm {\tilde \rho}$}}

\newcommand{\vgt}{\mbox{$\bm \gt$}}
\newcommand{\vgth}{\mbox{$\bm {\hat \tau}$}}
\newcommand{\vgtt}{\mbox{$\bm {\tilde \tau}$}}
\newcommand{\vpsi}{\mbox{$\bm \psi$}}
\newcommand{\vphi}{\mbox{$\bm \phi$}}
\newcommand{\vxi}{\mbox{$\bm \xi$}}
\newcommand{\vth}{\mbox{$\bm \theta$}}
\newcommand{\vthh}{\mbox{$\bm {\hat \theta}$}}

\newcommand{\mgG}{\mbox{$\bm \Gamma$}}
\newcommand{\mgGh}{\mbox{$\hat {\bm \Gamma}$}}
\newcommand{\mgD}{\mbox{$\bm \Delta$}}
\newcommand{\mgU}{\mbox{$\bm \Upsilon$}}
\newcommand{\mgL}{\mbox{$\bm \Lambda$}}
\newcommand{\mPsi}{\mbox{$\bm \Psi$}}
\newcommand{\mgX}{\mbox{$\bm \Xi$}}
\newcommand{\bSigma}{\mbox{$\bm \Sigma$}}

%Abbreviatians for blackboard bold
\newcommand{\oA}{{\open A}}
\newcommand{\oC}{{\open C}}
\newcommand{\oF}{{\open F}}
\newcommand{\oN}{{\open N}}
\newcommand{\oP}{{\open P}}
\newcommand{\oQ}{{\open Q}}
\newcommand{\oR}{{\open R}}
\newcommand{\oZ}{{\open Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Macros by Joseph
\newcommand{\nt}{{\begin{tiny}{\rm t} \end{tiny}}}
\newcommand{\nr}{{\begin{tiny}{\rm r} \end{tiny}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Macros by Joseph
\newcommand{\avec}{{\bf{a}}}
\newcommand{\bvec}{{\bf{b}}}
\newcommand{\cvec}{{\bf{c}}}
\newcommand{\dvec}{{\bf{d}}}
\newcommand{\evec}{{\bf{e}}}
\newcommand{\fvec}{{\bf{f}}}
\newcommand{\epsvec}{{\bf{\epsilon}}}
\newcommand{\pvec}{{\bf{p}}}
\newcommand{\qvec}{{\bf{q}}}
\newcommand{\Yvec}{{\bf{Y}}}
\newcommand{\yvec}{{\bf{y}}}
%\newcommand{\Yvec}{{\bf{y}}}
\newcommand{\uvec}{{\bf{u}}}
\newcommand{\wvec}{{\bf{w}}}
\newcommand{\xvec}{{\bf{x}}}
\newcommand{\zvec}{{\bf{z}}}
\newcommand{\mvec}{{\bf{m}}}
\newcommand{\nvec}{{\bf{n}}}
\newcommand{\rvec}{{\bf{r}}}
\newcommand{\Svec}{{\bf{S}}}
\newcommand{\Tvec}{{\bf{T}}}
\newcommand{\svec}{{\bf{s}}}
\newcommand{\vvec}{{\bf{v}}}
\newcommand{\gvec}{{\bf{g}}}
\newcommand{\gveca}{\gvec_{\alphavec}}
\newcommand{\uveca}{\uvec_{\alphavec}}
\newcommand{\hvec}{{\bf{h}}}
\newcommand{\ivec}{{\bf{i}}}
\newcommand{\kvec}{{\bf{k}}}
\newcommand{\etavec}{{\bf{\eta}}}
\newcommand{\onevec}{{\bf{1}}}
\newcommand{\zerovec}{{\bf{0}}}
\newcommand{\nuvec}{{\bf{\nu}}}
\newcommand{\tauvec}{{\bf{\tau}}}
%\newcommand{\muvec}{{\bf{\mu}}}
\newcommand{\alphavec}{{\bf{\alpha}}}
%\newcommand{\psivec}{{\bf{\psi}}}
%\newcommand{\xsivec}{{\bf{\xi}}}
\newcommand{\Phivec}{{\bf{\Phi}}}
\newcommand{\deltakvec}{{\bf{\Delta k}}}
\newcommand{\Lambdamat}{{\bf{\Lambda}}}
\newcommand{\invLambdamat}{\Lambdamat^{-1}}
\newcommand{\Gammamat}{{\bf{\Gamma}}}
\newcommand{\Amat}{{\bf{A}}}
\newcommand{\Bmat}{{\bf{B}}}
\newcommand{\tr}{{\rm{T}}}
\newcommand{\Cmat}{{\bf{C}}}
\newcommand{\Dmat}{{\bf{D}}}
\newcommand{\Emat}{{\bf{E}}}
\newcommand{\Fmat}{{\bf{F}}}
\newcommand{\Kmat}{{\bf{K}}}
\newcommand{\Gmat}{{\bf{G}}}
\newcommand{\Hmat}{{\bf{H}}}
\newcommand{\Jmat}{{\bf{J}}}
\newcommand{\Imat}{{\bf{I}}}
\newcommand{\Lmat}{{\bf{L}}}
\newcommand{\Pmat}{{\bf{P}}}
\newcommand{\Mmat}{{\bf{M}}}
\newcommand{\Nmat}{{\bf{N}}}
\newcommand{\Pmatperp}{{\bf{P^{\bot}}}}
\newcommand{\Ptmatperp}{{\bf{P_2^{\bot}}}}
\newcommand{\Qmat}{{\bf{Q}}}
\newcommand{\invQmat}{\Qmat^{-1}}
\newcommand{\Smat}{{\bf{S}}}
\newcommand{\Tmat}{{\bf{T}}}
\newcommand{\Tmattilde}{\tilde{\bf{T}}}
\newcommand{\Tmatcheck}{\check{\bf{T}}}
\newcommand{\Tmatbar}{\bar{\bf{T}}}
\newcommand{\Rmat}{{\bf{R}}}
\newcommand{\Umat}{{\bf{U}}}
\newcommand{\Vmat}{{\bf{V}}}
\newcommand{\Wmat}{{\bf{W}}}
\newcommand{\Xmat}{{\bf{X}}}
\newcommand{\Ymat}{{\bf{Y}}}
\newcommand{\Zmat}{{\bf{Z}}}
\newcommand{\Ry}{\Rmat_{\yvec}}
\newcommand{\Rz}{\Rmat_{\zvec}}
\newcommand{\RyInv}{\Rmat_{\yvec}^{-1}}
\newcommand{\Ryhat}{\hat{\Rmat}_{\yvec}}
\newcommand{\Rs}{\Rmat_{\svec}}
\newcommand{\Rn}{\Rmat_{\nvec}}
\newcommand{\Rninv}{\Rmat_{\nvec}^{-1}}
\newcommand{\Reta}{\Rmat_{\etavec}}
\newcommand{\Ralpha}{\Rmat_{\alphavec}}
\newcommand{\Ck}{\Cmat_{\kvec}}
\newcommand{\Cn}{\Cmat_{\nvec}}
\newcommand{\Cg}{\Cmat_{\gvec}}
\newcommand{\invRn}{\Rmat_{\nvec}^{-1}}
\newcommand{\w}{\bf w}
\newcommand{\E}{{\rm{E}}}
%\newcommand{\D}{{\rm{E}}}
\newcommand{\dbsdalpha}{\Tmat_1 \frac{\partial b\svec_1(\alphavec )}{\partial \alphavec}}
\newcommand{\dbsHdalpha}{\frac{\partial b\svec_1^H(\alphavec )}{\partial \alphavec} \Tmat_1^H}
\newcommand{\dbstdalpha}{\Tmat_2 \frac{\partial b\svec_2(\alphavec )}{\partial \alphavec}}
\newcommand{\dbstHdalpha}{\frac{\partial b\svec_2^H(\alphavec )}{\partial \alphavec} \Tmat_2^H}
\newcommand{\dtdw}{\left[ \frac{d\hat{\theta} (\hat{\wvec})}{d \wvec} \right]_{\wvec = \wvec_o}}
\newcommand{\dtdu}{\left[ \frac{d\hat{\theta} (\hat{\uvec})}{d \uvec} \right]_{\uvec = \uvec_o}}

\newcommand{\Jww}{J_{\wvec \wvec}}
\newcommand{\Jbb}{J_{\bvec \bvec}}
\newcommand{\Jaa}{J_{\alphavec \alphavec}}
\newcommand{\Jtb}{J_{\thetavec \bvec}}
\newcommand{\Jbt}{J_{\bvec \thetavec}}
\newcommand{\Jwt}{J_{\wvec \thetavec}}
\newcommand{\Jtw}{J_{\thetavec \wvec}}
\newcommand{\Jtu}{J_{\thetavec \uvec}}
\newcommand{\Jtt}{J_{\thetavec \thetavec}}
\newcommand{\Jee}{J_{\etavec \etavec}}
\newcommand{\Jae}{J_{\alphavec \etavec}}
\newcommand{\Jea}{J_{\etavec \alphavec}}
\newcommand{\fww}{f_{\wvec \wvec}}
\newcommand{\fwt}{f_{\wvec \thetavec}}
\newcommand{\ftw}{f_{\thetavec \wvec}}
\newcommand{\ftt}{f_{\thetavec \thetavec}}
\newcommand{\Juu}{J_{\uvec \uvec}}
\newcommand{\Jub}{J_{\uvec \bvec}}
\newcommand{\Jbu}{J_{\bvec \uvec}}
\newcommand{\Jaatilde}{\tilde{J}_{\alphavec \alphavec}}
\newcommand{\Jqq}{J_{\qvec \qvec}}
\newcommand{\Jaq}{J_{\alphavec \qvec}}
\newcommand{\Jqa}{J_{\qvec \alphavec}}
\newcommand{\JTT}{J_{\Thetavec \Thetavec}}
\newcommand{\Tr}{{\rm Tr}}
\newcommand{\vecc}{{\rm vec}}
\newcommand{\Imm}{{\rm Im}}
\newcommand{\Ree}{{\rm Re}}
\newcommand{\cum}{{\rm cum}}
\newcommand{\real}{{\mathbb{R}}}
\newcommand{\comp}{{\mathbb{C}}}
\newcommand{\nat}{{\mathbb{N}}}
\newcommand{\integer}{{\mathbb{Z}}}
\newcommand{\BorelN}{{\cal B}(\Real^N)}
\newcommand{\BorelL}{{\cal B}(\Real^L)}
\newcommand{\dftheta}{{\partial f_{X,\Phi}(x,\phi;\theta)}/{\partial \theta}}
\newcommand{\dfphi}{{\partial f_{X,\Phi}(x,\phi;\theta)}/{\partial \phi}}
\newcommand{\dlogftheta}{{\partial \log f_{\Xmat,\Phivec}(\Xmat,\Phivec;\thetavec)}/{\partial \thetavec^T}}
\newcommand{\Dlogftheta}{\frac{\partial \log f_{\Xmat,\Phivec}(\Xmat,\Phivec;\thetavec)}{\partial \thetavec^T}}
\newcommand{\dlogfphi}{{\partial \log f_{\Xmat,\Phivec}(\Xmat,\Phivec;\thetavec)}/{\partial \phivec^T}}
\newcommand{\F}{{\mathbf F}}
\newcommand{\Fp}{{\mathbf {F_p}}}
\newcommand{\D}{{\mathbf {D}}}
\newcommand{\FH}{{\mathbf {\tilde F}}}
\newcommand{\0}{{\mathbf {0}}}

%\newcommand{\Hmat}{{\mathbf H}}

\newcommand{\FHt}{{\mathbf {\tilde F_{\theta}}}}
\newcommand{\FHp}{{\mathbf {\tilde F_{\phi}}}}
\newcommand{\FHtp}{\mathbf {\tilde F_{{\theta,\phi}}}}
\newcommand{\define}{\stackrel{\triangle}{=}}
\newcommand{\Intiger}{{\mathbb{Z}}}
%\newcommand{\E}{{\rm E}}

%%% For BOLD Greek Letters

\newcommand{\Psimat}{\mbox{\boldmath $\Psi$}}
\newcommand{\blambda}{\mbox{\boldmath $\lambda$}}

\newcommand{\bzeta}{\mbox{\boldmath $\zeta$}}

\def\bzeta{{\mbox{\boldmath $\zeta$}}}

\def\btheta{{\mbox{\boldmath $\theta$}}}

\def\bgamma{{\mbox{\boldmath $\gamma$}}}

\def\Beta{{\mbox{\boldmath $\eta$}}}

\def\lam{{\mbox{\boldmath $\Gamma$}}}

\def\bomega{{\mbox{\boldmath $\omega$}}}

\def\bxi{{\mbox{\boldmath $\xi$}}}

\def\brho{{\mbox{\boldmath $\rho$}}}

\def\bmu{{\mbox{\boldmath $\mu$}}}

\def\bnu{{\mbox{\boldmath $\nu$}}}

\def\btau{{\mbox{\boldmath $\tau$}}}

\def\bphi{{\mbox{\boldmath $\phi$}}}

\def\bsigma{{\mbox{\boldmath $\Sigma$}}}

\def\bLambda{{\mbox{\boldmath $\Lambda$}}}

%%% For BOLD Greek Letters

\def\btheta{{\mbox{\boldmath $\theta$}}}
\def\Thetavec{{\mbox{\boldmath $\Theta$}}}

\def\bomega{{\mbox{\boldmath $\omega$}}}

\def\brho{{\mbox{\boldmath $\rho$}}}

\def\bmu{{\mbox{\boldmath $\mu$}}}

\def\bGamma{{\mbox{\boldmath $\Gamma$}}}

\def\bnu{{\mbox{\boldmath $\nu$}}}

\def\btau{{\mbox{\boldmath $\tau$}}}

\def\bphi{{\mbox{\boldmath $\phi$}}}

\def\bPhi{{\mbox{\boldmath $\Phi$}}}

\def\bxi{{\mbox{\boldmath $\xi$}}}


\def\bvarphi{{\mbox{\boldmath $\varphi$}}}

\def\bepsilon{{\mbox{\boldmath $\epsilon$}}}

\def\balpha{{\mbox{\boldmath $\alpha$}}}

\def\bvarepsilon{{\mbox{\boldmath $\varepsilon$}}}

\def\bXsi{{\mbox{\boldmath $\Xi$}}}

%% Ilya

%\newcommand{\betavec}{{\bf{\beta}}}
\def\betavec{{\mbox{\boldmath $\beta$}}}
\def\betavecsc{{\mbox{\boldmath \tiny $\beta$}}}

\def\psivec{{\mbox{\boldmath $\psi$}}}

\def\xsivec{{\mbox{\boldmath $\xi$}}}
\def\xsivecsc{{\mbox{\boldmath \tiny $\xsivec$}}}

\def\alphavec{{\mbox{\boldmath $\alpha$}}}
\def\alphavecsc{{\mbox{\boldmath \tiny $\alpha$}}}

\def\gammavec{{\mbox{\boldmath $\gamma$}}}

\def\etavec{{\mbox{\boldmath $\eta$}}}

\def\thetavec{{\mbox{\boldmath $\theta$}}}
\def\deltavec{{\mbox{\boldmath $\delta$}}}
\def\phivec{{\mbox{\boldmath $\phi$}}}
\def\evec{{\mbox{\boldmath $e$}}}
\def\tvec{{\mbox{\boldmath $t$}}}

\def\thetavecsc{{\mbox{\boldmath \tiny $\theta$}}}
\def\WHML{\hat\Wmat_{\rm ML/MAP}}


\def\muvec{{\mbox{\boldmath $\mu$}}}

\def\Ximat{{\mbox{\boldmath $\Xi$}}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beqna}{\begin{eqnarray}}
\newcommand{\eeqna}{\end{eqnarray}}



%\newcommand{\}{}
%\mathaccent{\mjm}{$J_{m}$}

\newcommand{\postscript}[4]
{
 \begin{figure}[htb]
 \par
 \hbox{\vbox to #1
        {
        \vfil
        \special{psfile= #2.ps}
        }
      }
 \caption{#3}
 \label{#4}
 \end{figure}
}
%matrix operation
\def\mc#1{\multicolumn{1}{c|}{#1}}



==> Chapters/notation.TEX <==
\begin{tabular}{ll}

%Functional Notation
%${x}$& scalar\\
$[a,b]$& row vector with two entries; a and b\\
$\textbf{x}$& column vector; i.e., boldface lowercase letters\\
$\textbf{X}$&  matrix; i.e., boldface uppercase letters \\
$(\cdot)^T$ & transpose operation \\
% $k$ & time index\\
$\sigma^2_x$ & covariance of variable $x$ \\
${\mathbb E}\left[x\right] $ & expectation of variable $x$\\

$g(\mathbf{x})$ & a scalar function of a vector $\mathbf{x}$\\
$\partial g(\mathbf{x})/\partial \mathbf{x}$& gradient operation \\
$\partial \mathbf{g}(\mathbf{x})/\partial\mathbf{x}$ &Jacobian of $\mathbf{g}(\mathbf{x})$\\

$[\mathbf{A}]_{ij}$ & denotes the $i,j$-th entry of matrix $\textbf{A}$ \\

$(\Vert\cdot \Vert)$ & spectral norm operator \\

% ${\rm blockdiag}(\mathbf{A},\mathbf{B})$ &  block-diagonal matrix whose upper-left and\\ $$& lower-right are equal to $\mathbf{A}$ and $\mathbf{B}$, respectively. \\

%General Mathematical Notation




%Problem-Specific Notation 

%\\
%Hagi:
%\\
%%Functional Notation
%${x}$ & scalar\\
%$\textbf{x}$ & vector\\
%${X}$ &  random variable\\
%$\bfX$ & random vector\\
%${\cal X}$ & set\\
%${\cal X}^n$ & n-fold cartesian power of ${\cal X}$\\
%
%%General Mathematical Notation
%$|x|$ &absolute value of $x$\\
%$\|\cdot\|$ & 1-norm\\
%${\mathbb E}(X)$ &expectation of random variable $X$\\
%$H(X)$ &entropy of random variable $X$\\
%$I(X;Y)$ & mutual information between $X$ and $Y$\\
%$\inf$ &infimum \\
%$\sup$ &supremum \\
%$\Sigma_X$ &covariance matrix of random vector $\bfX$ \\
%
%$\log_2^+{}(x)$ &$\max\{0,\log_2(x)\}$\\
%$\mathbb{R}$ &set of real numbers\\
%
%%Problem-Specific Notation 
%$\alpha$ & excess distortion ratio\\
%$D_i$ & expected squared-error distortion of source output at user i\\
%$\gamma_{i}$ & energy-to-noise ratio of user i\\
%$i$ & user index\\
%$k$ & time index\\
%$m$ & source block length\\
%$n$ & channel block length\\
%$N$ &additive noise variance\\
%$E$ &average total energy constraint\\
%$P$ &average power constraint\\
%$\phi^{(i)}$ & reconstruction function at receiver i\\
%$\varphi^{(m,n)}(\cdot)$ & encoding function\\
%$R_i$ & message rate\\
%$R_D(\cdot)$ &rate-distortion function\\
%$R_{S_2|S_1}(\cdot)$ &conditional rate-distortion function of $\{S_{2,k}\}$ conditioned on $\{S_{1,k}\}$\\
%$\rho$ & bandwidth expansion factor\\
%$S_{k}$ & time-k source output \\
%$\hat{S}_{i,k}$ & estimate of $S_{k}$ at user i\\
%\end{tabular}
%\newpage
%\begin{tabular}{ll}
%$\sigma^2$ &source variance \\
%$X_{k}$ & time-k channel input\\
%$Y_{i,k}$ & time-k channel output at user i\\
%$Z_{i,k}$ &time-k additive noise term at user i\\
\end{tabular}







==> Chapters/numerical_results.tex <==
In this section we present the numerical results for the three simulation setups. In the first setup, whose results are presented in Sec. \ref{uaaConf}, the sensors are organized in UAA-type configurations, and some comparisons are made. In the second setup, whose results are presented in Sec. \ref{circConf}, the sensors are organized in a half circle which is centered on the source and key aspects are examined. In the third setup, whose results are presented in the same section, the sensors are organized as a uniform linear array. 

\section{UAA Type Configurations}\label{uaaConf}
In this section, different shapes of UAA are compared. The simulation's setup details are as follows: the pathloss exponent is $\gamma=2$, the signal's period time is $T=10^{-8}$, the noise is AWGN with spectral density $N_0=10^{-3}$ and the signal's energy is determined by the SNR, the signal's propagation speed is the speed of light, $c=3\cdot10^8$ and the effective bandwidth is $We=2 c^2$. The first comparison is between two configurations with the same number of sensors (seven in this case), but differently organized: in one network all the sensors belong to the same UAA, whereas in a second network they are divided into two UAAs. The maximal radius is similar in both networks. In the simulation, TDOA estimation performance and CRB are compared to TOA estimation performance and CRB. The different networks are presented in fig. \ref{fig:uaa_confs}, and the results are presented in fig. \ref{fig:CRBs_diff_UAA_m7}.
\begin{figure}[!h]
	\centering
	\includegraphics[height=0.3\textwidth]{1uaa_net_m7}
	~ 
	\includegraphics[height=0.3\textwidth]{2uaa_net_m7}
	\caption{Comparison of UAA Type Configurations}
	\label{fig:uaa_confs}
\end{figure}
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.5\textwidth]{CRBs_diff_UAA_m7}
	\caption{MSE VS TDOA and TOA CRBs for the different UAAs}
	\label{fig:CRBs_diff_UAA_m7} 
\end{figure}
\\As expected, the TOA CRB equals the TDOA CRB in both cases. Naturally, the CRB decreases when changing the configuration from a single UAA to two UAAs, since some sensors become closer and no sensor becomes farther away. This change, as well known, improves the estimation performance. \\
In real life, the UAA situation is rare. However, a highly similar situation can certainly occure. Thus, an important insight is the relationship between TOA and TDOA CRBs when the source moves from the UAA's center. In this expression, there are six sensors, organized into a single UAA. During the simulation, the sensors' location is constant while the source moves along a line from the UAA's center to its edge. At the end, the source is located exactly between the two sensors. The results are presented in fig. \ref{fig:shifted_uaa_lin_M6} below.
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.5\textwidth]{shifted_uaa_lin_M6}
	\caption{TDOA CRB and TOA CRB when shifting the source from the UAA center to the UAA itself}
	\label{fig:shifted_uaa_lin_M6} 
\end{figure}
 When looking at the relationship between the TDOA and TOA CRBs, a number of features emerge. As described in Sec \ref{chap:insight1UAA}, in the small shift situation the CRBs converge to each other. In addition, when the source gets closer to the UAA itself, a key difference between TOA and TDOA emerges: while TOA estimation requires at least two sensors, TDOA estimation requires three. Thus, when becoming closer to two sensors in particular and farther from the others, TOA estimation is improved, but TDOA estimation becomes worse.
 
\section{Other Configurations}\label{circConf}
In this section, two configurations are compared. In one network, there are six sensors located at the same distance from the source, uniformly distributed over half a circle. This configuration looks similar to UAA but typicaly does not maintain the basic condition defined in Sec. \ref{chap:insight1UAA}. The simulation setup was identical to that described in the previous section. MLE performance using TDOA estimation is first compared to the TDOA CRB are presented in fig. \ref{fig:circleVSlin_MSE}. For comparison purposes, the TOA CRB is presented as well. Another network whose CRBs and performance are presented in the same graph is a uniform linear array, which is a commonly used configuration. In this case, the source is located facing the middle of the array, and the distance between them equals the radius of the half circle. Once again there are six sensors, and the distance between two adjacent sensors is constant. The different configurations are presented in fig. \ref{fig:confs} below.  
\begin{figure}[!h]
	\centering
	\includegraphics[height=0.5\textwidth]{half_circ_m6}
	~ 
	\includegraphics[height=0.5\textwidth]{lin_array_m6}
	\caption{Compared Network Configurations}
	\label{fig:confs}
\end{figure}
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.5\textwidth]{circleVSlin_MSE}
	\caption{MSE vs. TDOA and TOA CRBs for the different configurations}
	\label{fig:circleVSlin_MSE} 
\end{figure}

The results show convergence of the MLEs MSE to the TDOA CRB. As expected, in both cases the TDOA CRB was larger than the TOA CRB. The gap between TOA CRB and TDOA CRB in the linear array is consistent with the precondition, there are only two sensors with the same distance from the source, but every UAA must contain at least three sensors, as noted in Sec. \ref{chap:insight1UAA}. In the half circle configuration, however, there is less of a difference, and the condition needs to be verified. All the sensors are located at the same distance from the source, so they can be considered one UAA. When plugging the data in the condition expression, using eq. (\ref{gen_sum})
\begin{equation}
	\sum_{n=0}^{M-1}\cos\left(\psi+\frac{n\pi}{M}\right)=\frac{\sin\left(\frac{M\pi}{2M}\right)\cos\left(\psi+\frac{(M-1)\pi}{2M}\right)}{\sin\left(\frac{\pi}{2M}\right)}=\frac{\cos\left(\psi+\frac{(M-1)\pi}{2M}\right)}{\sin\left(\frac{\pi}{2M}\right)}
\end{equation}
In general, it does not equal zero, and thus its TDOA CRB and TOA CRB are not the same.\par
Another interesting set of configurations is a half circle with a constant radius and a varying number of sensors. One approach is to verify the TDOA CRB orientation when the increasing the number of sensors. In fig. \ref{fig:TOA_TDOA_linVScirc_growingM} below, the TDOA CRB and TOA CRB, with low SNR and high SNR are presented, in two different configurations. The first is described above, and the second is an expanding uniform linear array. The distance between two adjacent sensors is preserved, but the total array length varies. As in the previous simulations, the minimal distance in the linear array equals the half circle's radius.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.6\textwidth]{TOA_TDOA_linVScirc_growingM}
	\caption{TDOA and TOA CRBs in different configurations with increasing numbers of sensors at low and high SNRs}
	\label{fig:TOA_TDOA_linVScirc_growingM} 
\end{figure}
A more in-depth examination of fig. \ref{fig:TOA_TDOA_linVScirc_growingM}, reveals some interesting findings. First, as was shown in eq. (\ref{CRBlast}), the SNR is only a constant that has no relationship to the configuration itself. This conclusion is manifested in the identity between the low SNR lines and the high SNR lines, except when multiplying by a constant.\\
Second, an interesting but common sense difference can be seen between the lines belonging to the circle network and the lines belonging to the linear network. While the circle lines converge to zero, even by different routes, the linear lines converge to constants. One possible explanation is as follows. Adding more sensors to the circle network is equivalent to increasing the sensor density. Thus, the CRBs converge to zero. By contrast, in linear networks, adding sensors negatively impacts on the network performance due to their increasing distance from the source, hence their contribution to the CRBs converges to zero.\\
One more takeaway from this figure is the constant gap between TOA CRB and TDOA CRB. In contrast to the convergence of TDOA CRB to TOA CRB when the SNR increases, in this case the CRBs do not converge. This would be an interesting direction for future research.\par
As detailed in Sec. \ref{chap:insight2compModels}, TDOA estimation performance when the received signals amplitudes are known and TDOA estimation performance when the amplitudes are estimated as nuisance parameters theoretically converge to each other. In fig. $fff$ below, the simulation results are presented. In this simulation, the configuration is ten sensors that uniformly scattered on a half of a circle centered on the source. TDOA is estimated in three different ways. In the first, the real amplitudes are known to the estimator but not their connection to the source location. In the second one, the amplitudes are unknown and are estimated as nuisance parameters. In the last one, TDOA-RSS estimation is applied. In other words, the estimator knows the connection between the source location and the received signal amplitudes. 
%\begin{figure}[H]
%	\centering
%	\includegraphics[width=0.6\textwidth]{TDOA_3Methods_M10}
%	\caption{TDOA estimation MSE in three different methods for amplitude estimation}
%	\label{fig:TDOA_3Methods_M10} 
%\end{figure}
As can be seen, the first two methods converge to each other. In this configuration the TDOA-RSS estimation converges to the same CRB as well. Since it does not converge to a higher CRB but rather to the same values, and its estimation performance is always lower than the other methods' performance values, the results are still consistent with the theoretical analysis. As is well known and detailed in Sec. \ref{chap:background_rss}, RSS estimation loses its advantages at larger distances. This may explain the limit identity. 

==> Chapters/numerical_results_after_itsik.tex <==
In this section we present the numerical results for the three simulation setups. In the first setup, whose results are presented in Sec. \ref{uaaConf}, the sensors are organized in UAA-type configurations, and some comparisons are made. In the second setup, whose results are presented in Sec. \ref{circConf}, the sensors are organized in a half circle which is centered on the source and key aspects are examined. In the third setup, whose results are presented in the same section, the sensors are organized as a uniform linear array.  In addition, all the mentioned distances are in kilometer, and the SNR values are in $dB$ and at $1$ kilometer.

\section{UAA Type Configurations}\label{uaaConf}
In this section, different shapes of UAA are compared. The simulation's setup details are as follows: the pathloss exponent is $\gamma=2$, the signal's period time is $T=10^{-8}s$, the noise is AWGN with spectral density $N_0=10^{-3}$ and the signal's energy is determined by the SNR, the signal's propagation speed is the speed of light, $c=3\cdot10^8$ and the effective bandwidth is $W_e=18\cdot 10^{16}(=2c^2)$.\\
The first comparison is between two configurations with the same number of sensors (seven in this case), but differently organized: in one network all the sensors belong to the same UAA with radius $3.5$, whereas in a second network they are divided into two UAAs with radiuses $0.5$ and $3.5$. The maximal radius is similar in both networks. In the simulation, TDOA estimation performance and CRB are compared to TOA estimation performance and CRB. The different networks are presented in Fig. \ref{fig:uaa_confs}, and the results are presented in Fig. \ref{fig:CRBs_diff_UAA_m7}.
\begin{figure}[!t]
	\centering
	\includegraphics[height=0.3\textwidth]{1uaa_net_m7}
	~ 
	\includegraphics[height=0.3\textwidth]{2uaa_net_m7}
	\caption{Comparison of UAA Type Configurations}
	\label{fig:uaa_confs}
\end{figure}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.7\textwidth]{CRBs_diff_UAA_m7}
	\caption{MSE VS TDOA and TOA CRBs for the different UAAs}
	\label{fig:CRBs_diff_UAA_m7} 
\end{figure}
\\
As expected, the TOA CRB equals the TDOA CRB in both cases. Naturally, the CRB decreases when changing the configuration from a single UAA to two UAAs, since some sensors become closer and no sensor becomes farther away. This change, as well known, improves the estimation performance. \\
In real life, the UAA situation is rare. However, a highly similar situation can certainly occure. Thus, an important insight is the relationship between TOA and TDOA CRBs when the source moves from the UAA's center.\\
In the following scenario, there are six sensors, organized into a single UAA with radius $1$. During the simulation, the sensors' location is constant while the source moves along a line from the UAA's center to its edge. At the end, the source is located exactly between two sensors. The results are presented in Fig. \ref{fig:shifted_uaa_lin_M6} below.
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.7\textwidth]{shifted_uaa_lin_M6}
	\caption{TDOA CRB and TOA CRB when shifting the source from the UAA center to the UAA itself}
	\label{fig:shifted_uaa_lin_M6} 
\end{figure}
 \\
 When looking at the relationship between the TDOA and TOA CRBs, a number of features emerge. As described in Sec \ref{chap:insight1UAA}, in the small shift situation the CRBs converge to each other. In addition, when the source gets closer to the UAA itself, a key difference between TOA and TDOA emerges: while TOA estimation requires at least two sensors, TDOA estimation requires three. Thus, when becoming closer to two sensors in particular and farther from the others, TOA estimation is improved, but TDOA estimation becomes worse.
 
\section{Other Configurations}\label{circConf}
In this section, two configurations are compared. In one network, there are six sensors located at the same distance from the source, uniformly distributed over half a circle. This configuration looks similar to UAA but typically does not maintain the basic condition defined in Sec. \ref{chap:insight1UAA}. \\
The simulation setup is almost identical to that described in the previous section, but the radius is $1.5$. MLE performance using TDOA estimation is first compared to the TDOA CRB are presented in Fig. \ref{fig:circleVSlin_MSE}. For comparison purposes, the TOA CRB is presented as well. \\
Another network whose CRBs and performance are presented in the same graph is a uniform linear array, which is a commonly used configuration. In this case, the source is located facing the middle of the array, and the distance between them equals the radius of the half circle. Once again there are six sensors, and the distance between two adjacent sensors is constant- $3.6$. The different configurations are presented in Fig. \ref{fig:confs} below.  
\begin{figure}[!h]
	\centering
	\includegraphics[height=0.5\textwidth]{half_circ_m6}
	~ 
	\includegraphics[height=0.5\textwidth]{lin_array_m6}
	\caption{Compared Network Configurations}
	\label{fig:confs}
\end{figure}
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\textwidth]{circleVSlin_MSE}
	\caption{MSE vs. TDOA and TOA CRBs for the different configurations}
	\label{fig:circleVSlin_MSE} 
\end{figure}

The results show convergence of the MLEs MSE to the TDOA CRB. As expected, in both cases the TDOA CRB was larger than the TOA CRB. The gap between TOA CRB and TDOA CRB in the linear array is consistent with the precondition, there are only two sensors with the same distance from the source, but every UAA must contain at least three sensors, as noted in Sec. \ref{chap:insight1UAA}. In the half circle configuration, however, there is less of a difference, and the condition needs to be verified. All the sensors are located at the same distance from the source, so they can be considered one UAA. When plugging the data in the condition expression, using eq. (\ref{gen_sum})
\begin{equation}
	\sum_{n=0}^{M-1}\cos\left(\psi+\frac{n\pi}{M}\right)=\frac{\sin\left(\frac{M\pi}{2M}\right)\cos\left(\psi+\frac{(M-1)\pi}{2M}\right)}{\sin\left(\frac{\pi}{2M}\right)}=\frac{\cos\left(\psi+\frac{(M-1)\pi}{2M}\right)}{\sin\left(\frac{\pi}{2M}\right)}
\end{equation}
In general, it does not equal zero, and thus its TDOA CRB and TOA CRB are not the same.\par
Another interesting set of configurations is the same type of configuration but with  a varying number of sensors. For example, a half circle with a constant radius. In Fig. \ref{fig:TOA_TDOA_linVScirc_growingM_high} below, the TDOA CRB and TOA CRB with SNR at $1$ kilometer $\rho=5dB$ are presented, in two different configurations. The first is a half circle with radius $1.5$ and increasing number of sensors that uniformly distributed, and the second is an expanding uniform linear array with distance $1.5$ from the source. The distance between two adjacent sensors is always $1.5$ , but the total array length varies. As in the previous simulations, the minimal distance in the linear array equals the half circle's radius.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.8\textwidth]{TOA_TDOA_linVScirc_growingM_high}
	\caption{TDOA and TOA CRBs in different configurations with increasing numbers of sensors at low and high SNRs}
	\label{fig:TOA_TDOA_linVScirc_growingM_high} 
\end{figure}
A more in-depth examination of Fig. \ref{fig:TOA_TDOA_linVScirc_growingM_high}, reveals some interesting findings. First, an interesting but common sense difference can be seen between the lines belonging to the circle network and the lines belonging to the linear network. While the circle lines converge to zero, even by different routes, the linear lines converge to constants. This is because the added sensors in the linear configuration are at increasing distance from the source, hence their contribution to the CRBs converges to zero.\\
One more takeaway from this figure is the constant gap between TOA CRB and TDOA CRB. This would be an interesting direction for future research.\par
As detailed in Sec. \ref{chap:insight2compModels}, TDOA estimation performance when the received signals amplitudes are known and TDOA estimation performance when the amplitudes are estimated as nuisance parameters theoretically converge to each other. In Fig. $fff$ below, the simulation results are presented. In this simulation, the configuration is ten sensors that are uniformly scattered on a half of a circle centered on the source.\\
TDOA is estimated in three different ways. In the first, the real amplitudes are known to the estimator but not their relation to the source location. In the second one, the amplitudes are unknown and are estimated as nuisance parameters. In the last one, TDOA-RSS estimation is applied. In other words, the estimator knows the relation between the source location and the received signal amplitudes. \\
%\begin{figure}[H]
%	\centering
%	\includegraphics[width=0.6\textwidth]{TDOA_3Methods_M10}
%	\caption{TDOA estimation MSE in three different methods for amplitude estimation}
%	\label{fig:TDOA_3Methods_M10} 
%\end{figure}
As can be seen, the first two methods converge to each other. In this configuration the TDOA-RSS estimation converges to the same CRB as well. Since it does not converge to a higher CRB but rather to the same values, and its estimation performance is always lower than the other methods' performance values, the results are still consistent with the theoretical analysis. As is well known and detailed in Sec. \ref{chap:background_rss}, RSS estimation loses its advantages at larger distances. This may explain the limit identity. 

==> Chapters/sat_ACRBE_h_goes_0.tex <==
As can be seen, ${\rm ACRB_{E,xy}}$ and ${\rm ACRB_{E,z}}$ converge to constants when $h$ goes to zero. Although small values of $h$ are not feasible, the limits are interesting and are calculated. 
\begin{theorem}
	\begin{eqnarray}
		\lim_{h\rightarrow 0}{\rm ACRB_{E,xy}}&=&\frac{-16r^2}{\eta N \Big(2\log\cos\phi_{max,\alpha}+\sin^2\phi_{max,\alpha}\Big)}\label{limhACRBExy}\\
		\lim_{h\rightarrow 0}{\rm ACRB_{E,z}}&=&\frac{4r^2}{\eta N[\sin^2\phi_{max,\alpha}+\frac{2(1-\cos\phi_{max,\alpha})^2}{\log\cos\phi_{max,\alpha}}]}\label{limhACRBEz}
	\end{eqnarray}
\end{theorem}
\begin{IEEEproof}
	Before these calculations, we produce some partial limits, and use them later.\\
The first limit is 
\begin{equation}
	\lim_{h\rightarrow 0}\frac{D_M}{h}=\lim_{h\rightarrow 0}\frac{\sqrt{(r+h)^2-r^2+r^2\zeta^2}-r\zeta}{h}
\end{equation}
It is clear that this limit can be solved using L'H\^{o}pital's rule. In other words:
\begin{eqnarray}
	\lim_{h\rightarrow 0}\frac{D_M}{h}=\lim_{h\rightarrow 0}\frac{2(r+h)}{2\sqrt{(r+h)^2-r^2+r^2\zeta^2}}=\frac{r}{|r\zeta|}=\frac{1}{\zeta}
	\label{limDm_H}
\end{eqnarray}
We assume that $\zeta$ is positive because $\phi_{max,\alpha}$ is assumed to be in $[0,\pi/2]$. \\
Secondly, $D_M$ goes to zero when $h$ goes to zero, so we approximate $D_M$ using Taylor series:
\begin{equation}
	D_M\approx \frac{h}{\zeta}-h^2\frac{1-\zeta^2}{2r\zeta^3}
\end{equation}
Second order approximation is enough for us. As a result, 
\begin{equation}
	h-D_{M}\zeta\approx h^2\frac{1-\zeta^2}{2r\zeta^2}=\frac{h^2\tan^2\phi_{max,\alpha}}{2r}
	\label{tylr}
\end{equation}
Using the formulas above, we can produce the wanted limits:
\begin{eqnarray}
	{\rm ACRB_{E,xy}}&=&\frac{8(r+h)}{\eta N(h-D_M\zeta) \Big(\log\left(\frac{D_{M}}{h}\right)\frac{((r+h)^2+r^2)}{2r^3(h-D_{M}\zeta)}-\frac{(r+h)^2+r(r+h-D_{M}\zeta)}{2r^2D_{M}^2}\Big)}\nonumber\\
	&=&\frac{8(r+h)}{\eta N \Big(\log\left(\frac{D_{M}}{h}\right)\frac{((r+h)^2+r^2)}{2r^3}-\frac{(h-D_M\zeta)((r+h)^2+r(r+h-D_{M}\zeta))}{2r^2D_{M}^2}\Big)}\nonumber\\
	&\approx&\frac{8(r+h)}{\eta N \Big(\log\left(\frac{D_{M}}{h}\right)\frac{((r+h)^2+r^2)}{2r^3}-\frac{h^2\tan^2\phi_{max,\alpha}((r+h)^2+r(r+\frac{h^2\tan^2\phi_{max,\alpha}}{2r}))}{4r^3D_{M}^2}\Big)}
\end{eqnarray}
Using Eq. \ref{limDm_H} and \ref{tylr}, the limit is simply produced:
\begin{eqnarray}
\lim_{h\rightarrow 0}{\rm ACRB_{E,xy}}&=&\lim_{h\rightarrow 0}\frac{8(r+h)}{\eta N \Big(\log\left(\frac{D_{M}}{h}\right)\frac{((r+h)^2+r^2)}{2r^3}-\frac{h^2\tan^2\phi_{max,\alpha}((r+h)^2+r(r+\frac{h^2\tan^2\phi_{max,\alpha}}{2r}))}{4r^3D_{M}^2}\Big)}\nonumber\\
&=&\frac{8(r+h)}{\eta N \Bigg(-\log\zeta\frac{(r+h)^2+r^2}{2r^3}-\frac{\zeta^2\tan^2\phi_{max,\alpha}\left((r+h)^2+r\left(r+\frac{h^2\tan^2\phi_{max,\alpha}}{2r}\right)\right)}{4r^3}\Bigg)}
\end{eqnarray}
Using ${\rm ACRB_{E,xy}}$ continuity in $h$ and $\zeta$ definition, the proof for Eq. \ref{limhACRBExy} is completed. Using the same equations, $\lim_{h\rightarrow 0}{\rm ACRB_{E,z}}$ is produced:
\begin{eqnarray}
	{\rm ACRB_{E,z}}&=&\frac{2(r+h)}{\eta N(h-D_M\zeta)}\Bigg[\Bigg(\frac{(r+h)^2+r(r+h-D_{M}\zeta)}{2r^2D_{M}^2}-\frac{h(2r+h)}{2r^3(h-D_{M}\zeta)} \log\Big(\frac{D_{M}}{h}\Big)\nonumber\\
	&&-\frac{[r+h-D_{M}^{-1}(r(h-D_{M}\zeta)+h(r+h))]^2}{r^3\log\Big(\frac{D_{M}}{h}\Big)(h-D_{M}\zeta)}\Bigg)\Bigg]^{-1} \nonumber\\
	&=&\frac{2(r+h)}{\eta N}\Bigg[\frac{(h-D_M\zeta)((r+h)^2+r(r+h-D_{M}\zeta))}{2r^2D_{M}^2}-\frac{h(2r+h)}{2r^3} \log\Big(\frac{D_{M}}{h}\Big)\nonumber\\
	&&-\frac{[r+h-D_{M}^{-1}(r(h-D_{M}\zeta)+h(r+h))]^2}{r^3\log\Big(\frac{D_{M}}{h}\Big)}\Bigg]^{-1} 
\end{eqnarray}
When calculating the limit, we can use the approximations from Eq. \ref{limDm_H} and \ref{tylr} and the proof for Eq. \ref{limhACRBEz} is completed.  
\end{IEEEproof}
In reality, $h$ is very large, and the limit $h\rightarrow0$ has almosts no meaning. Thus,  
we also present an intersting approximation for the limit $h\rightarrow\infty$, that is closer to reality. ${\rm ACRB_{E}}$ itself strives for infinity, but we find out that ${\rm ACRB_{E}}/h^2$ converges to a finite limit, and its value. 
\begin{theorem}
	\begin{eqnarray}
	\lim_{h\rightarrow \infty}\frac{{\rm ACRB_{E,xy}}}{h^2}&=&\frac{24}{\eta N(\zeta+2) (1-\zeta)^2}\label{limhACRBExyinf}\\
	\lim_{h\rightarrow  \infty}\frac{{\rm ACRB_{E,z}}}{h^2}&=&\frac{24}{\eta N(1-\zeta)^3}\label{limhACRBEzinf}
	\end{eqnarray}
\end{theorem}
\begin{IEEEproof}
	Using Taylor series, the limit is simply the ratio between the highest powers of $h$ in the numerator and the denominator. 
\subsection{${\rm ACRB_{E,xy}}$}
First, we approximate two non-polynomial functions using Taylor series of third degree.
\begin{eqnarray}
	&&\log\left(\frac{\sqrt{h^2 + 2 h r + r^2\zeta^2}-r\zeta}{h}\right)\approx-\frac{r (\zeta-1)}{h}+\frac{r^2 (\zeta-1)}{h^2}+\frac{r^3 \left(\zeta^3-9\zeta+8\right)}{6 h^3}\label{approxLog}\\
	&&\sqrt{h^2+2 h r+r^2\zeta ^2}\approx\frac{-r^4 (\zeta^4-6\zeta^2+5)}{8 h^3}-\frac{r^3 \left(\zeta^2-1\right)}{2 h^2}+\frac{r^2 (\zeta^2-1)}{2 h}+h+r
	\label{approxSqrt}
\end{eqnarray}
Putting these approximations in ${\rm ACRB_{E,xy}}$ yields:
\begin{eqnarray}
	{\rm ACRB_{E,xy}}&\approx&\frac{8 r^3 (h+r)}{ N\eta}\times\Big(\frac{r \left(h^2+2 h r+2 r^2\right) (\zeta-1) \left(-6 h^2+6 h r+r^2 \zeta  (\zeta+1)-8 r^2\right)}{6 h^3}\nonumber\\
	&&+r \zeta \Big(\frac{-r^4 (\zeta^4-6\zeta^2+5)}{8 h^3}-\frac{r^3 \left(\zeta^2-1\right)}{2 h^2}+\frac{r^2 (\zeta^2-1)}{2 h}+h+r\Big)\nonumber\\
	&&-r (h+r)\Big)^{-1}
	\end{eqnarray}
	After reorganizing the formula, 
	\begin{eqnarray}
		{\rm ACRB_{E,xy}}&\approx&\frac{96 r^3h^3 (h+r)}{ N\eta}\times\Big(4 h^2 r^3(1-\zeta)^2 (\zeta+2)-h r^4 \left(\zeta^3+3 \zeta-4\right)\\\nonumber
		&&+\frac{1}{4} r^5 \left(-3 \zeta^5+26 \zeta^3-87 \zeta+64\right)\Big)^{-1}
	\end{eqnarray}
	As can be seen, in order to get a finit limit when $h$ goes to infinity, both the numerator and the denominator must have the same highest power of $h$. Thus, we divide ${\rm ACRB_{E,xy}}$ by $h^2$ and get the limit:
	\begin{equation}
		\lim_{h\rightarrow \infty}\frac{{\rm ACRB_{E,xy}}}{h^2}=\frac{24}{\eta N(\zeta+2) (1-\zeta)^2}
	\end{equation}
\subsection{${\rm ACRB_{E,z}}$}
\begin{eqnarray}
	{\rm ACRB_{E,z}}&=&\frac{2(r+h)}{\eta N}\Bigg[\frac{(h-D_M\zeta)((r+h)^2+r(r+h-D_{M}\zeta))}{2r^2D_{M}^2}-\frac{h(2r+h)}{2r^3} \log\Big(\frac{D_{M}}{h}\Big)\nonumber\\
	&&-\frac{[r+h-D_{M}^{-1}(r(h-D_{M}\zeta)+h(r+h))]^2}{r^3\log\Big(\frac{D_{M}}{h}\Big)}\Bigg]^{-1} 
\end{eqnarray}
When putting the approximations \ref{approxLog} and \ref{approxSqrt} in ${\rm ACRB_{E,z}}$ and reorganizing, we get a new shape of it:
\begin{eqnarray}
	{\rm ACRB_{E,z}}&\approx&\Big[192 h^3 (h+r) \left(6 h^2-6 h r-\left(\zeta^2+\zeta-8\right) r^2\right)\Big]\times\Big[\eta N (\zeta-1)\Big(-48 h^4 (\zeta-1)^2\nonumber\\
	&&-48 h^3 (\zeta(\zeta+7)-14) r-4 h^2 (\zeta-1) (\zeta+5) (\zeta (\zeta+7)-26) r^2\nonumber\\
	&&+4 h (\zeta-1) (\zeta (\zeta (7 \zeta+30)-15)-166) r^3\nonumber\\
	&&+3 (\zeta+1) \left(\zeta^2-5\right) \left(\zeta^3+\zeta^2+\zeta-15\right) r^4\Big)\Big]^{-1}
\end{eqnarray}
In order to get a finite limit, it is clearer now that ${\rm ACRB_{E,z}}$ must be divided by $h^2$, and this limit is the ratio between the highest power coefficients:
\begin{equation}
\lim_{h\rightarrow \infty}\frac{{\rm ACRB_{E,z}}}{h^2}=\frac{24}{\eta N(1-\zeta)^3}
\end{equation}
\end{IEEEproof}
As a result, we can produce an approximated formula, that is close to ${\rm ACRB_{E}}$ but simpler:
\begin{eqnarray}
	{\rm AACRB_{E,xy}}&=&\frac{-16r^2}{\eta N \Big(2\log\cos\phi_{max,\alpha}+\sin^2\phi_{max,\alpha}\Big)}+\frac{24h^2}{\eta N(\zeta+2) (1-\zeta)^2}\\
	{\rm AACRB_{E,z}}&=&\frac{4r^2}{\eta N\big[\sin^2\phi_{max,\alpha}+\frac{2(1-\cos\phi_{max,\alpha})^2}{\log\cos\phi_{max,\alpha}}\big]}+\frac{24h^2}{\eta N(1-\zeta)^3}
\end{eqnarray}


==> Chapters/sat_formulation.tex <==
	We consider a single land terminal (LT), at an unknown Earth location, that receives a known signal $s(t)$ from $M$ satellites. %isotropically over $\mathbb{R}^{3}$.
	 The signal transmission begins at time $t=T_0$, unknown to the receiver.
	\begin{figure}[t]
		\centering
		\includegraphics[width=0.6\textwidth]{newfiggood}
		\caption{System model. The satellites are randomally scattered around Earth in the gray sphere cup that defined by $\phi_{max}$.}
		\label{fig:sys_mod} 
	\end{figure}
\\
We assume that the satellites are located on a sphere with radius $R=r+h$ around the Earth, where $h$ is the height of the satellites from the Earth's surface, and $r$ is the Earth's radius, as illustrated in Fig. \ref{fig:sys_mod}. We further assume that the satellites are  identical independent distributed (i.i.d.) with a uniform distribution on the surface of the special cup of the sphere in which the satellites are deployed. I.e., the receiver is located on the ray from the center of the sphere and the apex of the cup (cf. Fig \ref{fig:sys_mod}) with a polar angle $\phi_{max}\in(0,\pi/2]$ that is centered above the receiver. The receiver's position is determined by three coordinates $(x,y,z)$. The estimation is based on a continuous time signal and exploits TDOA.
\par
 
	In the TDOA localiztion problem at hand, the unknown parameters of interest are the receiver coordinates $(x,y,z)$, and the signal initial transmission time, $T_0$. These are collected in a vector $\gammavec=[x,y,z,T_0]^T$. Moreover, the amplitudes\footnote{The amplitudes depend on the received signal gain, that depends on the transmission power, antenna gains, carrier frequency and the distance between the receiver and the satellite.} ${\bf a}=[A_1 \hdots A_M]^T$ are unknown nuisance parameters, and therefore the overall unknown parameter vector is given by $\tilde{\gamma}=[\gammavec^T, {\bf a}^T]^T$. Let $\psi_m=(x_m,y_m,z_m)\in\mathbb{R}^3$  be the location of satellite $m$, then the received signal observed at that satellite is given by \cite{YnoamIbergelTOA}
	\begin{equation}
	r_m(t)=A_m s(t-\tau_m-T_0)+v_m(t),~t\in\mathbb{R}_+,m\in\mathbb{N}
	\end{equation}
	where $s(t)$ is a known transmitted waveform and $v_m(t)$ is a white Gaussian noise with spectral density $N_0/2$. The time delay is given by $\tau_m = D_m/c$, where $c$ is the speed of light, and
	\begin{equation}
	D_m=\sqrt{(x_m-x)^2+(y_m-y)^2+(z_m-z)^2}
	\end{equation}
	is the distance between the receiver and the $m$-th satellite.\\
	This paper considers algorithms that use the TDOA and ignores the received signal strength (RSS). This is done because at long distances it is difficult to measure the amplitude attenuation accurately using RSS, and TDOA estimation usually yields better results. Accordingly, we ignore the information embedded in the amplitudes.
	% relevant references: myref11, weiss2003accuracy, Shang2009Multiuser
	 In Appendix A, it is shown that there is no coupling between the $\gammavec$ estimation and the ${\bf a}$ estimation. In more explicit terms, the cross entries of the FIM are zero and therefore, the CRB on the estimation error of $\gammavec$ is the same whether $\avec$ is known or unknown. Thus, the amplitudes are assumed known and we consider the unknown parameter vector is $\gammavec$.\par 
	 
	We assume that the following regularity conditions are satisfied. The signal $s(t)$  is continuous, differentiable,  $s(t)=0$ for all $t\leq 0$ and satisfies
	\begin{equation}
	|s(t)|, \left|\frac{ds(t)}{dt}\right|, \int_{0}^{\infty}|s(t)|dt,  \int_{0}^{\infty}\left|\frac{ds(t)}{dt}\right|dt <\infty.
	\end{equation} 
	Moreover, there exists a monotonic decreasing function $h(t)$, with $\int_{0}^{\infty}h(t)dt<\infty$, such that:
	\begin{equation}
	|s(t)|, \left|\frac{ds(t)}{dt}\right|\leq h(t)\qquad\forall t.
	\end{equation}
	Finally, we denote  $E_s\triangleq \int_{-\infty}^{\infty}s(t)dt$ and 
	\begin{equation}
	W_e\triangleq\frac{\int_{-\infty}^{\infty}(ds(t)/dt)^2dt}{\int_{-\infty}^{\infty}s^2(t)dt}
	\end{equation}
	where the latter is known as the effective bandwidth. In addition, we denote the signal energy when the satellite is exactly above the receiver by $E_{s,{\rm max}}$ where in the system described below, $E_{s,max}=E_s/h^2$. We also denote the polar angle that corresponds  satellite $m$ location by $\phi_m$, and the azimuth angle by $\theta_m$. In addition, we use two coordinate systems as follows:
	\begin{definition}
\begin{itemize}
	\item 		The $\alpha$ coordinate system is a spherical coordinate system that centered at the receiver.
	\item 	The $\beta$ coordinate system is a spherical coordinate system that centered at Earth's center.
\end{itemize}
	\end{definition}
	Note that the azimuth angle is the same in both coordinate systems; i.e., $\theta_{i,\alpha}=\theta_{i,\beta}$. The polar angles under both systems, $\phi_{m,\alpha}, \phi_{m,\beta}$, however, are different and related to each other as follows.
	\begin{equation}
	\sin\phi_{m,\alpha}=\frac{R}{D_m}\sin\phi_{m,\beta}\qquad \cos\phi_{m,\alpha}=\frac{R\cos\phi_{m,\beta}-r}{D_m}.
	\label{coordinateTransformation}
	\end{equation} 


==> Chapters/sat_formulation1.tex <==
	We consider a single land terminal (LT), at an unknown Earth location, that receives a known signal $s(t)$ from $M$ satellites. %isotropically over $\mathbb{R}^{3}$.
	 The signal transmission begins at time $t=T_0$, unknown to the receiver.
	\begin{figure}[t]
		\centering
		\includegraphics[width=0.7\textwidth]{newfiggood}
		\caption{System model. The satellites are randomally scattered around Earth in the gray sphere cup that defined by $\phi_{max}$.}
		\label{fig:sys_mod} 
	\end{figure}
\\
We assume that the satellites are located on a sphere with radius $R=r+h$ around the Earth, where $h$ is the height of the satellites from the Earth's surface, and $r$ is the Earth's radius, as illustrated in Fig. \ref{fig:sys_mod}. We further assume that the satellites are  identical independent distributed (i.i.d.) with a uniform distribution on the surface of the special cup of the sphere in which the satellites are deployed. I.e., the receiver is located on the ray from the center of the sphere and the apex of the cup (cf. Fig \ref{fig:sys_mod}) with a polar angle $\phi_{max}\in(0,\pi/2]$ that is centered above the receiver. The receiver's position is determined by three coordinates $(x,y,z)$. The estimation is based on a continuous time signal and exploits TDOA.
\par
 
	In the TDOA localiztion problem at hand, the unknown parameters of interest are the receiver coordinates $(x,y,z)$, and the signal initial transmission time, $T_0$. These are collected in a vector $\gammavec=[x,y,z,T_0]^T$. Moreover, the amplitudes\footnote{The amplitudes depend on the received signal gain, that depends on the transmission power, antenna gains, carrier frequency and the distance between the receiver and the satellite.} ${\bf a}=[A_1 \hdots A_M]^T$ are unknown nuisance parameters, and therefore the overall unknown parameter vector is given by $\tilde{\gammavec}=[\gammavec^T, {\bf a}^T]^T$. Let $\psi_m=(x_m,y_m,z_m)\in\mathbb{R}^3$  be the location of satellite $m$, and $\psivec_M=\{\psi_m\}_{m=1}^M$ is the collection of the locations of all the satellites. Then the received signal observed at that satellite is given by \cite{YnoamIbergelTOA}
	\begin{equation}
	r_m(t)=A_m s(t-\tau_m-T_0)+v_m(t),~t\in\mathbb{R}_+,m\in\mathbb{N}
	\label{rec_sig}
	\end{equation}
	where $s(t)$ is a known transmitted waveform and $v_m(t)$ is a white Gaussian noise with spectral density $N_0/2$. The time delay is given by $\tau_m = D_m/c$, where $c$ is the speed of light, and
	\begin{equation}
	D_m=\sqrt{(x_m-x)^2+(y_m-y)^2+(z_m-z)^2}
	\label{Dm}
	\end{equation}
	is the distance between the receiver and the $m$-th satellite.\par
		We assume that the following regularity conditions are satisfied. The signal $s(t)$  is continuous, differentiable,  $s(t)=0$ for all $t\leq 0$ and satisfies
	\begin{equation}
	|s(t)|, \left|\frac{\partial s(t)}{\partial t}\right|, \int_{0}^{\infty}|s(t)|dt,  \int_{0}^{\infty}\left|\frac{\partial s(t)}{\partial t}\right|dt <\infty.
	\end{equation} 
	Moreover, there exists a monotonic decreasing function $h(t)$, with $\int_{0}^{\infty}h(t)dt<\infty$, such that:
	\begin{equation}
	|s(t)|, \left|\frac{\partial s(t)}{\partial t}\right|\leq h(t)\qquad\forall t.
	\end{equation}
	Finally, we denote  $E_s\triangleq \int_{-\infty}^{\infty}s(t)dt$ and 
	\begin{equation}
	W_e\triangleq\frac{\int_{-\infty}^{\infty}(\partial s(t)/\partial t)^2dt}{\int_{-\infty}^{\infty}s^2(t)dt}
	\end{equation}
	where the latter is known as the effective bandwidth. In addition, we denote the signal energy when the satellite is exactly above the receiver by $E_{s,{\rm max}}$ where in the system described below, $E_{s,max}=E_s/h^2$. We also denote the polar angle that corresponds  satellite $m$ location by $\phi_m$, and the azimuth angle by $\theta_m$. In addition, we use two coordinate systems as follows:
	\begin{definition}
		\begin{itemize}
			\item 		The $\alpha$ coordinate system is a spherical coordinate system that centered at the receiver.
			\item 	The $\beta$ coordinate system is a spherical coordinate system that centered at Earth's center.
		\end{itemize}
	\end{definition}
	Note that the azimuth angle is the same in both coordinate systems; i.e., $\theta_{i,\alpha}=\theta_{i,\beta}$. The polar angles under both systems, $\phi_{m,\alpha}, \phi_{m,\beta}$, however, are different and related to each other as follows.
	\begin{equation}
	\sin\phi_{m,\alpha}=\frac{R}{D_m}\sin\phi_{m,\beta}\qquad \cos\phi_{m,\alpha}=\frac{R\cos\phi_{m,\beta}-r}{D_m}.
	\label{coordinateTransformation}
	\end{equation} 
	In this work, we examine both TDOA+RSS performance and TDOA performance. To avoid confusion, we use the subscript $\rm c$ for the complete model TDOA+RSS, and the subscript $\rm t$ for only TDOA.
	

==> Chapters/sat_formulation_rss.tex <==
	We consider a single land terminal (LT), at an unknown location, and $N$ satellites uniformly distributed all around Earth. The LT receives signals from $M$ satellites located in a sphere cup above it, as depicted in Fig. \ref{fig:sys_mod}. Let $N$ be the overall number of satellites that uniformly distributed in the same sphere around Earth.
	 The signal transmission begins at time $t = T_0$, unknown to the receiver. Usually, GNSS use CDMA to distinguish signals from different satellites; for example, GPS, Galileo, and BeiDou systems. Thus, the intersymbol interference is negligible. Moreover, we assume different satellite signals are transmitted at different times $T_m$, which are known to the LT, and chosen such that the inter symbol interference is negligible.
	\begin{figure}[t]
		\centering
		\includegraphics[width=0.7\textwidth]{newfiggood}
		\caption{System model. The satellites are randomally scattered around Earth, and the LT can receive only from satellites that are located in the gray sphere-cup, which is this paper dubbed LT look-cup, and is defined by $\phi_{max}$.}
		\label{fig:sys_mod} 
	\end{figure}
\par
We assume that the satellites are located on a sphere of radius $R=r+h$ around the Earth, where $h$ is the satellite height relative to Earth surface, and $r$ is Earth radius, as depicted in Fig. \ref{fig:sys_mod}. We further assume that the satellites are identical independent distributed (i.i.d.), uniformly around Earth. Moreover, we assume that the LT receives signals only from satellites located on the surface of the spherical cup above it, dubbed here as LT look-cup. Explicitly, the LT is located on the ray from the sphere center to the apex of the cup (cf. Fig \ref{fig:sys_mod}), with a polar angle $\phi_{max,l}\in(0,\pi/2]$ that is centered above the receiver. The receiver position $\xivec$ is represented by three coordinates $[x,y,z]^{\top}$. The estimation is based on continuous-time signals and hence, may eploit both TDOA and RSS information.
\par
 
	The unknown parameters are the receiver coordinates  vector $\xivec$, and the signal initial transmission time, $T_0$, which are collected in a vector $\gammavec=[\xivec^{\top},T_0]^{\top}$. 
	\begin{comment}
		Moreover, the amplitudes\footnote{The amplitudes depend on the received signal gain, that depends on the transmission power, antenna gains, carrier frequency and the distance between the receiver and the satellite.} ${\bf a}=[A_1 \hdots A_M]^{\top}$ are unknown nuisance parameters, and therefore the overall unknown parameter vector is given by $\tilde{\gammavec}=[\gammavec^{\top}, {\bf a}^{\top}]^{\top}$. 
	\end{comment}
	Let $\xivec_m=(x_m,y_m,z_m)\in\mathbb{R}^3$  be the location of satellite $m$, and $\xivec_1^N=\{\xivec_m\}_{m=1}^N$. The received signal from satellite $m$ is given by \cite{YnoamIbergelTOA}
	\begin{equation}
	r_m(t)=D_m^{-1} s(t-\tau_m-T_0-T_m)\mathbf{1}_{[\phi_{m,l}<\phi_{max,l}]}+v_m(t)
	\label{rec_sig}
	\end{equation}
	where $t\in\mathbb{R}_+,m\in\mathbb{N}$, $s(t)$ is a known transmitted waveform, $\mathbf{1}_{[\cdot]}$ is the indicator function and $v_m(t)$ is a white Gaussian noise with spectral density $N_0/2$. The time delay is given by $\tau_m = D_m/c$, where $c$ is the speed of light, and
	\begin{equation}
	D_m=\sqrt{(x_m-x)^2+(y_m-y)^2+(z_m-z)^2}
	\label{Dm}
	\end{equation}
	is the distance between the receiver and the $m$-th satellite.\par
	We assume that the following regularity conditions are satisfied: The signal $s(t)$  is continuous, differentiable,  equals $0$ for all $t\leq 0$ and satisfies \cite{YnoamIbergelTOA}
	\begin{equation}
	|s(t)|, \left|\frac{\partial s(t)}{\partial t}\right|, \int_{0}^{\infty}|s(t)|dt,  \int_{0}^{\infty}\left|\frac{\partial s(t)}{\partial t}\right|dt <\infty.
	\end{equation} 
	Moreover, there exists a monotonic decreasing function $g(t)$, with $\int_{0}^{\infty}g(t)dt<\infty$, such that:
	\begin{equation}
	|s(t)|, \left|\frac{\partial s(t)}{\partial t}\right|\leq g(t)\qquad\forall t.
	\end{equation}
	Finally, we denote  $E_{\rm s}\triangleq \int_{-\infty}^{\infty}s^2(t)dt$ and 
	\begin{equation}
	W_e\triangleq\frac{\int_{-\infty}^{\infty}(\partial s(t)/\partial t)^2dt}{\int_{-\infty}^{\infty}s^2(t)dt}
	\end{equation}
	where the latter is known as the effective bandwidth. In addition, we denote by $E_{\rm s,\max}$ the received signal energy if a satellite is located exactly above the receiver . Note that the latter serves as a reference energy and does not require a satellite in that location.  \par 
	We also denote the polar and azimuth angles corresponding to  satellite $m$ by $\phi_m$ and $\theta_m$, respectively. Furthermore, we use two coordinate systems as follows:
	\begin{definition}
	The ${\rm l}$ coordinate system is a spherical coordinate system that is centered at the LT.
	The ${\rm e}$ coordinate system is a spherical coordinate system that is centered at Earth center.
	\end{definition}
	Note that the azimuth angles are identical in both coordinate systems; i.e., $\theta_{m,l}=\theta_{m,e}=\theta_{m}$, whereas the polar angles, $\phi_{m,l}, \phi_{m,e}$, are different and related to each other as follows
	\begin{equation}
	\sin\phi_{m,{\rm l}}=\frac{R}{D_m}\sin\phi_{m,{\rm e}}\qquad \cos\phi_{m,{\rm l}}=\frac{R\cos\phi_{m,{\rm e}}-r}{D_m}.
	\label{coordinateTransformation}
	\end{equation} 


==> Chapters/sat_insights.tex <==
In this section we examine different insights of the bounds. 

what I want to write?
\begin{enumerate}
\item We suggest to decline the satellites height as possible.
 
\end{enumerate}
